Optimal Fairness Scheduling for Coded Caching in Multi-AP Multi-antenna WLAN

Coded caching (CC) schemes exploit the cumulative cache memory of network users, outperforming traditional uncoded schemes where cache contents are only used locally. Interestingly, this CC gain can also be combined with the spatial multiplexing gain of multi-antenna transmissions. In this paper, we extend the existing results of CC-aided data delivery in multi-access point (AP) wireless local area networks (WLAN) and video streaming applications by assuming multi-antenna transmitters at AP nodes. We present two distinct methods for using the extra resource that multi-antenna transmitters provide. While the first method tries to reduce the number of interference links in the network graph, the second one aims to remove inter-stream interference so that users with similar cache contents can be served simultaneously. While both methods provide increased throughput, they differ significantly in the underlying concept. Numerical simulations are used to compare the performance of different methods.

==> AnalyticalMethods.tex <==
In this section, we let $\alpha=1$ and first discuss codeword creation choices for a given activation pattern $\Bp_j$. Then, we review how the rate vector $\Br(j,s_j)$ can be calculated for policy $\pi(j,s_j)$, how the  utility function $\Sff$ could be optimized over $\mathrm{Conv}(\Br(j,s_j))$, and how the computation complexity of the optimization problem can be reduced by restricting the throughput region.

\subsubsection{Codeword Creation}
\label{section:codeowrd_creation}
Assume activation pattern $\Bp_j$ is given and helper $h_i$ is active in $\Bp_j$. Let us denote the set of users that can be served by $h_i$ as $\CU_i$. Clearly, $\CU_i$ includes the set of users within distance $r_{\mathrm{trans}}$ of $h_i$ but out of distance $r_{\mathrm{inter}}$ of every other active helper. Now, let us use $\CU_i^l$ to represent the subset of users of $\CU_i$ all assigned to the cache profile $l \in L$. In other words, for every $u_k \in \CU_i^l$ we have $\SfL(u_k) = l$. Let us use $\Sfl(i)$ to denote the number of $\CU_i^l$ sets, $l \in [L]$, for which $|\CU_i^l| = 0$.

The first step in codeword creation is to build a \emph{feasible} subset $\CV_i$ of $\CU_i$, where every user in $\CV_i$ is assigned to a different profile. Clearly, $|\CV_i| \le L-\Sfl(i)$, and the number of possible ways to build $\CV_i$ is $\prod_{l \in [L]} {(|\CU_i^l|+1)} - 1$, where addition with one (inside parentheses) is to account for the case no user is selected from $\CU_i^l$ and the subtraction of one is to exclude the empty set.

The users in a feasible set $\CV_i$ can be served by a number of codewords transmitted through helper $h_i$. To find these codewords, we build the \emph{support} set of $\CV_i$ as $\CL(\CV_i) =  \{l |$ s.t. $|\CV_i^l|>0,l\in{[L]}\}$ %\{\SfL(u_k), \forall u_k \in \CV_i \}$
, and then create its \emph{extended} set $\hat{\CV}_i$ by adding $L - |\CV_i|$ \emph{phantom} users $u_{l}^*$, $\SfL(u_l^*) = l$, for every $l \in [L] \backslash \CL(\CV_i)$. Next, a \emph{preliminary} codeword $\hat{X}(\hat{\CT}_i)$ can be built for every subset $\hat{\CT}_i$ of $\hat{\CV}_i$ with size $|\hat{\CT}_i| = t+1$ as
\begin{equation}
    \hat{X}(\hat{\CT}_i) = \bigoplus_{u_{k} \in {\hat{\CT}_i}} W_{d_{k}, \CL(\hat{\CT}_i) \backslash \SfL(u_k) } ,
\end{equation}
where $\CL({\hat{\CT}_i}) = \{\SfL(u_k), \forall u_k \in \hat{\CT}_i \}$ and $d_k \in [N]$ is the index of the file requested by $u_k$. Finally, the codeword $X(\CT_i)$ is built from $\hat{X}(\hat{\CT}_i)$ by removing the effect of phantom users. Note that $\CT_i$ denotes the set resulting after phantom users are removed from $\hat{\CT}_i$. The following example clarifies this process.

\begin{exmp}
\label{exmp:codeword_creation}
    Consider the network shown in Figure~\ref{fig:network_model}. Assume $L=3$ and $t=1$. 
    Let us consider the activation pattern $\Bp_j = [0,1]$. For active helper $h_2$, we have $\CU_2^1 = \{u_4\}$, $\CU_2^2 = \{u_3,u_5\}$, and $\CU_2^3 = \varnothing$. We have five options to choose $\CV_i$; let us assume $\CV_2 = \{u_3,u_4\}$, and hence, $\CL(\CV_2) = \{1,2\}$ and $\hat{\CV}_2 = \{u_3,u_4,u_3^*\}$. We have three subsets $\hat{\CT}_2$ of $\hat{\CV}_i$ with size $t+1$, resulting in preliminary codewords
    \begin{equation*}
        \begin{aligned}
            \hat{X}(\{u_3,u_4\}) &= W_{d_3,\{2\}} \oplus W_{d_4,\{1\}}, \\
            \hat{X}(\{u_3,u_3^*\}) &= W_{d_3,\{3\}} \oplus W_{d_{3^*},\{1\}}, \\
            \hat{X}(\{u_4,u_3^*\}) &= W_{d_4,\{3\}} \oplus W_{d_{3^*},\{2\}}. \\
        \end{aligned}
    \end{equation*}
    After removing the effect of phantom users, final codewords are built as $X(\{u_3,u_4\}) = W_{d_3,\{2\}} \oplus W_{d_4,\{1\}}$, $X(\{u_3\}) = W_{d_3,\{3\}}$, and  $X(\{u_4\}) = W_{d_4,\{3\}}$.
\end{exmp}

The codeword creation process clarifies exactly which codewords are generated for any given feasible set $\CV_i$. As a result, the total number of policies for activation pattern $\Bp_j$ can be calculated as
\begin{equation}
\label{eq:activation_pattern_count}
    \Sfc(\Bp_j) = \prod_{\substack{i \in [H]\\ \Bp_j[i] = 1}} \big( \prod_{l \in [L]} {(|\CU_i^l|+1)} - 1 \big) .
\end{equation}

% \begin{figure}[t]
%     \centering
%     \begin{tikzpicture}[scale=0.4,transform shape]          
%         \tikzstyle{helper}=[circle, draw=red!50,fill=red!50,scale=1.8]
%         \tikzstyle{user}=[circle, draw=blue!50,fill=blue!50]

%         \node[user] (User1) at (2,0) {$1(1)$} ;
%         \node[user] (User2) at (6,0) {$2(3)$};
%         \node[user] (User3) at (10,0) {$3(2)$};
%         \node[user] (User4) at (14,0) {$4(1)$};
%         \node[user] (User5) at (18,0) {$5(2)$};
        
%         \node[helper] (Helper1) at (6,5) {$1$} ;
%         \node[helper] (Helper2) at (14,5) {$2$} ;
        
%         \draw (Helper1) to (User1);
%         \draw (Helper1) to (User2);
%         \draw (Helper1) to (User3);
%         \draw[loosely dashed] (Helper2) to (User2);
%         \draw (Helper2) to (User3);
%         \draw (Helper2) to (User4);
%         \draw (Helper2) to (User5);
%     \end{tikzpicture}
%     \caption{Caption}
%     \label{fig:network_graph}
% \end{figure}

%\todo[inline]{the old text (more general one)}

%Every codeword transmitted through helper $h_i$ should include useful data for a subset of users of $\CU_i$. Let us use $\CV_i$ to denote a general subset of $\CU_i$ and call $\CV_i$ is \emph{feasible} if it is possible to create a codeword $X(\CV_i)$ that includes useful data for every user $u_k \in \CV_i$. From~\cite{caire}, two necessary conditions for the feasibility of $\CV_i$ are 1) $0 < |\CV_i| \le t+1$ and 2) every user in $\CV_i$ is assigned to a different cache profile, i.e., $\SfL(u_k)$ is distinct for every $u_k \in \CV_i$. 

%In order to find the number of feasible subsets $\CV_i$, we first define $\CL$ to denote any subset of $[L]$ with size $|\CL| = t+1$. For a given $\CL$, picking at most one user from every $\CU_i^l$, $l \in \CL$, results in a feasible subset. Let us use $\CV_i^{\CL}$ to denote such a feasible subset. Clearly, there exist $\prod_{l \in \CL} {(|\CU_i^l|+1)} - 1$ possibilities for $\CV_i^{\CL}$, where addition with one (inside parentheses) is to account for the case no user is selected from $\CU_i^l$, and the subtraction of one is to exclude the empty set. As a result, the total number of possible codewords to be transmitted through helper $h_i$ is
%\begin{equation}
%    \sum_{\substack{\CL \subseteq [L] \\ |\CL| = t+1}} \big( \prod_{l \in \CL} {(|\CU_i^l|+1)} - 1 \big) ,
%\end{equation}
%and the total number of policies for activation pattern $\Bp_j$ is
%\begin{equation}
%\label{eq:activation_pattern_count}
%    \Sfc(\Bp_j) = \prod_{\substack{i \in [H]\\ \Bp_j[i] = 1}} \sum_{\substack{\CL \subseteq [L] \\ |\CL| = t+1}} \big( \prod_{l \in \CL} {(|\CU_i^l|+1)} - 1 \big) .
%\end{equation}

%Now, let us review how the codeword $X(\CV_i^{\CL})$ is made for a feasible $\CV_i^{\CL}$. The first step is that for every profile index $l \in \CL$, if there is no user in $\CV_i^{\CL}$ assigned to cache profile $l$, we add a \emph{phantom} user $u_{l^*}$ to $\CV_i^{\CL}$, such that $\SfL(u_{l^*}) = l$. Then, similar to~\cite{caire}, we create the \emph{preliminary} XOR codeword $\hat{X}(\CV_i^{\CL})$ as
%\begin{equation}
%    \hat{X}({\CV}_i^{\CL}) = \bigoplus_{u_{k} \in {\CV}_i^{\CL}} W_{d_{k}, \CL \backslash \SfL(u_k) } ,
%\end{equation}
%where $W_{d_k}$ denotes the video chunk requested by $u_k$ (for phantom users, this can be any chunk), and $\oplus$ represents the XOR operation over a finite field. Finally, the real codeword ${X}(\CV_i^{\CL})$ is found by removing the effect of phantom users from $\hat{X}(\CV_i^{\CL})$. The following example clarifies this process.

%\begin{exmp}
%\label{exmp:codeword_creation}
%Consider the network shown in Figure~\ref{fig:network_model}, for which the graph representation and cache profile assignment are shown in Figure~\ref{fig:network_graph}. Assume $L=3$ and $t=1$. 

%Let us consider the activation pattern $\Bp_j = [0,1]$. Then, for active helper $h_2$, we have $\CU_2^1 = \{u_4\}$, $\CU_2^2 = \{u_3,u_5\}$, and $\CU_2^3 = \varnothing$. Also, as $L=3$ and $t=1$, we have three choices for $\CL$. We review possible codewords for $\CL = \{1,2\}$ and $\CL = \{1,3\}$:
%\begin{itemize}
%    \item If $\CL=\{1,2\}$, we don't need any phantom users, and five codewords can be created as $X(\{u_4\}) = W_{d_4,2}$, $X(\{u_3\}) = W_{d_3,1}$, $X(\{u_5\}) = W_{d_5,1}$, $X(\{u_4,u_3\}) = W_{d_4,2} \oplus W_{d_3,1}$, and $X(\{u_4,u_5\}) = W_{d_4,2} \oplus W_{d_5,1}$.
%    \item If $\CL=\{1,3\}$, we first need to add a phantom user $u_{3^*}$ to $\CU_2^3$. One preliminary codeword can be built as $\hat{X}(\{u_4,u_{3^*}\}) = W_{d_4,3} \oplus W_{d_{3^*},1}$. After removing the effect of $u_{3^*}$, we get ${X}(\{u_4\}) = W_{d_4,3}$.
%\end{itemize}
%It can be easily verified that after the transmission of a codeword $X(\CV_i^{\CL})$, every user $u_k \in \CV_i^{\CL}$ can remove unwanted terms using its cache contents and decode a subpacket of its requested video chunk interference-free.

%\begin{rem}
%\label{rem:maximum_codeword_length}
%    Codeword creation helps improve the rate as the same multicast message can be used by multiple users. Thus we can safely assume that for every $\CL$, only feasible subsets $\CV_i^{\CL}$ with the maximum size are selected. In other words, for a given $\CL$, as long as $|\CU_i^l| > 0$ for $l \in \CL$, we pick exactly one user from $\CU_i^l$ to built $\CV_i^{\CL}$. It can be seen that with this approach, the number of policies for activation pattern $\Bp_j$ is upper-bounded by
%    \begin{equation}
%    \label{eq:activation_pattern_count_bound}
%        \Sfc(\Bp_j) \le \prod_{\substack{i \in [H]\\ \Bp_j[i] = 1}} \sum_{\substack{\CL \subseteq [L] \\ |\CL| = t+1}} \prod_{l \in \CL} {\max(|\CU_i^l|,1)} .
%    \end{equation}
%\end{rem}

%\end{exmp}

\subsubsection{Rate Calculation}
%As discussed, every policy $\pi(j,s_j)$ results in a rate vector $\Br(j,s_j)$. 
Let us consider an activation pattern $\Bp_j$ and an active helper $h_i$ in this pattern. It can be easily verified that after the codeword creation process of Section~\ref{section:codeowrd_creation}, every user $u_k$ in the feasible set $\CV_i$ can successfully decode their requested chunk after $ \Sfn(\CV_i) = {\binom{L}{t+1} - \binom{L-|\CV_i|}{t+1}}$ codeword transmissions. Hence, the rate of every user $u_k \in \CV_i$ can be simply calculated as $r(\CV_i) = {1}/{\Sfn(\CV_i)}$. 
%\begin{equation}
    %$r(\CV_i) = {1}/({\binom{L}{t+1} - \binom{L-|\CV_i|}{t+1}})$.
%\end{equation}
%which results from the fact that only phantom users appear in $\binom{L-|\CV_i|}{t+1}$ number of preliminary codewords $\hat{X}(\hat{\CT}_i)$. 
Now, to find the rate vector $\Br(j,s_j)$, we only need to 1) for every active helper $h_i$, choose the feasible set $\CV_i$, 2) for every $u_k \in \CV_i$, set the element $k$ of the vector $\Br(j,s_j)$ as $r(\CV_i)$, and 3) fill other elements of $\Br(j,s_j)$ as zero. Note that $r(\CV_i)$ is calculated according to the fact that $\binom{L-|\CV_i|}{t+1}$  preliminary codewords $\hat{X}(\hat{\CT}_i)$ are ignored as they include only phantom users.
%only phantom users appear in $\binom{L-|\CV_i|}{t+1}$ number of preliminary codewords $\hat{X}(\hat{\CT}_i)$. 

%every user $u_k$ in the feasible set $\CV_i$ appears exactly in the same number of codewords, and hence, perceives the same rate $r({\CV_i})$. Also, as the number of codewords increases, every $u_k \in \CV_i$ appears in a smaller share of all codewords, and $r({\CV_i})$ is decreased. As the goal is to optimize a fairness function over $\mathrm{Conv}(\Br(j,s_j))$, any scaling in rate values does not change the optimal solution. So, without any loss of generality, we can choose
%Recall that the goal is to find $a(j,s_j)$ values maximizing the proportional fairness function $\Sff = \sum_k \log(r_k)$. Any scaling in rate values does not change the optimal solution as it only changes $\Sff$ by a constant, and hence, we can choose the time unit freely. For convenience, let us choose the time required to deliver one codeword via a helper as the unit. 


%For every helper $h_i$, the total number of $\CL$ sets resulting in at least one possible codeword $X(\CV_i^{\CL})$ is $\Sfn(i) = \binom{L}{t+1}-\binom{\Sfl(i)}{t+1}$, where $\Sfl(i)$ is the number of $l$ values for which $|\CU_i^l| = 0$.
%In the general case, we may select only a selection of all such $\CL$ sets. However, this makes the optimization problem intractable as the bound on the number of policies per activation pattern in~\eqref{eq:activation_pattern_count_bound} grows by a factor of $\CO \big(2^{H \binom{L}{t+1}} \big)$. To avoid this issue, we only consider the \emph{maximal} case where 1) a total number of $\Sfn(i)$ codewords are transmitted through every active helper $h_i$ and 2) every user receiving data from $h_i$ appears in the same number of codewords.\footnote{In fact, the name `maximal' is chosen as the coded caching gain is maximized with these constraints. However, proving the global optimality of the maximal case is challenging and is part of our ongoing research.} This results in the perceived maximal rate of $r_{\Sfk(i)} = \frac{1}{\Sfn(i)}$ for every user receiving data from $h_i$.

%Now, to find the rate vector $\Br(j,s_j)$, we need to follow these steps: 1) for every active helper $h_i$, find the set of users receiving data from $h_i$ in policy $\pi(j,s_j)$, 2) for every such user $u_k$, we set the element $k$ of the vector $\Br(j,s_j)$ as $r_{\Sfk(i)}$, and 3) we fill other elements of $\Br(j,s_j)$ as zero. The following example clarifies this procedure.

\begin{exmp}
\label{exmp:rate_vector}
    Consider the same network and activation pattern as in Example~\ref{exmp:codeword_creation}. For active helper $h_2$, if $\CV_2 = \{u_3,u_4\}$, we get the three codewords shown in Example~\ref{exmp:codeword_creation}, and the rate vector is $[0,0,\frac{1}{3},\frac{1}{3},0]$. Similarly, it can be seen that for $\CV_2 = \{u_3\}$, we get two codewords $X(\{u_3\}) = W_{d_3,\{2\}}$ and $X(\{u_3\}) = W_{d_3,\{3\}}$, and the rate vector becomes $[0,0,\frac{1}{2},0,0]$.
    
    %As $|\CU_2^l| = 0$ only for $l=3$, we have $\Sfl(2) = 1$ and $\Sfn(2) = 3$. Assume for selections of $\CL$ as $\{1,2\}$, $\{1,3\}$, $\{2,3\}$, codewords $X(\{u_3,u_4\})$, $X(\{u_4\})$, $X(\{u_3\})$ are selected for transmission, respectively. Then, for this policy, the maximal rate vector will be $\Br(j,s_j) = [0,0,\frac{1}{3},\frac{1}{3},0]$.
\end{exmp}

We call a rate vector $\Br(j_1,s_{j_1})$ to be \emph{dominated} by $\Br(j_2,s_{j_2})$ if every element of $\Br(j_1,s_{j_1})$ is smaller than or equal to the corresponding element of $\Br(j_2,s_{j_2})$, and at least one element is strictly smaller. We call a rate vector \emph{maximal} if it is not dominated by any other rate vector.

Larger feasible sets $\CV_i$ result in more users being served and enhance multicasting. As a result, we restrict ourselves to maximal rate vectors that also maximize the coded caching gain for each helper. These vectors correspond to sets $\CV_i$ with the maximum possible length, i.e., $|\CV_i| = L-\Sfl(i)$.\footnote{Proving that the same fairness optimality is achieved after restricting the convex hull to the maximal rate vectors that also maximize the coded caching gain is not obvious and may depend on the specific fairness function.} With this choice, the rates of users in $\CV_i$ become $r_{\Sfk(i)} = {1}/({\binom{L}{t+1}-\binom{\Sfl(i)}{t+1}})$. It can also be easily verified that the number of policies per activation pattern $\Bp_j$ gets upper bounded by
\begin{equation}
\label{eq:activation_pattern_count_maximal}
    \Sfc(\Bp_j) \leq \prod_{\substack{i \in [H]\\ \Bp_j[i] = 1}} \prod_{l \in [L]} {\max(|\CU_i^l|,1)} ,
\end{equation}
where the inequality results from the rate vectors that maximize the coded caching gain for each active helper but are not necessarily maximal.

\subsection{The Optimization Problem}
\label{section:analytical_solution}
As mentioned in Section~\ref{section:sys_model}, in this paper, we aim to optimize the proportional fairness function over $\mathrm{Conv}(\Br(j,s_j))$. So, we need to solve the following convex optimization problem:
\begin{equation}
\label{eq:optimization_problem_main}
    \begin{aligned}
        \max_{a(j,s_j)} \Sff &= \sum_{k \in [K]} \log(\Br_{\mathrm{sum}}[k]) \\
        s.t. \qquad & \Br_{\mathrm{sum}} = \sum_{j \in [2^H]} \sum_{s_j \in [\Sfc(\Bp_j)]} a(j,s_j) \Br(j,s_j), \\
        & a(j,s_j)\geq{0}, \quad \sum_{j \in [2^H]} \sum_{s_j \in [\Sfc(\Bp_j)]} a(j,s_j) = 1 . \\
        %& 0 \le a(j,s_j) \le a_{\max}, \quad \forall j\in[2^H], s_j \in [\Sfc(\Bp_j)],
    \end{aligned}
\end{equation}
%the optimization problem can be formulated easily. Recalling that $r_k$ is the element $k$ of $\Br_{\mathrm{sum}}$, we need to solve
%\begin{equation}
%\label{eq:optimization_problem_main}
%    \begin{aligned}
%        \max_{a(j,s_j)} \Sff &= \sum_{k \in [K]} \log(r_k) \\
%        s.t. \qquad & \Br_{\mathrm{sum}} = \sum_{j \in [2^H]} \sum_{s_j \in [\Sfc(\Bp_j)]} a(j,s_j) \Br(j,s_j), \\
%        & 0 \le a(j,s_j) \le 1, \quad \forall j\in[2^H], s_j \in [\Sfc(\Bp_j)].
%    \end{aligned}
%\end{equation}
%where $a_{\max}$ avoids unbounded growth of $\Sff$.
%The constraint $a(j,s_j) \le 1$ is added to avoid unbounded growth of $\Sff$. The optimization problem~\eqref{eq:optimization_problem_main} is convex and can be solved with any available solver. 
The problem with this optimization problem is its large dimensions: there exist $2^H$ activation patterns and the number of policies per activation pattern in the order given by~\eqref{eq:activation_pattern_count_maximal}. This number grows very large, even for moderate-sized networks. %For example, \textbf{put an example case here}.

\begin{rem}
    The optimization problem in~\eqref{eq:optimization_problem_main} can also be interpreted as a scheduler design problem, where we aim to find the amount of resource (frequency, time, power, etc.) allocated to policy $\pi(j,s_j)$. For example, if each policy $\pi(j,s_j)$ is activated over a different time slot, $a(j,s_j)$ represents the normalized length of that time slot.
\end{rem}

%\begin{rem}
%The complexity of~\eqref{eq:optimization_problem_main} can be reduced by removing rate vectors %that are \emph{dominated} by others. We call a vector $\Br(j_1,s_{j_1})$ to be dominated by %$\Br(j_2,s_{j_2})$ if every element of $\Br(j_1,s_{j_1})$ is smaller than or equal to the %corresponding element of $\Br(j_2,s_{j_2})$. 
%%It is clear that in this case, $a(j_1, s_{j_1}) = 0$ in the optimal solution. 
%Although this idea reduces the optimization complexity, finding the set of dominated rate %vectors requires an exhaustive search, adding to the computational complexity.
%\end{rem}

%\begin{rem}
%Solving~\eqref{eq:optimization_problem_main} is not the only way to achieve the optimality of the fairness function. It can be %done algorithmically, as time-averaged rates of the virtual queue method (Lyapunov Drift Plus Penalty) according to the well-%known approach in~\cite{georgiadis2006resource}. However, such a scheduler needs to 
%collect the status of the virtual queues for each user and 
%solve at each scheduling slot the weighted sum rate problem over rate vectors, which requires the enumeration of all possible %rate vectors and essentially has the same complexity of solving~\eqref{eq:optimization_problem_main} directly. The dynamic DPP %scheduling algorithm has the advantage of being ‘on-line,' i.e., if the network topology evolves with time (e.g., users move and %join/leave the network), the algorithm seamlessly adapts to the new topology (reflected by changes in the set of maximal rate %vectors).
%\end{rem}

\subsection{The Super-user Solution}
\label{section:super-user}
The complexity of the optimization problem~\eqref{eq:optimization_problem_main} can be reduced significantly by restricting the network throughput region (i.e., reducing $\mathrm{Conv}(\Br(j,s_j))$). The idea is that, for every activation pattern $\Bp_j$, we reduce the number of policies $\Sfc(\Bp_j)$ to one by grouping users being served by the same active helper and assigned to the same cache profile into a \emph{super-user}. Then, the rate of every super-user is shared equally among all the users forming that super-user, as in the codeword formation, users sharing the same cache profile are interchangeable (i.e., the same codeword can carry data for any of these users).
This affects the rate vectors: for every active helper $h_i$ in pattern $\Bp_j$, if $u_k \in \CU_i$, we fill the element $k$ of $\Bar{r}(j,s_j)$ with $\frac{r_{\Sfk(i)}}{|\CU_i^{\SfL(u_k)}|}$.
The super-user approach imposes some ``local’’ fairness among the users sharing the same cache profile and served by a common active helper. However, it generally restricts the convex hull, resulting in the throughput region getting smaller. As a result, the optimum of the fairness function could deteriorate compared with the solution of the original problem. 
%
%From~\eqref{eq:activation_pattern_count}, the main contributor in $\Sfc(\Bp_j)$ is $|\CU_i^l|$, which denotes the number of selections we have for choosing the user to be served by active helper $h_i$ among the set of users assigned to cache profile $l$. The super-user method basically removes this problem by giving all users in $\CU_i^l$ an equal share of the time to receive part of their requested data. 
%
%The effects appear in the rate vector $\Bar{r}(j,s_j)$: 


%For every activation pattern $\Bp_j$, we have one super-user policy $\Bar{\pi}(j,1)$, for which the rate vector $\Bar{\Br}(j,1)$ is the average of all the maximal rate vectors of the policies for the same activation pattern in the original setup, i.e., $\Br(j,s_j)$ for all $s_j \in \Sfc(\Bp_j)$.

\begin{exmp}
    Consider the same network and activation pattern as in Example~\ref{exmp:codeword_creation}. 
    Following the discussions in Example~\ref{exmp:rate_vector}, we have $r_{\Sfk(2)} = \frac{1}{3}$. As a result, the rate vector $\Bar{r}(j,s_j)$ for the super-user case is given as $[0,0,\frac{1}{6},\frac{1}{3},\frac{1}{6}]$.
    %A maximal rate vector $[0,0,\frac{1}{3},\frac{1}{3},0]$ for this network is provided in Example~\ref{exmp:rate_vector}. It can be verified that there exists another maximal rate vector $[0,0,0,\frac{1}{3},\frac{1}{3}]$, if we choose codewords $X(\{u_4,u_5\})$, $X(\{u_4\})$, and $X(\{u_5\})$ for transmission. Now, with the super-user method, we group users $u_3$ and $u_5$ into a super-user, and the new rate vector will be $[0,0,\frac{1}{6},\frac{1}{3},\frac{1}{6}]$. 
\end{exmp}

%It should be noted that the super-user solution only affects the way we calculate the portion %of resources assigned to each policy; the codewords transmitted through helpers are the same %as before. Moreover, as we have restricted $\mathrm{Conv}(\Br(j,s_j))$, it may result in a sub-%optimal solution to~\eqref{eq:optimization_problem_main}. 
%%In Section~\ref{section:sim_results}, we use numerical simulations to investigate this gap. 
%Nevertheless, the complexity is reduced significantly.%; for example, \textbf{put the example %here. we may reuse the example in the previous subsection}.



%\todo[inline]{Mohammad to revise parts of this section by 27.1}

%Let $G$ be a graph such that the set of vertices $\mathbf{V}$ of $G$ can be written as $\mathbf{V}=\mathbf{H}\bigcup{\mathbf{U}}$ where $\mathbf{H}$ is the set of helpers and $\mathbf{U}$ is the set of users. Let $\mathbf{E}$ be the edge set of $G$ such that $\mathbf{E}=\mathbf{E}_t\bigcup{\mathbf{E}_i}$ where $\mathbf{E}_t$ corresponds to the set of the transmission edges and $\mathbf{E}_i$ corresponds to the set of the interference edges. Every $e\in{\mathbf{E}}$ can be written as $e=hu$(or $uh$) where $h\in{\mathbf{H}}$  and $u\in{\mathbf{U}}$. So $G$ is a actually a bipartite graph with an additional degree of freedom, i.e. there are two different kinds of edges. 

%We assume that for every user $u_k\in{\mathbf{U}}$ there is at least one edge $e\in{\mathbf{E}_t}$ adjacent to $u_k$, i.e. $\exists$ $h\in{V}$ such that  $hu_k\in{\mathbf{E}_t}$, otherwise one can not reliably transmit a message to user $u_k$. If there are some users which can not be served, we don't include those users in the transmission topology. We are not interested in the outage probability for the sake of this paper.

%Let degree $d(v)$ of a vertex $v\in{\mathbf{V}}$ be the number of edges adjacent to $v$.

%(Helpers transmit the messages to the users column by column.)

%In any kind of delivery scheme one can construct, one has maximum of $2^H$ helper activation pattern, i.e. a helper can either be `active' or `inactive' at the same time. Let us fix an activation pattern. We first find the users to which we can multicast XOR messages. To do that, we erase the edges adjacent to the vertices of corresponding to `inactive' helpers $h_i$ from the graph, we also erase the edges adjacent to users $u_k$ with degree $d(u_k)>1$ or $d(u_k)=1$ and its adjacent edge $e\in{\mathbf{E}_i}$ so that in the graph the users $u_k$ with positive degree $d(u_k)>0$ all have $d(u)=1$ with transmission edges $e_t$ adjacent to them which are the users we can reliably multicast XOR messages. Which user combinations one can serve in a delivery column of a helper depends on the cache configuration. Let us fix a user combination. The `active' helpers serve the users in respective delivery columns, however since the number of users in their delivery columns may be different, their finishing times of their respective columns may also differ. Let $T_k$, $k\in\lbrace1,2,...,\rbrace$ be the delivery time of the user $u_k$ which is the finishing time of the delivery column  where the user $u_k$ is. We say that the `instantaneous rate' $IR_k$ of the user $u_k$ which is the percentage of  the demanded file received per XOR transmission is $1/T_k$ if $T_k>0$ or $0$, i,e, if the user is not served, otherwise. Then the instantaneous rate vector $\mathbf{IR}$ for this helper activation pattern and user combination is given by $[IR_1,IR_2,...,IR_K]$. We say that an instantaneous rate vector $\mathbf{IR'}$ is `dominated' by another instantaneous rate vector $\mathbf{IR^{''}}$ if $IR'_k\leq{}IR^{''}_k$ $\forall{}k\in{\lbrace1,2,...,K\rbrace}$ and $\exists{}k$ such that $IR'_k<IR^{''}_k$.



%\subsection{Optimal solution using the extended matrix}

%By going through all the helper activation patterns and user combinations we list all the instantaneous rate vectors and we erase the instantaneous rate vectors which are dominated by other rate vectors from the list and we erase the duplicates from the list. We call these instantaneous rate vectors `maximal' instantaneous rate vectors since each of them is not dominated by one other. We put these maximal instantaneous rate vectors into a matrix $\mathbf{MIR}$ such that each row of  $\mathbf{MIR}$ corresponds to a maximal instantaneous rate vector.

%By using (time division) we can achieve any rate in the convex hull of the maximal instantaneous rate vectors and it is easy to see that since the instantaneous rate vectors in $\mathbf{MIR}$ are maximal, any (final or average vector) we can achieve by (any delivery scheme) is either be dominated by the convex hull of the vectors in $\mathbf{MIR}$ or it will exactly lie in the in the convex hull. Since we use proportional fairness utility function as our metric ($pf(\mathbf{R}):=\sum_{R_k}\log(R_k)$), what we want to achieve is 
%\begin{equation}
%\max_{\mathbf{a}}{pf(\mathbf{a}^T\mathbf{MIR})}     
%\end{equation}
%such that 
%\begin{eqnarray}
%\mathbf{a}^T\mathbf{1}=1 \\
%\mathbf{a}\geq{0}
%\end{eqnarray}
%$\mathbf{a}^*$ which maximizes this convex optimization problem gives us the optimal rate $\mathbf{R}^*=(\mathbf{a}^{*})^{T}\mathbf{MIR}$.

%We (assume, or don't assume, or prove in appendix, or it is easy to see) that if the helpers maximize their coded caching gain, i.e. they serve maximum number of users possible in every helper activation pattern, and we just take into consideration these maximal instantaneous rate vectors to construct $MIR$, this is also optimal. And this drastically decreases the computational load and also it is interesting to notice this from a theoretical perspective.

==> Extended_Summary.tex <==

\begin{itemize}
\color{blue}
    \item Generally, Creating Different Sections such as Introduction, System Model, MISO part and SISO part, and Simulation Results and dividing the text and incorportating them appropriately and expanding them when necessary
    \item Do we explicitly write about the difference between spatial multiplexing gain and the number of antennas, if so we must I think then add more notation and technical explanation
    \item Do we talk about the assumption that for MIMO, beamforming does not change connectivity/interference of the other users? Or just leave it like that?
    \item We should definitely give an example for interference nulling, explain mathematically and technically the cache congestion control scheme in a general notation (I have done this before it should be somewhere in this document, I can revise it).% The thing is that it would be nice if we can also explain mathematically in a general way interference nulling also but how? For instance, Giuseppe said interference nulling does not need signal level coding, on the contrary cache congestion control needs signal level coding due to zero forcing vectors. I am not expert in this area, then how do we write mathematically interference nulling more rigorously and if it is not done in signal level where do we do interference nulling explicitly in reality? Because from my point of view, zero forcing in a simpler manner can also do interfrence nulling but then it is still in signal level:) But maybe these last parts are not too important.
    \item Simulation for instance for 3 antennas and also give an example from the figure where one antenna is used for cache control and the other antenna is used for interference nulling. We can leave this to do in the end, also if there is space we may add more simulations.
    \item Do we clarify and extend the discussion regarding degree of freedom (DoF) difference between two methods(in last paragraph of text)? One issue is how to define them appropriately, and if we can define, the other issue is maybe calculating them for our topological parameters. These might be done easily but I am not sure if we have enough space for these? We may also think about these in the end I think.
\end{itemize}

The increasing amount of data traffic, especially driven by multimedia applications, has necessitated more efficient usage of existing network resources and exploring new possibilities. One interesting resource is on-device memory; it is cheap and can be used to store a large part of multimedia content proactively. In this regard, coded caching (CC) techniques provide an exciting opportunity to use memory as a communication resource, as they enable a speedup factor in the achievable rate that scales with the cumulative cache size in the network~\cite{maddah2014fundamental} and is additive with the spatial multiplexing gain of multi-antenna communications~\cite{shariatpanahi2018physical,parrinellomultiantenna}.

%, e.g., for video-on-demand (VoD) and extended reality (XR) applications. Many researchers have considered the efficient use of onboard memory in the context of \emph{caching}, with pioneering works introducing femtocaching~\cite{shanmugam2013femtocaching} and F-RAN models~\cite{park2016joint}. A major breakthrough later happened with the introduction of coded caching (CC)~\cite{maddah2014fundamental}, which showed a speedup factor in the achievable rate, scaling with the cumulative cache size in the network, is possible by multicasting carefully created codewords. Later, many works extended the original work of~\cite{maddah2014fundamental}, e.g., for wireless~\cite{tolli2017multi}, multi-server~\cite{shariatpanahi2016multi}, and multi-antenna~\cite{shariatpanahi2018physical,parrinellomultiantenna} networks. Meantime, many challenges hindering the applicability of CC techniques in real networks were addressed. For example, the subpacketization bottleneck was studied for single- and multi-antenna setups~\cite{lampiris2018adding,salehi2020lowcomplexity}, simpler beamformer designs were introduced~\cite{salehi2020lowcomplexity,mahmoodi2021low}, and the problem of supporting network dynamicity was addressed~\cite{caire,salehi2021low,abolpour2022coded}.

This paper considers a coded caching system model originally proposed in~\cite{mozhgan} and later extended in~\cite{akcay2023optimal} for two-hop wireless local area networks (WLAN), where a single server transmits data to a large number of users through multiple access points (AP), hereby called \textit{helper} nodes.
%WLANs play an essential role in our everyday lives; they facilitate data access, e.g., in our homes, malls, airports, and cars. 
Two important properties of WLANs are a) unit frequency reuse due to the scarce availability of unlicensed bands and b) the collision-type interference model (i.e., packets are lost if a receiver gets the superposition of concurrent packets, all above a certain interference threshold, from different helpers). Considering multi-helper WLANs and single per-user requests, the authors in~\cite{mozhgan} 
used the multi-round delivery method in~\cite{caire} (which was later proved by~\cite{parrinellomultiantenna} to be optimal for the shared-cache model) and graph coloring to construct a reuse pattern of helpers and optimize the helper-user association to minimize the delivery time.
%optimized the worst-case delivery time of all requests. Using basic principles of the multi-round delivery method in~\cite{caire} (which was later proved by~\cite{parrinellomultiantenna} to be optimal for the shared-cache model), they first used graph coloring to construct a reuse pattern of helpers and optimized the helper-user association to minimize the delivery time. Next, they introduced the heuristic `Avalanche' algorithm to leverage the interference-free state of the users as helpers finished their multi-round delivery. 
This work was later extended in~\cite{akcay2023optimal}, where the authors developed a computational method to determine the theoretical throughput region of the users' content delivery rates (defined as the number of chunks delivered per unit of time per user) and solved the fairness scheduling problem by maximizing the desired fairness metric over this throughput region. 
%Two low-complexity heuristic methods were also introduced in~[ISIT], where one maximized the desired fairness metric over a sub-region of the entire throughput region, and the other used a greedy algorithmic approach to fairly associate users with helpers.

Both~\cite{mozhgan},~\cite{akcay2023optimal} consider single-input single-output (SISO) setups only. Given the undoubted importance of multi-antenna communications~\cite{rajatheva2020white}, this paper provides an extension of~\cite{akcay2023optimal} to multi-input single-output (MISO) setups where multi-antenna helpers communicate with single-antenna users. Specifically, we recognize two broad methods to use the additional networking resource provided by the MISO extension. The first method tries to reduce the number of interference links in the network graph, and the second one aims to remove inter-stream interference so that users with similar cache contents can be served simultaneously. \textbf{Until here introduction seems generally fine, we can then here explain the two methods better in  couple of sentences. We may add notation part also if we have space.}
%. In the first method, called \emph{interference cancellation}, we assume that at each helper, appropriate beamformers are used to suppress the transmitted signal at a well-defined subset of users in the transmission range of the helper, enabling these users to be served by other nearby helpers simultaneously. On the other hand, with the other method, called \emph{cache congestion control}, we assume beamformers are designed to remove the inter-stream interference at users with the same cache content (which is a natural result of the cache placement of~\cite{caire}), enabling these users to be served simultaneously in a similar way to the shared-cache model of~\cite{parrinello2019fundamental,parrinello2020extending}. 
While both methods enable serving more users with each transmission, they differ significantly in the underlying concept and resulting performance. In this extended summary, we provide a simplified definition of the system model, the intuition behind each method, and preliminary simulation results comparing them. More detailed explanations are due for the extended version. In the following, by $[L]$, we mean the set of numbers $\{1,\cdots,L\}$.

For the network setup, we consider $H$ multi-antenna helper nodes, each capable of attaining the spatial multiplexing gain of $\alpha$ (the actual number of antennas may be larger), serving the requests of $K$ single-antenna users. 
The transmission and interference radii of all helpers are the same.
%Every helper $h_i$ has a transmission radius of $r_{\textrm{trans}}$ and an interference radius of $r_{\mathrm{inter}} \ge r_{\mathrm{trans}}$, and may be either active or inactive (i.e., not transmitting any signal) at any time interval. 
A user $u_k$ can successfully decode the message transmitted by the active helper $h_i$ if 1) it is within the transmission radius of $h_i$, and 2) it is not within the interference radius of any other active helper $h_{i'}$ unless the interference caused by $h_{i'}$ on $u_k$ is suppressed by beamforming at $h_{i'}$. 
%A graphical representation of the system model is shown in Figure~\ref{fig:network_model}.
%
Like~\cite{akcay2023optimal}, we consider a video streaming application where every video file is split into multiple `chunks' (each representing a few seconds of the video), and every user generates a sequence of requests for the chunks of the video it is streaming. All chunks have the same size, and every user's cache memory can store a portion $\gamma$ of all the chunks. System operation consists of two phases, placement and delivery. 
%During the placement phase, users' cache memories are filled up with subpackets (i.e., smaller portions) of all the video chunks. 
Similar to~\cite{akcay2023optimal}, to keep the subpacketization level low, we use the decentralized cache replication algorithm of~\cite{caire,parrinellomultiantenna} for the placement phase: we fix a number of $L < K$ \emph{cache profiles} and assign each user randomly to one of the profiles. 
%Let us use $\SfL(u_k) \in [L]$ to denote the cache profile assigned to user $u_k$. Given $L$, 
Defining the CC gain as $t = L \gamma$, we divide every video chunk $W$ into $\binom{L}{t}$ non-overlapping equal-sized subpackets $W_{\CS}$, where $\CS$ can be any subset of $[L]$ with $|\CS| = t$, and, if a user $u_k$ is assigned to profile $l$, we store every subpacket $W_{\CS}$, for every chunk $W$ and every $\CS \ni l$, in the cache memory of $u_k$ (clearly, all users assigned to the same profile will cache the same data).
%
%
%
Then, during the delivery phase, after users reveal their requested video chunks, the server creates a number of transmission vectors and transmits them through a selection of active helpers. 
%We assume users can start streaming at arbitrary times, and when they start streaming, they repeatedly generate requests for consecutive video chunks. With this model, we can safely assume a single chunk is requested by at most one user at a given time, as even if two users are streaming the same video, it is unlikely that they have started streaming at the same time. Given the set of user requests and using a delivery algorithm, 
%The server then creates a number of transmission vectors and transmits them through a selection of active helpers. The goal is to serve requested video chunks while optimizing a performance function of, e.g., delivery time, energy, or fairness.
%
With $H$ helpers that can be either active or inactive, there exist $2^H$ selections for the \emph{activation pattern} of the helpers. Let us use vectors $\Bp_j$, $j \in [2^H]$, with binary elements, to denote activation patterns.

%\begin{figure}[t]
    %\begin{subfigure}{0.3\columnwidth}
%        \centering
%        \includegraphics[width = 0.7\columnwidth]{Figs/NetworkModel.png} \label{fig:network_model}
%        \vspace{-1pt}
%    \caption{Example network with $H=2$, $K=5$, $L=3$. Figure from~\cite{akcay2023optimal}.}
%    \vspace{-12pt}
%    \label{fig:network_model}
%\end{figure}

\noindent\textbf{A. SISO setups:}
%
%Every $\Bp_j$ has $H$ binary elements $\Bp_j[i]$, $i \in [H]$, and $\Bp_j[i] = 1$ only if helper $h_i$ is active in the corresponding activation pattern. 
As discussed in~\cite{akcay2023optimal}, the activation pattern uniquely defines the set of users $\CU_i$ that could be served by each active helper $h_i$. 
%Let us use $\CU_i$ to denote the set of users that can be served by helper $h_i$. 
%According to the cache placement strategy, we may have multiple users with the same cache profile (hence, the same cache content). However, 
However, given the cache placement strategy, the codewords can be built only for users in the same $\CU_i$ that are assigned to different cache profiles. So, we may have multiple choices for codeword creation for every active helper $h_i$. Let's call every possible selection of codewords for all active helpers in an activation pattern $\Bp_j$ a \emph{policy} and denote it by $(\pi,\Bp_j)$. Given a policy $(\pi,\Bp_j)$, every user $k$ obtains an instantaneous rate $r_k(\pi,\Bp_j)$. A scheduler chooses a sequence of policies $(\pi,\Bp_j)$, each for a fraction of time $a(\pi,\Bp_j)$, over a sequence of time units. The long-term (time-averaged) throughput of user $k$, measured in delivered video chunks per unit time, is given by $r_{\textrm{avg}}[k] = \sum_{(\pi,\Bp_j)} a(\pi,\Bp_j) r_k(\pi,\Bp_j)$, and the achievable user throughput region $R$ is the convex hull of all instantaneous rates of all users. A canonical fairness scheduling problem consists of finding the scheduling rule (i.e., the fractions of time $a(\pi,\Bp_j)$) that maximizes a suitable component-wise non-decreasing concave function of 
user throughputs over the region $R$~\cite{georgiadis2006resource}. In particular, the so-called proportional fairness criterion~\cite{fairness} considers the network utility function $f(\Br_{\textrm{avg}}) = \sum_k \log(r_{\textrm{avg}}[k])$. The resulting optimization problem is convex: 
\begin{equation}
\label{eq:optimization_problem_main}
    \begin{aligned}
        \max_{a(\pi,\Bp_j)} f(\Br_{\textrm{avg}}) \quad s.t. \quad  a(\pi,\Bp_j)\geq{0}, \: \sum_{(\pi,\Bp_j)} a(\pi,\Bp_j) = 1 . \\
        %& 0 \le a(j,s_j) \le a_{\max}, \quad \forall j\in[2^H], s_j \in [\Sfc(\Bp_j)],
    \end{aligned}
\end{equation}

%Every policy $\pi$ under a given activation pattern $\Bp_j$ uniquely defines an instantaneous $K \times 1$ rate vector $\Br(\pi,\Bp_j)$, where the rate is defined as the number of codewords delivered per unit time per user. A scheduler sequentially chooses policies to continuously serve users, aiming to maximize a component-wise non-decreasing concave fairness function~\cite{fairness} over the fraction of time $a(\pi,\Bp_j)$ of the policy $(\pi,\Bp_j)$. We choose proportional fairness $f(\Br_{\mathrm{avg}})=\sum_{k \in [K]} \log(\Br_{\mathrm{avg}}[k])$ where $\Br_{\mathrm{avg}}[k]$ is the long-term average throughput of user $u_k$. So we have the following convex optimization problem:


%A scheduler uses each policy $\pi$ $a(\pi,\Bp_j)$ fraction of time by maximizing a componentwise nondecreasing fairness function.
%is to optimize the proportional fairness function (or any other member of the $\alpha$-fairness family~\cite{fairness}) over the convex hull of all rate vectors by solving
%\begin{equation}
%\label{eq:optimization_problem_main}
%    \begin{aligned}
%        \max_{a(\pi,\Bp_j)} \Sff &= \sum_{k \in [K]} \log(\Br_{\mathrm{avg}}[k]) \\
%        s.t. \qquad & \Br_{\mathrm{avg}} = \sum_{j \in [2^H]} \sum_{\pi} a(\pi,\Bp_j) \Br(\pi,\Bp_j), \\
%        & a(\pi,\Bp_j)\geq{0}, \quad \sum_{j \in [2^H]} \sum_{\pi} a(\pi,\Bp_j) = 1 . \\
%        %& 0 \le a(j,s_j) \le a_{\max}, \quad \forall j\in[2^H], s_j \in [\Sfc(\Bp_j)],
%    \end{aligned}
%\end{equation}

\begin{exmp}
\label{exmp:siso}
Consider the network in Figure~\ref{fig:network_model}. Assume $t=1$, and consider the activation pattern $\Bp_j = [0,1]$ (i.e., only helper $h_2$ is active). Given the cache configuration in the figure, we have two possible policies, which are to serve either $\{u_4,u_3\}$ or $\{u_4,u_5\}$ (note that $u_2$ is \emph{not} in the transmission radius of $h_2$). Let us consider the policy $(\pi,\Bp_j)$ to serve $\{u_4,u_3\}$, and denote the chunks requested by $u_3$ and $u_4$ as $C$ and $D$, respectively. As $u_3$ and $u_4$ belong to cache groups $2$ and $1$, they have $\{C_2,D_2\}$ and $\{C_1,D_1\}$ in their caches, respectively. As a result, we need to send $C_1 \oplus D_2$, $C_3$, $D_3$ (in 3 time slots) through $h_2$, so that $u_3$ and $u_4$ can decode $\{C_1,C_3\}$ and $\{D_2,D_3\}$, respectively. The rate vector of all users is $\Br(\pi,\Bp_j) = [0,0,\frac{1}{3},\frac{1}{3},0]$ \textbf{Can we leave here like this?, i.e. check for more details?}(check~\cite{akcay2023optimal} for more details). \textbf{Until here generally system model and SISO seems fine.}
\end{exmp}

\begin{figure}[t]
    %\begin{subfigure}{0.3\columnwidth}
        \centering
        \includegraphics[width = 0.6\columnwidth]{Figs/NetworkModel.png} \label{fig:network_model}
        \vspace{-1pt}
    \caption{Example network with $H=2$, $K=5$, $L=3$. Figure from~\cite{akcay2023optimal}.}
    \label{fig:network_model}
    \vspace{-12pt}
\end{figure}

\noindent\textbf{B. MISO setups:} We make the simplifying assumption that \textit{beamforming for interference suppression at any user(s) does not alter the connectivity/interference status of other users in the network}. With this assumption, we consider two transmission strategies for MISO networks:

\noindent\textbf{B.1. Interference nulling: } With this strategy, after selecting the activation pattern, for every active helper $h_i$, we: 1) select a subset of users $\CZ_i$, with $|\CZ_i| < \alpha$, from the set of users that are in the interference radius of $h_i$, and 2) design transmit beamformers at $h_i$ such that the transmitted signal is suppressed at every user in $\CZ_i$ (recall that the spatial multiplexing gain of $\alpha$ is attainable). Then, we repeat the same process as the SISO case, assuming that users in every $\CZ_i$ do not receive any interference from the signal sent by $h_i$. This strategy improves the performance by allowing more users to be served simultaneously.

%\begin{exmp}
%Consider the same network as ...
%\end{exmp}
%A helper may need to serve several users with the same cache profile since $L<K$ and users are randomly assigned to one of $L$ cache profiles. However, users with the same cache profile can not be served with the same codewords when they request distinct files. We call this \textit{cache congestion}. %Our second method helps us to reduce cache congestion by using MISO spatial gain.

\noindent\textbf{B.2. Cache congestion control: } Beyond interference, another throughput limiting factor is the limited number of cache profiles. Since cache profiles are assigned to users randomly and users can move arbitrarily in the network, it may happen that one active helper must serve several users assigned with the same profile. In this case, these users must be served sequentially, and no CC gain is achieved (recall that only users with different cache types can be served by multicasting CC codewords). We refer to this type of impairment as ``cache congestion’’. Our second approach consists of using the MISO spatial multiplexing capability to reduce cache congestion. We define the set of users $\CU_i$ that can be served by active helper $h_i$ similar to the SISO case, but design beamformers at $h_i$ to suppress the inter-stream interference, similar to the shared-cache and dynamic CC models~\cite{parrinellomultiantenna,parrinello2020extending,abolpour2023cache}, to allow users with similar cache contents (i.e., users assigned with the same cache profile) to be served simultaneously.

\vspace{-4pt}
\begin{exmp}
    Consider the same network and activation pattern as Example~\ref{exmp:siso} and let $t=1$. With the cache congestion control strategy, $h_2$ can serve users $\{u_3,u_4,u_5\}$ simultaneously, by transmitting
    \begin{equation*}
        \begin{aligned}
            C_1 \Bw_5 + E_1 \Bw_3 + D_2, \quad C_3 \Bw_5 + E_3 \Bw_3, \quad D_3,
        \end{aligned}
    \end{equation*}
    where the beamformer $\Bw_k$ suppresses data at user $u_k$, and $C,D,E$ denote the files requested by $u_3,u_4,u_5$, respectively. The rate vector for this policy is $\Br(\pi,\Bp_j) = [0,0,\frac{1}{3},\frac{1}{3},\frac{1}{3}]$.
\end{exmp}
\vspace{-3.5pt}

\textbf{Simulation Results start here.}
In Figures~\ref{fig:cdf_l=all}-\ref{fig:cdf_l=6}, we have provided our preliminary simulation results comparing the performance of the proposed methods for SISO and MISO schemes. In the figures, $L=1$ corresponds to the case no CC technique is applied (lower bound), and the `optimum selection' strategy for MISO systems selects the best performance among interference nulling and cache congestion control methods (upper bound). The users are placed in the vicinity of helpers according to a homogeneous Poisson Point Process, and $U$ denotes the average number of users per helper. For all MISO setups, we have set $\alpha = 2$.

As can be seen in Figure~\ref{fig:cdf_l=all}, MISO setups provide much better performance than SISO, which is expected as they benefit from the extra resource provided by multi-antenna transmitters. Moreover, from Figures~\ref{fig:cdf_l=1}-\ref{fig:cdf_l=6}, we see that the cache congestion control method generally outperforms interference nulling. This is because the underlying shared cache model of the cache congestion control method has a larger degree of freedom (DoF), hence enabling more users to be served simultaneously~\cite{parrinellomultiantenna,parrinello2020extending}. However, as the $\frac{U}{L}$ ratio decreases, there is less chance of finding users with the same cache contents, and the performance gap between the two methods narrows. In fact, as can be seen from Figure~\ref{fig:cdf_l=6}, when $L=U$, in some realizations, the interference nulling method provides superior performance. More detailed discussions are due for the extended version of this paper.


\input{Figs-MISO/Plot-Comp}
\input{Figs-MISO/Plot-L1}
\input{Figs-MISO/Plot-L3}
\input{Figs-MISO/Plot-L6}

%\todo[inline]{Revised up to here.}

%We use numerical results to compare the performance of various solutions. We assume $H$ helpers are located at the center of hexagons on a limited hexagonal grid. Every hexagon has a radius of~$1$, and we have $r_{\mathrm{trans}} = 1$ and $r_{\mathrm{inter}}  =1.2$. The users are placed according to a homogeneous Poisson Point Process in the transmission area of helpers. The average number of users per helper, shown by $U$, is determined by the density of the Poisson process. Every user is randomly assigned with a cache profile $l \in [L]$.

%In Figures~\ref{fig:cdf_l=1}, \ref{fig:cdf_l=3} and \ref{fig:cdf_l=6} we have compared the CDF of the achievable rate (in terms of delivered chunks per time) of all users for SISO analytical solver, MISO congestion control, MISO interference cancellation and MISO optimum selection for $L=1$, $L=3$ and $L=6$, respectively where MISO optimum selection uses in the utility maximization (eq. ...) all the rates attained by congestion control and interference cancellation. From the figures we can see that MISO congestion control, interference cancellation and optimum selection outperforms SISO analytical solver for all $L=\{1,3,6\}$. As $L$ increases
%the performance difference between SISO analytical solver and interference cancellation as well as the performance difference between congestion control and optimum selection increases since congestion decreases and interference cancellation can have a more significant effect. 

%In Figure \ref{fig:cdf_l=all} we have compared the CDF of the achievable rate of all users for SISO analytical solver and MISO optimum selection for $L=\{1,3,6\}$. As can be seen from Figure \ref{fig:cdf_l=all} it turns out that optimum selection for $L=3$ outperforms the optimum selection for $L=6$ as opposed to the case where as $L$ increases the performance of SISO analytical solver increases and converges [X]. (We will investigate this further.) OR (We can give intuition why congestion control is worse as we have talked before, in this case congestion control is more effective than interference cancellation so optimal selection is best at L=3 since congestion control is best at L=3, then we should say we investigate why congestion control is better than interference cancellation[We can also give intuition for this  in general as we have talked but it will be vague and tricky I think]) OR (We dont talk about and plot the optimal selection, just plot congestion control and interference cancellation and argue why congestion control is best at L=3). (I am not sure here which one to follow, maybe just the first one since we may not have space and we just say we will investigate this further since these are preliminary results.)



==> Figs-MISO/MISO_Data_April27.tex <==
Rate-L1-A1	CDF-L1-A1	Rate-L1-A2-CC	CDF-L1-A2-CC	Rate-L1-A2-IC	CDF-L1-A2-IC	Rate-L1-A2-OPT	CDF-L1-A2-OPT	Rate-L3-A1	CDF-L3-A1	Rate-L3-A2-CC	CDF-L3-A2-CC	Rate-L3-A2-IC	CDF-L3-A2-IC	Rate-L3-A2-OPT	CDF-L3-A2-OPT	Rate-L6-A1	CDF-L6-A1	Rate-L6-A2-CC	CDF-L6-A2-CC	Rate-L6-A2-IC	CDF-L6-A2-IC	Rate-L6-A2-OPT	CDF-L6-A2-OPT
0.056997857	0	0.099114202	0	0.107142857	0	0.105532656	0	0.076170727	0	0.088203042	0	0.141213846	0	0.101605252	0	0.073753703	0	0.088262528	0	0.122560345	0	0.097427072	0
0.056997857	0.004081633	0.099114202	0.004081633	0.107142857	0.004081633	0.105532656	0.004081633	0.076170727	0.004081633	0.088203042	0.004081633	0.141213846	0.004081633	0.101605252	0.004081633	0.073753703	0.004081633	0.088262528	0.004081633	0.122560345	0.004081633	0.097427072	0.004081633
0.056997857	0.008163265	0.103710311	0.008163265	0.107142857	0.008163265	0.114663207	0.008163265	0.076170727	0.008163265	0.118492682	0.008163265	0.141213846	0.008163265	0.122432912	0.008163265	0.081599504	0.008163265	0.093643052	0.008163265	0.138704178	0.008163265	0.097757176	0.008163265
0.062499946	0.012244898	0.114663248	0.012244898	0.107142857	0.012244898	0.114663207	0.012244898	0.077054557	0.012244898	0.122432902	0.012244898	0.163470086	0.012244898	0.122432914	0.012244898	0.081599505	0.012244898	0.096052626	0.012244898	0.148464126	0.012244898	0.102307695	0.012244898
0.074309532	0.016326531	0.114663248	0.016326531	0.107142857	0.016326531	0.121504949	0.016326531	0.086242991	0.016326531	0.122432902	0.016326531	0.166666568	0.016326531	0.129165554	0.016326531	0.08554146	0.016326531	0.096052627	0.016326531	0.171181531	0.016326531	0.105520307	0.016326531
0.078479622	0.020408163	0.120820746	0.020408163	0.107142857	0.020408163	0.127984522	0.020408163	0.094373737	0.020408163	0.127334121	0.020408163	0.166666666	0.020408163	0.129165564	0.020408163	0.08554146	0.020408163	0.102294042	0.020408163	0.174346444	0.020408163	0.125464737	0.020408163
0.078479622	0.024489796	0.127984621	0.024489796	0.107142857	0.024489796	0.127984525	0.024489796	0.094373737	0.024489796	0.127334123	0.024489796	0.166666666	0.024489796	0.137925633	0.024489796	0.088260465	0.024489796	0.102294042	0.024489796	0.174346444	0.024489796	0.141076699	0.024489796
0.081609063	0.028571429	0.127984623	0.028571429	0.107142857	0.028571429	0.145078119	0.028571429	0.095371184	0.028571429	0.132257535	0.028571429	0.166666666	0.028571429	0.146572445	0.028571429	0.093749736	0.028571429	0.117762246	0.028571429	0.187499214	0.028571429	0.142825951	0.028571429
0.081609063	0.032653061	0.132754321	0.032653061	0.107142857	0.032653061	0.145910098	0.032653061	0.098202234	0.032653061	0.143038625	0.032653061	0.166666666	0.032653061	0.153013969	0.032653061	0.098041983	0.032653061	0.118230716	0.032653061	0.187499897	0.032653061	0.157961469	0.032653061
0.084033593	0.036734694	0.140224087	0.036734694	0.107142857	0.036734694	0.156902458	0.036734694	0.111110707	0.036734694	0.14318132	0.036734694	0.166666666	0.036734694	0.153013969	0.036734694	0.098356015	0.036734694	0.125216121	0.036734694	0.1875	0.036734694	0.161175903	0.036734694
0.095197375	0.040816327	0.156902715	0.040816327	0.107142857	0.040816327	0.156902458	0.040816327	0.111110799	0.040816327	0.146149055	0.040816327	0.166666671	0.040816327	0.16388661	0.040816327	0.098356016	0.040816327	0.134145207	0.040816327	0.1875	0.040816327	0.166395508	0.040816327
0.096773448	0.044897959	0.156902715	0.044897959	0.107142857	0.044897959	0.163504408	0.044897959	0.116315388	0.044897959	0.150840706	0.044897959	0.166666686	0.044897959	0.172305861	0.044897959	0.098356016	0.044897959	0.138485309	0.044897959	0.1875	0.044897959	0.179335958	0.044897959
0.096773448	0.048979592	0.157574906	0.048979592	0.107142857	0.048979592	0.164391024	0.048979592	0.116315394	0.048979592	0.150840706	0.048979592	0.166666686	0.048979592	0.189387211	0.048979592	0.100601711	0.048979592	0.143892098	0.048979592	0.1875	0.048979592	0.179335958	0.048979592
0.099998592	0.053061224	0.163504353	0.053061224	0.107142857	0.053061224	0.168780456	0.057142857	0.117934879	0.053061224	0.157281218	0.053061224	0.166666686	0.053061224	0.193599707	0.053061224	0.101463818	0.053061224	0.143892099	0.053061224	0.1875	0.053061224	0.191054349	0.053061224
0.099998592	0.057142857	0.164391148	0.057142857	0.107142857	0.057142857	0.185205811	0.06122449	0.122943501	0.057142857	0.163886654	0.057142857	0.166666686	0.057142857	0.199999681	0.057142857	0.107142218	0.057142857	0.143892099	0.057142857	0.1875	0.057142857	0.199700619	0.057142857
0.10075819	0.06122449	0.169184335	0.06122449	0.136363636	0.06122449	0.199953326	0.065306122	0.129503126	0.06122449	0.167551223	0.06122449	0.166666686	0.06122449	0.199999709	0.06122449	0.124860538	0.06122449	0.149423917	0.06122449	0.1875	0.06122449	0.202806137	0.06122449
0.10242042	0.065306122	0.169184335	0.065306122	0.136363636	0.069387755	0.199953335	0.069387755	0.140740594	0.065306122	0.175319455	0.065306122	0.176174256	0.065306122	0.214826137	0.065306122	0.126653071	0.065306122	0.157894663	0.065306122	0.1875	0.065306122	0.20293786	0.065306122
0.10242042	0.069387755	0.180113021	0.069387755	0.136363636	0.073469388	0.199998177	0.073469388	0.144659702	0.069387755	0.186697796	0.069387755	0.176174316	0.069387755	0.218134545	0.069387755	0.127678159	0.069387755	0.166666592	0.069387755	0.187500034	0.069387755	0.214893668	0.069387755
0.10242042	0.073469388	0.18187156	0.073469388	0.136363636	0.07755102	0.19999818	0.07755102	0.144659703	0.073469388	0.204640894	0.073469388	0.176174328	0.073469388	0.218134553	0.073469388	0.134398066	0.073469388	0.166666592	0.073469388	0.187500034	0.073469388	0.214894245	0.073469388
0.10242042	0.07755102	0.19822796	0.07755102	0.136363636	0.085714286	0.204739056	0.081632653	0.14552559	0.07755102	0.204640895	0.07755102	0.184700741	0.07755102	0.221383424	0.07755102	0.139396889	0.07755102	0.167603822	0.07755102	0.187500035	0.07755102	0.214894245	0.07755102
0.10242042	0.081632653	0.198227971	0.081632653	0.136363636	0.089795918	0.204739056	0.085714286	0.149538448	0.081632653	0.208317363	0.081632653	0.184700741	0.081632653	0.222221465	0.081632653	0.139396894	0.081632653	0.172702751	0.081632653	0.189888951	0.081632653	0.215585341	0.081632653
0.10242042	0.085714286	0.199998425	0.085714286	0.136363636	0.093877551	0.204739056	0.089795918	0.14953845	0.085714286	0.218134561	0.085714286	0.184700741	0.085714286	0.222221465	0.085714286	0.146583221	0.085714286	0.184188723	0.085714286	0.193270261	0.085714286	0.215585621	0.085714286
0.10242042	0.089795918	0.199998429	0.089795918	0.136363636	0.097959184	0.204739056	0.093877551	0.155539461	0.089795918	0.218134571	0.089795918	0.2	0.089795918	0.225415379	0.089795918	0.148630123	0.089795918	0.192429704	0.089795918	0.196528779	0.089795918	0.219448668	0.089795918
0.10242042	0.093877551	0.204739006	0.093877551	0.136363636	0.102040816	0.204739056	0.097959184	0.157123891	0.093877551	0.222223891	0.093877551	0.2	0.093877551	0.233378803	0.093877551	0.148630123	0.093877551	0.192429705	0.093877551	0.1965309	0.093877551	0.227143775	0.093877551
0.10242042	0.097959184	0.204739006	0.097959184	0.166658132	0.106122449	0.204739056	0.102040816	0.157123891	0.097959184	0.222223891	0.097959184	0.2	0.097959184	0.239249868	0.097959184	0.148630542	0.097959184	0.217553521	0.097959184	0.1965309	0.097959184	0.233938406	0.097959184
0.10242042	0.102040816	0.204739006	0.102040816	0.166658136	0.110204082	0.204739056	0.106122449	0.157123891	0.102040816	0.235052383	0.102040816	0.2	0.102040816	0.239249868	0.102040816	0.148630542	0.102040816	0.219353882	0.106122449	0.200511958	0.102040816	0.247072182	0.102040816
0.10242042	0.106122449	0.204739006	0.106122449	0.166658138	0.114285714	0.204739056	0.110204082	0.157123891	0.106122449	0.235052384	0.106122449	0.2	0.106122449	0.251745805	0.106122449	0.157888062	0.106122449	0.222925607	0.110204082	0.200511958	0.106122449	0.250950292	0.106122449
0.10242042	0.110204082	0.204739006	0.110204082	0.16665814	0.118367347	0.204739056	0.114285714	0.157123891	0.110204082	0.254485793	0.110204082	0.2	0.110204082	0.261097737	0.110204082	0.157888062	0.110204082	0.222925607	0.114285714	0.200511958	0.110204082	0.25115113	0.110204082
0.105262613	0.114285714	0.204739006	0.114285714	0.166658141	0.12244898	0.204739056	0.118367347	0.159357368	0.114285714	0.254485793	0.114285714	0.2	0.114285714	0.263831305	0.114285714	0.162910474	0.114285714	0.222925607	0.118367347	0.200653555	0.114285714	0.251151841	0.114285714
0.113395929	0.118367347	0.204739006	0.118367347	0.166658141	0.126530612	0.204739056	0.12244898	0.159357368	0.118367347	0.259687544	0.118367347	0.2	0.118367347	0.26514491	0.118367347	0.16291117	0.118367347	0.222925607	0.12244898	0.200653555	0.118367347	0.262458632	0.118367347
0.113395963	0.12244898	0.204739006	0.12244898	0.166658142	0.130612245	0.204739056	0.126530612	0.159357368	0.12244898	0.262056824	0.126530612	0.2	0.12244898	0.269393785	0.12244898	0.16291117	0.12244898	0.224762947	0.126530612	0.207838102	0.12244898	0.266082686	0.12244898
0.122018645	0.126530612	0.204739006	0.126530612	0.166658142	0.134693878	0.210687561	0.130612245	0.159357368	0.126530612	0.262056824	0.130612245	0.2	0.126530612	0.269393864	0.126530612	0.16291117	0.126530612	0.250000269	0.130612245	0.207983144	0.126530612	0.266082689	0.126530612
0.122018645	0.130612245	0.204739006	0.130612245	0.166658143	0.13877551	0.213505651	0.134693878	0.159357368	0.130612245	0.262056825	0.134693878	0.226540892	0.130612245	0.27058673	0.130612245	0.166114635	0.130612245	0.25000027	0.134693878	0.209146551	0.130612245	0.266867791	0.130612245
0.122018645	0.134693878	0.204739006	0.134693878	0.16666431	0.142857143	0.215147877	0.13877551	0.160161935	0.134693878	0.266700354	0.13877551	0.226540892	0.134693878	0.272993065	0.134693878	0.166114635	0.134693878	0.254516166	0.13877551	0.209146551	0.134693878	0.266867791	0.134693878
0.122018645	0.13877551	0.204739006	0.13877551	0.166665331	0.146938776	0.21577426	0.142857143	0.160162325	0.13877551	0.29517727	0.142857143	0.228508322	0.13877551	0.284815553	0.13877551	0.166114635	0.13877551	0.254516166	0.142857143	0.209146551	0.13877551	0.266868034	0.13877551
0.122413672	0.142857143	0.206284987	0.142857143	0.166665331	0.151020408	0.218119312	0.146938776	0.160644918	0.142857143	0.29517727	0.146938776	0.22850909	0.142857143	0.284815565	0.142857143	0.166114635	0.142857143	0.254516166	0.146938776	0.216523154	0.142857143	0.266868034	0.142857143
0.122413672	0.146938776	0.241147229	0.146938776	0.166665622	0.155102041	0.228428314	0.151020408	0.160644918	0.146938776	0.29517727	0.151020408	0.23116495	0.146938776	0.29039956	0.146938776	0.167099274	0.146938776	0.254516166	0.151020408	0.216523154	0.146938776	0.270927889	0.146938776
0.124999846	0.151020408	0.245409087	0.151020408	0.166666287	0.159183673	0.22842832	0.155102041	0.165598606	0.151020408	0.29517727	0.159183673	0.23116497	0.151020408	0.293282675	0.151020408	0.167100407	0.151020408	0.268345485	0.155102041	0.216523154	0.151020408	0.270927898	0.151020408
0.1249999	0.155102041	0.245409101	0.155102041	0.166666666	0.163265306	0.235092711	0.159183673	0.165598607	0.155102041	0.299369583	0.163265306	0.23116497	0.155102041	0.295186909	0.155102041	0.167100407	0.155102041	0.283217012	0.159183673	0.239193902	0.155102041	0.28082534	0.155102041
0.127697836	0.159183673	0.245409101	0.159183673	0.166666666	0.167346939	0.239760206	0.163265306	0.169633856	0.159183673	0.299369583	0.167346939	0.23442512	0.159183673	0.295186909	0.159183673	0.167100407	0.159183673	0.29770894	0.163265306	0.239194025	0.159183673	0.286177808	0.159183673
0.127698031	0.163265306	0.245495633	0.163265306	0.166666666	0.171428571	0.241147427	0.167346939	0.174267462	0.163265306	0.310057772	0.171428571	0.249135762	0.163265306	0.295186909	0.163265306	0.171713424	0.163265306	0.299999399	0.167346939	0.249998901	0.163265306	0.286177808	0.163265306
0.127698031	0.167346939	0.245495633	0.167346939	0.166666666	0.175510204	0.245495393	0.171428571	0.176889472	0.167346939	0.315840975	0.179591837	0.249999669	0.167346939	0.295186909	0.167346939	0.172835224	0.167346939	0.299999399	0.171428571	0.249998901	0.167346939	0.286177808	0.167346939
0.127698031	0.171428571	0.245495635	0.171428571	0.166666666	0.179591837	0.245495393	0.175510204	0.179014208	0.171428571	0.315840975	0.183673469	0.24999996	0.171428571	0.295186909	0.171428571	0.172835224	0.171428571	0.299999413	0.175510204	0.249999865	0.171428571	0.286969545	0.171428571
0.127698031	0.175510204	0.245495642	0.175510204	0.166666666	0.183673469	0.245495397	0.179591837	0.180044811	0.175510204	0.315840975	0.187755102	0.24999996	0.175510204	0.299999508	0.175510204	0.172835224	0.175510204	0.299999413	0.179591837	0.249999998	0.175510204	0.286991565	0.175510204
0.127698031	0.179591837	0.249999733	0.179591837	0.166666666	0.187755102	0.245495406	0.183673469	0.180784642	0.179591837	0.315840989	0.191836735	0.24999996	0.179591837	0.301024113	0.179591837	0.174535789	0.179591837	0.299999897	0.183673469	0.249999998	0.179591837	0.293398216	0.179591837
0.127698031	0.183673469	0.249999741	0.183673469	0.166666666	0.191836735	0.260628256	0.187755102	0.180784642	0.183673469	0.316160053	0.195918367	0.24999996	0.183673469	0.320000099	0.183673469	0.174655275	0.183673469	0.300002376	0.187755102	0.249999998	0.183673469	0.29784321	0.183673469
0.127698031	0.187755102	0.249999744	0.187755102	0.166666666	0.195918367	0.260628256	0.191836735	0.180784642	0.187755102	0.317524037	0.2	0.24999998	0.187755102	0.320000099	0.187755102	0.174655275	0.191836735	0.302867144	0.191836735	0.25	0.187755102	0.299999929	0.187755102
0.127698031	0.191836735	0.249999791	0.191836735	0.166666712	0.2	0.260628256	0.195918367	0.181125253	0.191836735	0.317524041	0.204081633	0.24999998	0.191836735	0.320000099	0.191836735	0.176345656	0.195918367	0.315789366	0.195918367	0.25	0.191836735	0.303707317	0.191836735
0.12852461	0.195918367	0.2504043	0.195918367	0.166666712	0.204081633	0.260628256	0.2	0.181125253	0.195918367	0.323781488	0.208163265	0.24999998	0.195918367	0.320000099	0.195918367	0.176345657	0.2	0.31880752	0.2	0.25	0.195918367	0.303708152	0.195918367
0.12852461	0.2	0.250404304	0.2	0.166666712	0.208163265	0.260628256	0.204081633	0.181125253	0.2	0.323781509	0.212244898	0.249999997	0.2	0.320000224	0.2	0.179666892	0.204081633	0.323852979	0.204081633	0.25	0.2	0.303708266	0.2
0.12852461	0.204081633	0.260628236	0.204081633	0.166666712	0.212244898	0.260628256	0.208163265	0.181125253	0.204081633	0.341190976	0.216326531	0.25	0.204081633	0.339820075	0.204081633	0.184899731	0.208163265	0.323852979	0.208163265	0.25	0.204081633	0.309854732	0.204081633
0.12852461	0.208163265	0.260628236	0.208163265	0.166666712	0.216326531	0.260628256	0.212244898	0.181125253	0.208163265	0.341190976	0.220408163	0.25	0.208163265	0.339820075	0.208163265	0.184899732	0.212244898	0.323852979	0.212244898	0.25	0.208163265	0.309854732	0.208163265
0.12852461	0.212244898	0.260628236	0.212244898	0.166666712	0.220408163	0.260628256	0.216326531	0.196922846	0.212244898	0.341190976	0.224489796	0.25	0.212244898	0.339820075	0.212244898	0.184899733	0.216326531	0.323852979	0.216326531	0.250000014	0.212244898	0.309854732	0.212244898
0.12852461	0.216326531	0.260628236	0.216326531	0.166666712	0.224489796	0.260628256	0.220408163	0.196922846	0.216326531	0.37551342	0.228571429	0.25	0.216326531	0.342265643	0.216326531	0.187499834	0.220408163	0.332861979	0.220408163	0.250000068	0.216326531	0.315789398	0.216326531
0.12852461	0.220408163	0.260628236	0.220408163	0.166666712	0.228571429	0.260628256	0.224489796	0.196922846	0.220408163	0.37551342	0.232653061	0.25	0.220408163	0.342265643	0.220408163	0.187499834	0.224489796	0.332861979	0.224489796	0.250000068	0.220408163	0.318069614	0.220408163
0.12852461	0.224489796	0.260628236	0.224489796	0.166667048	0.232653061	0.26627198	0.228571429	0.196922846	0.224489796	0.37551342	0.236734694	0.25	0.224489796	0.342265643	0.224489796	0.187952276	0.228571429	0.339025123	0.228571429	0.25000055	0.224489796	0.319988803	0.224489796
0.12852461	0.228571429	0.260628236	0.228571429	0.166667048	0.236734694	0.26627198	0.232653061	0.202352284	0.228571429	0.37551342	0.240816327	0.25	0.228571429	0.34462805	0.228571429	0.187952276	0.232653061	0.339027593	0.232653061	0.25000055	0.228571429	0.319988803	0.228571429
0.12852461	0.232653061	0.260628236	0.232653061	0.166667048	0.240816327	0.267930931	0.236734694	0.202352303	0.232653061	0.37551342	0.244897959	0.25	0.232653061	0.353761845	0.232653061	0.187952276	0.236734694	0.339027593	0.236734694	0.25000055	0.232653061	0.319988803	0.232653061
0.135922263	0.236734694	0.260628236	0.236734694	0.166667048	0.244897959	0.267930931	0.240816327	0.202352303	0.236734694	0.378717767	0.248979592	0.25	0.236734694	0.36304068	0.236734694	0.18964109	0.240816327	0.339027593	0.240816327	0.25000055	0.236734694	0.321138466	0.236734694
0.135922269	0.240816327	0.260628236	0.240816327	0.166667048	0.248979592	0.267930931	0.244897959	0.202352321	0.240816327	0.380430566	0.253061224	0.25	0.240816327	0.36417676	0.240816327	0.18964109	0.244897959	0.342377011	0.244897959	0.250195705	0.240816327	0.322341079	0.240816327
0.135922297	0.244897959	0.26486001	0.244897959	0.166667048	0.253061224	0.267930931	0.248979592	0.202352321	0.244897959	0.380430566	0.257142857	0.25	0.244897959	0.36417676	0.244897959	0.18964109	0.248979592	0.342377011	0.248979592	0.263157895	0.244897959	0.322341079	0.244897959
0.139246523	0.248979592	0.26486001	0.248979592	0.166667048	0.257142857	0.267930931	0.253061224	0.202352321	0.248979592	0.380430566	0.26122449	0.25	0.248979592	0.36417676	0.248979592	0.194348337	0.253061224	0.342377011	0.257142857	0.263157895	0.248979592	0.324180623	0.248979592
0.139249369	0.253061224	0.26486001	0.253061224	0.166667153	0.26122449	0.267930931	0.257142857	0.20321316	0.253061224	0.382359059	0.265306122	0.25	0.253061224	0.364176788	0.253061224	0.210253268	0.257142857	0.342377011	0.26122449	0.263157895	0.253061224	0.324180624	0.253061224
0.139249418	0.257142857	0.26486001	0.257142857	0.166667153	0.265306122	0.267930931	0.26122449	0.20321316	0.257142857	0.382359059	0.269387755	0.25	0.257142857	0.36417696	0.257142857	0.214001825	0.26122449	0.354702375	0.265306122	0.263159243	0.257142857	0.324180624	0.257142857
0.1392532	0.26122449	0.26486001	0.26122449	0.166667153	0.269387755	0.267930931	0.265306122	0.20321316	0.26122449	0.382359059	0.273469388	0.25	0.26122449	0.375513413	0.26122449	0.218750088	0.265306122	0.354702375	0.269387755	0.267554196	0.26122449	0.324180624	0.26122449
0.142246644	0.265306122	0.26486001	0.265306122	0.166667153	0.273469388	0.273706185	0.269387755	0.203213161	0.265306122	0.38235913	0.27755102	0.25	0.265306122	0.375513413	0.265306122	0.218750088	0.269387755	0.354702375	0.273469388	0.281250393	0.265306122	0.324813364	0.265306122
0.144737088	0.269387755	0.26486001	0.269387755	0.166667153	0.27755102	0.276069727	0.273469388	0.211114949	0.269387755	0.382360588	0.281632653	0.250000001	0.269387755	0.375513413	0.269387755	0.218750088	0.273469388	0.358648008	0.27755102	0.281250393	0.269387755	0.324813364	0.269387755
0.144737088	0.273469388	0.26486001	0.273469388	0.166667153	0.281632653	0.276069754	0.27755102	0.211115197	0.273469388	0.385893086	0.285714286	0.250000001	0.273469388	0.375513413	0.273469388	0.22148618	0.27755102	0.36165638	0.281632653	0.291753038	0.273469388	0.331773671	0.273469388
0.144737088	0.27755102	0.273706021	0.27755102	0.166667153	0.285714286	0.278944117	0.281632653	0.211115197	0.27755102	0.395697177	0.289795918	0.250000001	0.27755102	0.375513413	0.27755102	0.22148618	0.281632653	0.36165638	0.285714286	0.291757616	0.27755102	0.331773671	0.27755102
0.144737088	0.281632653	0.27894431	0.281632653	0.16667519	0.289795918	0.278944117	0.285714286	0.211115197	0.281632653	0.395697177	0.293877551	0.250000054	0.281632653	0.379188468	0.281632653	0.22148618	0.285714286	0.36165638	0.289795918	0.294173101	0.281632653	0.331773673	0.281632653
0.144737088	0.285714286	0.27894431	0.285714286	0.166675191	0.293877551	0.278944117	0.289795918	0.211914636	0.285714286	0.397811885	0.297959184	0.250000054	0.285714286	0.379188468	0.285714286	0.222149108	0.289795918	0.364661695	0.293877551	0.29417335	0.285714286	0.340932973	0.285714286
0.144737088	0.289795918	0.27894431	0.289795918	0.166675191	0.297959184	0.278944117	0.293877551	0.211914636	0.289795918	0.397811885	0.302040816	0.250000055	0.289795918	0.379188472	0.289795918	0.226108705	0.293877551	0.364661695	0.297959184	0.294173387	0.289795918	0.340932978	0.289795918
0.144737088	0.293877551	0.27894431	0.293877551	0.166675193	0.302040816	0.278944117	0.297959184	0.211914636	0.293877551	0.397811885	0.306122449	0.250000087	0.293877551	0.379188487	0.293877551	0.226108705	0.297959184	0.364661695	0.302040816	0.29479529	0.293877551	0.360667814	0.293877551
0.144737088	0.297959184	0.27894431	0.297959184	0.166675194	0.306122449	0.278944117	0.302040816	0.211914636	0.297959184	0.397811886	0.310204082	0.252701363	0.297959184	0.397811889	0.297959184	0.227586506	0.302040816	0.375039841	0.306122449	0.29479529	0.297959184	0.366332274	0.297959184
0.144898658	0.302040816	0.27894431	0.302040816	0.166675195	0.310204082	0.278944117	0.306122449	0.212615388	0.302040816	0.400000806	0.318367347	0.252701363	0.302040816	0.397811889	0.302040816	0.227586506	0.306122449	0.387088903	0.310204082	0.296042342	0.302040816	0.377706167	0.302040816
0.144898658	0.306122449	0.27894431	0.306122449	0.166675197	0.314285714	0.278944117	0.310204082	0.212615388	0.306122449	0.424579647	0.32244898	0.252701363	0.306122449	0.397811889	0.306122449	0.233841167	0.310204082	0.387088903	0.314285714	0.296042347	0.306122449	0.377706595	0.306122449
0.144898658	0.310204082	0.27894431	0.310204082	0.166675197	0.318367347	0.297022664	0.314285714	0.212615388	0.310204082	0.424579647	0.326530612	0.252701381	0.310204082	0.397811889	0.310204082	0.23452649	0.314285714	0.387088903	0.318367347	0.296042347	0.310204082	0.377956575	0.310204082
0.144898658	0.314285714	0.285581758	0.314285714	0.166675198	0.32244898	0.29762808	0.318367347	0.212615388	0.314285714	0.424579647	0.330612245	0.255190727	0.314285714	0.400000062	0.318367347	0.23452649	0.318367347	0.388888939	0.32244898	0.296042363	0.314285714	0.377956575	0.314285714
0.144898658	0.318367347	0.297628009	0.318367347	0.187491339	0.326530612	0.297628082	0.32244898	0.225454544	0.318367347	0.424579647	0.334693878	0.255192076	0.318367347	0.402706752	0.32244898	0.23452649	0.32244898	0.388888939	0.326530612	0.302930676	0.318367347	0.377956575	0.318367347
0.144898658	0.32244898	0.29762801	0.32244898	0.187491339	0.330612245	0.297628082	0.326530612	0.226157204	0.32244898	0.428409318	0.33877551	0.255192076	0.32244898	0.402706752	0.326530612	0.235313914	0.326530612	0.388888939	0.330612245	0.302930676	0.32244898	0.379291154	0.32244898
0.144898658	0.326530612	0.297628011	0.326530612	0.187491343	0.334693878	0.297628082	0.330612245	0.226157204	0.326530612	0.428409348	0.342857143	0.280295219	0.326530612	0.405654965	0.330612245	0.247996861	0.330612245	0.400763684	0.334693878	0.305407463	0.326530612	0.381481254	0.326530612
0.144898658	0.330612245	0.297628011	0.330612245	0.187491347	0.33877551	0.297628082	0.334693878	0.226157204	0.330612245	0.428409348	0.346938776	0.280296937	0.330612245	0.406186272	0.334693878	0.247996861	0.334693878	0.400763688	0.33877551	0.306077587	0.330612245	0.385215265	0.330612245
0.147473798	0.334693878	0.297628011	0.334693878	0.187491349	0.342857143	0.297628082	0.33877551	0.226157204	0.334693878	0.428409348	0.351020408	0.280296937	0.334693878	0.406186272	0.33877551	0.249999825	0.33877551	0.400763688	0.342857143	0.322386923	0.334693878	0.385215265	0.334693878
0.161994512	0.33877551	0.297628011	0.33877551	0.187491354	0.346938776	0.297628083	0.342857143	0.23654602	0.33877551	0.429354151	0.355102041	0.280296937	0.33877551	0.420599871	0.342857143	0.25	0.342857143	0.429076831	0.355102041	0.335811631	0.33877551	0.385215265	0.33877551
0.161994512	0.342857143	0.297628012	0.342857143	0.187491355	0.351020408	0.297628083	0.346938776	0.23654602	0.342857143	0.429354151	0.359183673	0.280297796	0.342857143	0.420599871	0.346938776	0.25	0.346938776	0.447132856	0.375510204	0.338086434	0.342857143	0.410332991	0.342857143
0.161994512	0.346938776	0.297628014	0.346938776	0.187491356	0.355102041	0.300274454	0.351020408	0.238049921	0.346938776	0.429354151	0.363265306	0.280297796	0.346938776	0.420599871	0.351020408	0.25	0.351020408	0.45229106	0.387755102	0.338086475	0.346938776	0.410332991	0.346938776
0.161994512	0.351020408	0.30247053	0.351020408	0.187497349	0.359183673	0.300274456	0.355102041	0.238049921	0.351020408	0.429354151	0.367346939	0.294348093	0.351020408	0.420599871	0.355102041	0.253549379	0.355102041	0.457292829	0.391836735	0.338086475	0.351020408	0.410332991	0.351020408
0.161994512	0.355102041	0.302470531	0.355102041	0.187498925	0.363265306	0.300274457	0.359183673	0.238049921	0.355102041	0.429354151	0.371428571	0.297305012	0.355102041	0.433712042	0.359183673	0.253549379	0.359183673	0.458910438	0.395918367	0.367412074	0.355102041	0.426113673	0.355102041
0.161994512	0.359183673	0.302470637	0.359183673	0.187500621	0.367346939	0.302471326	0.363265306	0.245633641	0.359183673	0.431627126	0.375510204	0.308641802	0.359183673	0.433714347	0.363265306	0.253549379	0.363265306	0.458910438	0.4	0.374924603	0.359183673	0.432528349	0.359183673
0.161994512	0.363265306	0.308537386	0.363265306	0.187500621	0.371428571	0.302471326	0.367346939	0.245633641	0.363265306	0.440753659	0.379591837	0.309417123	0.363265306	0.433714347	0.367346939	0.253549379	0.367346939	0.458910438	0.404081633	0.374924611	0.363265306	0.437654174	0.363265306
0.163933436	0.367346939	0.308537431	0.367346939	0.187500621	0.375510204	0.302471332	0.371428571	0.245633641	0.367346939	0.440753659	0.383673469	0.309417133	0.367346939	0.433714347	0.371428571	0.263157709	0.371428571	0.465901986	0.408163265	0.374999888	0.367346939	0.437654175	0.367346939
0.163933494	0.371428571	0.308537468	0.371428571	0.187500621	0.383673469	0.321862879	0.375510204	0.249999703	0.371428571	0.440753659	0.387755102	0.317303768	0.371428571	0.441699575	0.375510204	0.263924531	0.375510204	0.465901986	0.412244898	0.374999975	0.371428571	0.437654175	0.371428571
0.163933494	0.375510204	0.318404996	0.375510204	0.187500621	0.387755102	0.32186288	0.379591837	0.25	0.375510204	0.440753659	0.391836735	0.323924158	0.375510204	0.44546636	0.379591837	0.263926361	0.379591837	0.465901986	0.416326531	0.374999976	0.375510204	0.447457	0.375510204
0.165598466	0.379591837	0.318406089	0.379591837	0.187508561	0.391836735	0.32186288	0.383673469	0.25	0.379591837	0.443402952	0.395918367	0.323928275	0.379591837	0.44546636	0.383673469	0.280471865	0.383673469	0.487877184	0.432653061	0.374999998	0.379591837	0.453008991	0.379591837
0.165598466	0.383673469	0.318406223	0.383673469	0.187508569	0.395918367	0.32186288	0.387755102	0.25	0.383673469	0.443402952	0.4	0.323928275	0.383673469	0.44546636	0.387755102	0.282550133	0.387755102	0.5	0.436734694	0.374999998	0.383673469	0.463008433	0.383673469
0.165598466	0.387755102	0.318406223	0.387755102	0.187508573	0.4	0.321862881	0.391836735	0.25	0.387755102	0.44546636	0.404081633	0.323928275	0.387755102	0.44546636	0.391836735	0.282550133	0.391836735	0.5	0.440816327	0.374999998	0.387755102	0.463008433	0.387755102
0.165598466	0.391836735	0.318406223	0.391836735	0.18750867	0.404081633	0.321862882	0.395918367	0.25	0.391836735	0.44546636	0.408163265	0.333330799	0.391836735	0.451600073	0.395918367	0.282550134	0.395918367	0.5	0.444897959	0.374999998	0.391836735	0.463030455	0.391836735
0.165598466	0.395918367	0.318406223	0.395918367	0.187508681	0.408163265	0.321862882	0.4	0.25	0.395918367	0.44546636	0.412244898	0.333332768	0.395918367	0.451600073	0.4	0.282550134	0.4	0.506933032	0.46122449	0.374999999	0.395918367	0.470239899	0.395918367
0.165598466	0.4	0.318406223	0.4	0.187508684	0.412244898	0.325340377	0.404081633	0.25	0.4	0.44546636	0.416326531	0.333332793	0.4	0.451600073	0.404081633	0.282550134	0.404081633	0.518569601	0.465306122	0.374999999	0.4	0.470239901	0.4
0.165598466	0.404081633	0.319213126	0.404081633	0.187508685	0.416326531	0.325340377	0.408163265	0.25	0.404081633	0.467086944	0.420408163	0.333333324	0.404081633	0.451600073	0.408163265	0.282550134	0.408163265	0.521561931	0.47755102	0.375	0.404081633	0.470239901	0.404081633
0.16591947	0.408163265	0.319213126	0.408163265	0.187508689	0.420408163	0.325340377	0.412244898	0.250000099	0.408163265	0.467086944	0.424489796	0.333333324	0.408163265	0.461233915	0.412244898	0.296052716	0.412244898	0.52256902	0.481632653	0.375	0.408163265	0.474848558	0.408163265
0.165919476	0.412244898	0.319213126	0.412244898	0.199999793	0.424489796	0.325340377	0.416326531	0.250000099	0.412244898	0.467086944	0.428571429	0.333333324	0.412244898	0.461233915	0.416326531	0.296052716	0.416326531	0.52256902	0.485714286	0.375	0.412244898	0.474848558	0.412244898
0.167738534	0.416326531	0.319213126	0.416326531	0.199999793	0.428571429	0.325340377	0.420408163	0.250000099	0.416326531	0.476139581	0.432653061	0.333333333	0.416326531	0.461233915	0.420408163	0.297260665	0.420408163	0.526315506	0.493877551	0.375	0.416326531	0.474848558	0.416326531
0.167738534	0.420408163	0.319213126	0.420408163	0.199999793	0.432653061	0.325340377	0.424489796	0.252029271	0.420408163	0.487755403	0.436734694	0.333333333	0.420408163	0.476789616	0.424489796	0.297260665	0.424489796	0.526315506	0.502040816	0.375	0.424489796	0.499220194	0.420408163
0.167738534	0.424489796	0.319213126	0.424489796	0.199999793	0.436734694	0.325340377	0.428571429	0.252029271	0.424489796	0.487755403	0.440816327	0.333333333	0.424489796	0.476789616	0.428571429	0.297782588	0.428571429	0.527074393	0.510204082	0.375	0.432653061	0.49959936	0.424489796
0.167738534	0.428571429	0.319213126	0.428571429	0.199999793	0.440816327	0.32875094	0.432653061	0.252029271	0.428571429	0.487755403	0.444897959	0.333333333	0.428571429	0.476789616	0.432653061	0.297782589	0.432653061	0.527074393	0.534693878	0.375	0.436734694	0.49959936	0.428571429
0.167738534	0.432653061	0.321862776	0.432653061	0.199999793	0.444897959	0.32875094	0.436734694	0.259259498	0.432653061	0.491962117	0.448979592	0.333333333	0.432653061	0.484830053	0.436734694	0.30257564	0.436734694	0.537432839	0.53877551	0.375	0.440816327	0.499599361	0.432653061
0.169423036	0.436734694	0.321862777	0.436734694	0.199999793	0.448979592	0.32875094	0.440816327	0.259259498	0.436734694	0.491962117	0.453061224	0.333333333	0.436734694	0.48787918	0.440816327	0.31095734	0.440816327	0.538892516	0.542857143	0.375	0.444897959	0.499599361	0.436734694
0.169423036	0.440816327	0.321862778	0.440816327	0.199999793	0.453061224	0.32875094	0.444897959	0.259259498	0.440816327	0.491962117	0.457142857	0.333333333	0.440816327	0.48787918	0.444897959	0.312500109	0.444897959	0.538892516	0.546938776	0.375	0.448979592	0.500664292	0.440816327
0.169423038	0.444897959	0.321862785	0.444897959	0.199999793	0.457142857	0.32875094	0.448979592	0.263099076	0.444897959	0.5	0.46122449	0.333333333	0.444897959	0.48787918	0.448979592	0.312500109	0.448979592	0.538892516	0.551020408	0.375	0.453061224	0.500664297	0.444897959
0.169423038	0.448979592	0.32186279	0.448979592	0.199999793	0.46122449	0.328750941	0.453061224	0.263099077	0.448979592	0.5	0.465306122	0.333333333	0.448979592	0.499999997	0.453061224	0.317585638	0.453061224	0.538892516	0.555102041	0.375	0.457142857	0.501626658	0.448979592
0.177871981	0.453061224	0.321862791	0.453061224	0.199999793	0.465306122	0.328750942	0.457142857	0.263099085	0.453061224	0.5	0.469387755	0.333333333	0.453061224	0.499999997	0.457142857	0.317585638	0.457142857	0.543883276	0.563265306	0.375	0.46122449	0.523306461	0.453061224
0.180374669	0.457142857	0.321862792	0.457142857	0.199999793	0.469387755	0.328750942	0.46122449	0.265595612	0.457142857	0.5	0.473469388	0.333333333	0.457142857	0.499999997	0.46122449	0.317585638	0.46122449	0.562500128	0.575510204	0.375	0.465306122	0.523306461	0.457142857
0.180374669	0.46122449	0.34955718	0.46122449	0.199999793	0.473469388	0.328750942	0.465306122	0.265595612	0.46122449	0.5	0.481632653	0.333333333	0.46122449	0.499999997	0.465306122	0.317585638	0.469387755	0.56719178	0.591836735	0.375	0.469387755	0.523306461	0.46122449
0.180374669	0.465306122	0.349557221	0.465306122	0.199999793	0.47755102	0.328750942	0.469387755	0.265595612	0.465306122	0.5	0.485714286	0.333333333	0.465306122	0.499999998	0.469387755	0.321428891	0.473469388	0.583333408	0.608163265	0.375	0.473469388	0.523306461	0.465306122
0.180374669	0.469387755	0.349557221	0.469387755	0.200002896	0.481632653	0.328750942	0.473469388	0.265595613	0.469387755	0.5	0.489795918	0.333333333	0.469387755	0.499999998	0.473469388	0.321428891	0.47755102	0.60000007	0.624489796	0.375	0.47755102	0.532642085	0.469387755
0.180374669	0.473469388	0.349557221	0.473469388	0.214283247	0.485714286	0.328750942	0.47755102	0.265595613	0.473469388	0.518517406	0.493877551	0.333333333	0.473469388	0.499999998	0.47755102	0.321428891	0.481632653	0.600576084	0.628571429	0.375	0.481632653	0.533735825	0.473469388
0.180374669	0.47755102	0.349557221	0.47755102	0.214284435	0.489795918	0.32875131	0.481632653	0.265595613	0.47755102	0.518517406	0.497959184	0.333333333	0.47755102	0.499999998	0.481632653	0.321428891	0.485714286	0.602649022	0.644897959	0.375000173	0.485714286	0.533735825	0.47755102
0.185714688	0.481632653	0.349557221	0.481632653	0.214285896	0.493877551	0.343767311	0.485714286	0.274275578	0.481632653	0.518517406	0.502040816	0.333333333	0.481632653	0.518519024	0.485714286	0.328125131	0.489795918	0.603999612	0.648979592	0.375075389	0.489795918	0.54892654	0.481632653
0.185714688	0.485714286	0.35443695	0.485714286	0.21428661	0.497959184	0.343767313	0.489795918	0.274275578	0.485714286	0.531683858	0.506122449	0.333333333	0.485714286	0.518519024	0.489795918	0.328125131	0.493877551	0.606107901	0.657142857	0.375075393	0.493877551	0.548926542	0.485714286
0.185714688	0.489795918	0.354436962	0.489795918	0.21428661	0.502040816	0.343767313	0.493877551	0.274584895	0.489795918	0.531683858	0.510204082	0.333333333	0.489795918	0.518519024	0.493877551	0.328806849	0.497959184	0.614133966	0.669387755	0.376518552	0.497959184	0.551361049	0.489795918
0.185714688	0.493877551	0.358891345	0.497959184	0.21428661	0.506122449	0.354437254	0.497959184	0.274584895	0.493877551	0.553144175	0.514285714	0.333333333	0.493877551	0.518601981	0.497959184	0.331883151	0.502040816	0.619354792	0.67755102	0.376518552	0.502040816	0.552052753	0.493877551
0.185714688	0.497959184	0.358891347	0.502040816	0.21428661	0.510204082	0.354437261	0.502040816	0.276788714	0.497959184	0.553144175	0.518367347	0.333333333	0.497959184	0.533333393	0.502040816	0.33222927	0.506122449	0.632905392	0.697959184	0.376518552	0.506122449	0.552052753	0.497959184
0.185714688	0.502040816	0.35889135	0.506122449	0.249996377	0.514285714	0.371429091	0.506122449	0.276788714	0.502040816	0.553144175	0.52244898	0.333333683	0.502040816	0.533333393	0.506122449	0.33222927	0.510204082	0.647705957	0.710204082	0.376518552	0.510204082	0.562500089	0.502040816
0.185714688	0.506122449	0.35889135	0.510204082	0.249997342	0.518367347	0.371429091	0.510204082	0.276788714	0.506122449	0.558141263	0.526530612	0.333333684	0.506122449	0.533333822	0.510204082	0.33222927	0.514285714	0.648212002	0.714285714	0.377461651	0.514285714	0.562500089	0.506122449
0.186778009	0.510204082	0.364141776	0.514285714	0.249997342	0.52244898	0.371429091	0.514285714	0.281727961	0.510204082	0.55814135	0.530612245	0.3333337	0.510204082	0.535123134	0.514285714	0.33222927	0.518367347	0.649827103	0.730612245	0.377461897	0.518367347	0.562500091	0.510204082
0.186778009	0.514285714	0.364141776	0.518367347	0.249997381	0.526530612	0.371429091	0.518367347	0.281727961	0.514285714	0.55814135	0.534693878	0.3333337	0.514285714	0.535123134	0.518367347	0.334200248	0.52244898	0.653947373	0.746938776	0.387857483	0.52244898	0.57599354	0.514285714
0.186778009	0.518367347	0.364141776	0.52244898	0.249997381	0.530612245	0.371429091	0.52244898	0.285850235	0.518367347	0.574493092	0.53877551	0.333333965	0.518367347	0.542568988	0.52244898	0.334200248	0.526530612	0.664068408	0.755102041	0.388898493	0.526530612	0.583604494	0.518367347
0.186778009	0.52244898	0.364141776	0.526530612	0.249998511	0.534693878	0.371429091	0.526530612	0.285850237	0.52244898	0.574493092	0.542857143	0.3333346	0.52244898	0.553144172	0.526530612	0.334414473	0.530612245	0.664937861	0.759183673	0.394736842	0.530612245	0.5935667	0.526530612
0.186778009	0.526530612	0.364141776	0.530612245	0.249999171	0.53877551	0.371429091	0.530612245	0.285850238	0.526530612	0.579314391	0.546938776	0.3333346	0.526530612	0.553144173	0.530612245	0.334414473	0.534693878	0.666150599	0.771428571	0.394736842	0.534693878	0.60350668	0.53877551
0.19904689	0.530612245	0.364141776	0.534693878	0.249999171	0.542857143	0.375956952	0.534693878	0.285850238	0.530612245	0.579314391	0.551020408	0.345679099	0.530612245	0.553144173	0.534693878	0.347620166	0.53877551	0.673191237	0.779591837	0.394736842	0.53877551	0.615499486	0.542857143
0.19904689	0.534693878	0.37142902	0.53877551	0.249999171	0.546938776	0.375956952	0.53877551	0.285850238	0.534693878	0.579314391	0.555102041	0.345679099	0.534693878	0.57172813	0.53877551	0.351789735	0.542857143	0.688365657	0.791836735	0.394736842	0.542857143	0.615499486	0.546938776
0.19904689	0.53877551	0.37142902	0.542857143	0.249999171	0.551020408	0.375956952	0.542857143	0.292323319	0.53877551	0.581777251	0.559183673	0.351347493	0.53877551	0.57172813	0.542857143	0.351789735	0.546938776	0.698852978	0.795918367	0.403921264	0.546938776	0.623983337	0.551020408
0.19904689	0.542857143	0.37142902	0.546938776	0.249999579	0.555102041	0.375956952	0.546938776	0.292323319	0.542857143	0.581777251	0.563265306	0.351347493	0.542857143	0.57172813	0.546938776	0.361425586	0.551020408	0.698852978	0.8	0.438913403	0.551020408	0.628553436	0.559183673
0.19904689	0.546938776	0.37142902	0.551020408	0.249999872	0.559183673	0.375956952	0.551020408	0.292370412	0.546938776	0.581777251	0.567346939	0.36602535	0.546938776	0.580556294	0.551020408	0.361432635	0.555102041	0.721621562	0.808163265	0.443922412	0.555102041	0.632640704	0.563265306
0.214245081	0.551020408	0.37142902	0.555102041	0.249999928	0.563265306	0.375956952	0.555102041	0.292924338	0.551020408	0.585044732	0.571428571	0.375432259	0.551020408	0.580556294	0.555102041	0.365117331	0.559183673	0.738515053	0.812244898	0.448469578	0.559183673	0.632640704	0.567346939
0.214245115	0.555102041	0.37142902	0.559183673	0.25	0.567346939	0.384704706	0.559183673	0.292924338	0.555102041	0.585044732	0.575510204	0.375432339	0.555102041	0.580556294	0.559183673	0.365121421	0.563265306	0.75	0.828571429	0.46875	0.563265306	0.643652901	0.571428571
0.214245115	0.559183673	0.37142902	0.563265306	0.25	0.571428571	0.384704706	0.563265306	0.294561535	0.559183673	0.585044732	0.579591837	0.383588367	0.559183673	0.585044721	0.563265306	0.375	0.567346939	0.75	0.844897959	0.46875	0.567346939	0.647157619	0.575510204
0.214245115	0.563265306	0.394118867	0.567346939	0.25	0.575510204	0.386713582	0.567346939	0.294561535	0.563265306	0.585044732	0.583673469	0.383588367	0.563265306	0.585044721	0.567346939	0.375	0.571428571	0.75	0.869387755	0.46875	0.571428571	0.647772675	0.579591837
0.214245115	0.567346939	0.394121995	0.571428571	0.25	0.579591837	0.386713582	0.571428571	0.294561535	0.567346939	0.585044732	0.587755102	0.385743183	0.567346939	0.585044721	0.571428571	0.375	0.575510204	0.75	0.910204082	0.46875	0.575510204	0.648361247	0.583673469
0.214245115	0.571428571	0.394122382	0.575510204	0.25	0.583673469	0.386713582	0.575510204	0.299911937	0.571428571	0.585044732	0.591836735	0.385745839	0.571428571	0.585044721	0.575510204	0.375	0.579591837	0.75	0.930612245	0.46875	0.579591837	0.648361247	0.587755102
0.214529291	0.575510204	0.394122382	0.579591837	0.25	0.587755102	0.386713582	0.579591837	0.300002592	0.575510204	0.589216851	0.595918367	0.385745839	0.575510204	0.585044721	0.579591837	0.375	0.583673469	0.769818491	0.942857143	0.46875	0.583673469	0.650132616	0.591836735
0.214529344	0.579591837	0.394122382	0.583673469	0.25	0.591836735	0.386713582	0.583673469	0.300002592	0.579591837	0.589216851	0.6	0.385747727	0.579591837	0.585044721	0.583673469	0.375	0.587755102	0.789473684	0.955102041	0.46875	0.587755102	0.650132616	0.595918367
0.216667136	0.583673469	0.394122382	0.587755102	0.25	0.595918367	0.394120742	0.587755102	0.301875421	0.583673469	0.599999194	0.612244898	0.386729554	0.583673469	0.589764154	0.587755102	0.375	0.595918367	0.789473684	0.967346939	0.46875	0.591836735	0.652599696	0.6
0.216667136	0.587755102	0.394122382	0.591836735	0.25	0.604081633	0.394121105	0.591836735	0.301875421	0.587755102	0.610003469	0.616326531	0.386729554	0.587755102	0.589764154	0.591836735	0.38126767	0.6	0.886327713	0.983673469	0.46875	0.595918367	0.652599698	0.604081633
0.216667136	0.591836735	0.406362596	0.595918367	0.25	0.608163265	0.394122145	0.595918367	0.301875421	0.591836735	0.610003469	0.620408163	0.386729554	0.591836735	0.594014576	0.595918367	0.405873931	0.604081633	0.9375	1	0.46875	0.6	0.66033493	0.612244898
0.216667136	0.595918367	0.406362596	0.6	0.25	0.612244898	0.394122145	0.6	0.301875421	0.595918367	0.618933212	0.624489796	0.386729554	0.595918367	0.599999937	0.6	0.405873931	0.608163265	0.9375	1	0.48796707	0.604081633	0.66071975	0.616326531
0.216667136	0.6	0.406362596	0.604081633	0.250000023	0.616326531	0.394122145	0.604081633	0.301875421	0.6	0.618942734	0.628571429	0.414666565	0.6	0.599999937	0.604081633	0.429808907	0.612244898	0.9375	1	0.487980484	0.608163265	0.660735077	0.620408163
0.216667136	0.604081633	0.406362596	0.608163265	0.250000025	0.620408163	0.394122145	0.608163265	0.301875421	0.604081633	0.618942734	0.632653061	0.421863313	0.604081633	0.599999943	0.608163265	0.429808907	0.616326531	0.9375	1	0.499998719	0.612244898	0.68250373	0.632653061
0.220127416	0.608163265	0.406362596	0.612244898	0.250000025	0.624489796	0.394122145	0.612244898	0.308988021	0.608163265	0.649210049	0.640816327	0.424658187	0.608163265	0.608126553	0.612244898	0.440681594	0.620408163	0.9375	1	0.499999981	0.616326531	0.68390407	0.640816327
0.220127471	0.612244898	0.433333857	0.616326531	0.250000025	0.632653061	0.43333394	0.616326531	0.333333072	0.612244898	0.666666667	0.644897959	0.424658492	0.612244898	0.608126553	0.616326531	0.440681594	0.624489796	0.9375	1	0.499999984	0.620408163	0.684745813	0.644897959
0.220128536	0.616326531	0.433333857	0.620408163	0.250000025	0.636734694	0.43333394	0.620408163	0.333333333	0.616326531	0.666666667	0.648979592	0.424658492	0.616326531	0.634295335	0.620408163	0.440681594	0.628571429	0.9375	1	0.503189314	0.624489796	0.690922672	0.653061224
0.220128536	0.620408163	0.433333857	0.624489796	0.250000032	0.640816327	0.43333394	0.624489796	0.333333333	0.620408163	0.666666667	0.653061224	0.44417405	0.620408163	0.634295335	0.624489796	0.440681594	0.632653061	0.9375	1	0.512314077	0.628571429	0.693001396	0.657142857
0.220128536	0.624489796	0.433333857	0.628571429	0.250000032	0.644897959	0.43333394	0.628571429	0.333333333	0.624489796	0.666666667	0.657142857	0.44417405	0.624489796	0.635253884	0.628571429	0.450847533	0.636734694	0.9375	1	0.526314441	0.632653061	0.696946838	0.66122449
0.220128536	0.628571429	0.433333857	0.632653061	0.250000032	0.648979592	0.43333394	0.632653061	0.333333333	0.628571429	0.666666667	0.66122449	0.452049657	0.628571429	0.642629042	0.632653061	0.452217412	0.648979592	0.9375	1	0.532285801	0.636734694	0.703108558	0.665306122
0.226113671	0.632653061	0.433333857	0.636734694	0.250000032	0.653061224	0.43333394	0.636734694	0.333333333	0.632653061	0.666666667	0.665306122	0.456932984	0.632653061	0.649609425	0.636734694	0.455173012	0.653061224	0.9375	1	0.533578736	0.640816327	0.703108558	0.669387755
0.226113671	0.636734694	0.45733846	0.640816327	0.250000084	0.657142857	0.456102277	0.640816327	0.333333333	0.636734694	0.676218491	0.67755102	0.499970921	0.636734694	0.655371948	0.640816327	0.46875	0.657142857	0.9375	1	0.556729739	0.644897959	0.703108558	0.673469388
0.226113671	0.640816327	0.45733846	0.644897959	0.250000084	0.66122449	0.456102277	0.644897959	0.333333464	0.640816327	0.683839946	0.681632653	0.499970921	0.640816327	0.666666663	0.644897959	0.46875	0.66122449	0.9375	1	0.562500786	0.648979592	0.703108558	0.67755102
0.226113671	0.644897959	0.45733846	0.648979592	0.250000084	0.665306122	0.456102277	0.648979592	0.333333464	0.644897959	0.683839947	0.685714286	0.49999601	0.644897959	0.666666663	0.648979592	0.46875	0.665306122	0.9375	1	0.567690211	0.653061224	0.705164556	0.681632653
0.230768398	0.648979592	0.45733846	0.653061224	0.250000084	0.669387755	0.456102277	0.653061224	0.340235723	0.648979592	0.689942227	0.693877551	0.499999723	0.648979592	0.666666663	0.653061224	0.46875	0.669387755	0.9375	1	0.589590579	0.657142857	0.705164556	0.685714286
0.230768405	0.653061224	0.45733846	0.657142857	0.250000084	0.673469388	0.457338493	0.657142857	0.340235723	0.653061224	0.714199952	0.697959184	0.499999985	0.653061224	0.666666664	0.657142857	0.483500763	0.673469388	0.9375	1	0.605861367	0.669387755	0.705164556	0.689795918
0.233871092	0.657142857	0.45733846	0.66122449	0.250000298	0.67755102	0.457338493	0.66122449	0.340235723	0.657142857	0.718083118	0.702040816	0.499999985	0.657142857	0.666666664	0.66122449	0.497838646	0.67755102	0.9375	1	0.60587636	0.673469388	0.705164556	0.693877551
0.233871092	0.66122449	0.468367733	0.665306122	0.250000298	0.681632653	0.457338493	0.665306122	0.340235723	0.66122449	0.722745297	0.706122449	0.499999994	0.66122449	0.666666664	0.665306122	0.515156314	0.693877551	0.9375	1	0.615113077	0.67755102	0.705164556	0.697959184
0.233871092	0.665306122	0.468367733	0.669387755	0.250000298	0.685714286	0.457338493	0.669387755	0.362807304	0.665306122	0.722745297	0.710204082	0.499999997	0.665306122	0.675612902	0.669387755	0.523965822	0.706122449	0.9375	1	0.656452722	0.681632653	0.705164556	0.702040816
0.233871092	0.669387755	0.468367733	0.673469388	0.250000298	0.689795918	0.457338493	0.673469388	0.362807304	0.669387755	0.740312493	0.718367347	0.499999997	0.669387755	0.688099592	0.673469388	0.526315975	0.710204082	0.9375	1	0.737851583	0.685714286	0.705359849	0.706122449
0.233871092	0.673469388	0.468367733	0.67755102	0.250000298	0.693877551	0.457338493	0.67755102	0.371661683	0.673469388	0.741637465	0.72244898	0.499999999	0.673469388	0.688099592	0.67755102	0.52785089	0.714285714	0.9375	1	0.749999855	0.689795918	0.705359852	0.710204082
0.233871092	0.67755102	0.478624362	0.681632653	0.250000725	0.697959184	0.48207197	0.681632653	0.375266172	0.67755102	0.741637465	0.726530612	0.499999999	0.67755102	0.702992695	0.681632653	0.528509883	0.718367347	0.9375	1	0.749999913	0.693877551	0.710356225	0.714285714
0.236840687	0.681632653	0.478624362	0.685714286	0.250000725	0.702040816	0.48207197	0.685714286	0.375266172	0.681632653	0.741637465	0.730612245	0.5	0.681632653	0.702992695	0.685714286	0.533788166	0.72244898	0.9375	1	0.749999979	0.710204082	0.710356227	0.718367347
0.236840687	0.685714286	0.478624362	0.689795918	0.250000725	0.706122449	0.48207197	0.689795918	0.38172699	0.685714286	0.741637465	0.734693878	0.5	0.685714286	0.726835388	0.689795918	0.535998175	0.726530612	0.9375	1	0.749999996	0.714285714	0.712272837	0.72244898
0.236840687	0.689795918	0.478624362	0.693877551	0.250000725	0.710204082	0.48207197	0.693877551	0.38172699	0.689795918	0.744245732	0.742857143	0.5	0.689795918	0.734855088	0.693877551	0.54189379	0.730612245	0.9375	1	0.749999998	0.72244898	0.712272837	0.726530612
0.238362884	0.693877551	0.480497817	0.697959184	0.250000725	0.714285714	0.485513439	0.697959184	0.388889247	0.693877551	0.745514207	0.759183673	0.5	0.693877551	0.736168695	0.702040816	0.562500166	0.734693878	0.9375	1	0.749999999	0.734693878	0.746407207	0.730612245
0.238367749	0.697959184	0.480497817	0.702040816	0.250001171	0.718367347	0.485513439	0.702040816	0.388889247	0.697959184	0.764947616	0.763265306	0.5	0.697959184	0.742666949	0.706122449	0.562500166	0.73877551	0.9375	1	0.749999999	0.751020408	0.749999978	0.734693878
0.238367749	0.702040816	0.480497817	0.706122449	0.250001329	0.72244898	0.485513439	0.706122449	0.388889247	0.702040816	0.777776109	0.779591837	0.5	0.702040816	0.742666949	0.710204082	0.565100267	0.742857143	0.9375	1	0.749999999	0.759183673	0.749999978	0.73877551
0.238367749	0.706122449	0.480497817	0.710204082	0.250001329	0.726530612	0.485513439	0.710204082	0.388889247	0.706122449	0.781865415	0.791836735	0.5	0.706122449	0.751209507	0.714285714	0.565100268	0.746938776	0.9375	1	0.75	0.767346939	0.74999998	0.742857143
0.238367749	0.710204082	0.483503764	0.714285714	0.250001329	0.730612245	0.490504176	0.714285714	0.392820904	0.710204082	0.781865415	0.795918367	0.5	0.714285714	0.751209507	0.718367347	0.583635607	0.755102041	0.9375	1	0.75	0.787755102	0.749999996	0.759183673
0.253420033	0.714285714	0.483503764	0.718367347	0.250001329	0.734693878	0.490504176	0.718367347	0.392820906	0.714285714	0.822241822	0.8	0.5	0.718367347	0.751209507	0.72244898	0.592105433	0.763265306	0.9375	1	0.75	0.791836735	0.749999999	0.775510204
0.253420033	0.718367347	0.483503764	0.72244898	0.250001356	0.73877551	0.490504176	0.72244898	0.399994817	0.72244898	0.822241822	0.804081633	0.5	0.72244898	0.751209507	0.726530612	0.59452133	0.767346939	0.9375	1	0.75	0.808163265	0.749999999	0.791836735
0.253420033	0.72244898	0.483503764	0.726530612	0.250001356	0.742857143	0.490504176	0.726530612	0.409977595	0.726530612	0.824680545	0.812244898	0.5	0.726530612	0.766703613	0.730612245	0.607541869	0.775510204	0.9375	1	0.75	0.832653061	0.75	0.8
0.253420033	0.726530612	0.495632518	0.730612245	0.250001356	0.746938776	0.495630764	0.730612245	0.409977595	0.730612245	0.836113346	0.824489796	0.5	0.730612245	0.766703613	0.734693878	0.61757295	0.791836735	0.9375	1	0.75	0.853061224	0.75	0.812244898
0.25384632	0.730612245	0.501152956	0.734693878	0.250001658	0.751020408	0.519344199	0.734693878	0.417200697	0.734693878	0.849159294	0.828571429	0.5	0.734693878	0.777778536	0.742857143	0.625000219	0.795918367	0.9375	1	0.75	0.889795918	0.75	0.828571429
0.25384632	0.734693878	0.501152956	0.73877551	0.250001658	0.755102041	0.519344199	0.73877551	0.417200697	0.73877551	0.868893926	0.832653061	0.5	0.73877551	0.777778536	0.746938776	0.629679582	0.812244898	0.9375	1	0.75	0.897959184	0.75	0.844897959
0.25384632	0.73877551	0.501152956	0.742857143	0.299997172	0.759183673	0.519344199	0.742857143	0.425230773	0.742857143	0.868893926	0.836734694	0.5	0.742857143	0.777778536	0.751020408	0.631382488	0.828571429	0.9375	1	0.750000012	0.906122449	0.75	0.853061224
0.25384632	0.742857143	0.501152956	0.746938776	0.299999921	0.763265306	0.519344199	0.746938776	0.425230773	0.746938776	0.870156209	0.840816327	0.5	0.746938776	0.781238042	0.755102041	0.642857783	0.836734694	0.9375	1	0.750639378	0.910204082	0.75	0.86122449
0.25384632	0.746938776	0.52911261	0.751020408	0.299999921	0.767346939	0.529112549	0.751020408	0.425230773	0.751020408	0.870156209	0.844897959	0.5	0.751020408	0.781865433	0.763265306	0.643357608	0.840816327	0.9375	1	0.753037073	0.914285714	0.75	0.865306122
0.266918202	0.751020408	0.52911261	0.755102041	0.3	0.771428571	0.529112549	0.755102041	0.425230773	0.755102041	0.872665879	0.869387755	0.5	0.755102041	0.781865433	0.767346939	0.651643983	0.848979592	0.9375	1	0.773399608	0.92244898	0.75	0.889795918
0.266918202	0.755102041	0.52911261	0.759183673	0.3	0.775510204	0.529112549	0.759183673	0.44103256	0.759183673	0.881507318	0.873469388	0.5	0.759183673	0.781865433	0.771428571	0.653044483	0.853061224	0.9375	1	0.773467489	0.934693878	0.75	0.902040816
0.266918202	0.759183673	0.52911261	0.763265306	0.3	0.779591837	0.529112549	0.763265306	0.44103256	0.763265306	0.885031515	0.87755102	0.5	0.763265306	0.796482008	0.775510204	0.656250263	0.86122449	0.9375	1	0.788273638	0.93877551	0.757660989	0.914285714
0.266918202	0.763265306	0.52911261	0.767346939	0.3	0.783673469	0.529112549	0.767346939	0.441842306	0.767346939	0.895145854	0.893877551	0.5	0.767346939	0.800000304	0.779591837	0.66445854	0.865306122	0.9375	1	0.789473684	0.946938776	0.762210278	0.918367347
0.276899682	0.767346939	0.595256023	0.771428571	0.3	0.787755102	0.595256165	0.771428571	0.441842306	0.771428571	0.945073318	0.897959184	0.5	0.771428571	0.800000319	0.787755102	0.667279287	0.869387755	0.9375	1	0.789473684	0.959183673	0.775744451	0.92244898
0.276899682	0.771428571	0.595256024	0.775510204	0.3	0.791836735	0.595256166	0.775510204	0.441842306	0.775510204	0.945073318	0.902040816	0.5	0.775510204	0.800000332	0.791836735	0.668400495	0.873469388	0.9375	1	0.789473684	0.967346939	0.786676842	0.930612245
0.276899682	0.775510204	0.595256024	0.779591837	0.3	0.795918367	0.595256166	0.779591837	0.441842306	0.779591837	0.952180446	0.914285714	0.5	0.779591837	0.803025367	0.795918367	0.668400495	0.881632653	0.9375	1	0.789473684	0.971428571	0.789473683	0.934693878
0.276899682	0.779591837	0.595256025	0.783673469	0.3	0.8	0.595256167	0.783673469	0.441842306	0.783673469	0.999999962	0.92244898	0.5	0.783673469	0.803025367	0.8	0.668828946	0.889795918	0.9375	1	0.856072065	0.975510204	0.789473684	0.942857143
0.289797315	0.783673469	0.6	0.787755102	0.3	0.804081633	0.6	0.787755102	0.441842306	0.787755102	0.999999999	0.926530612	0.5	0.787755102	0.803599538	0.804081633	0.679933982	0.902040816	0.9375	1	0.903029833	0.979591837	0.789473684	0.955102041
0.289797315	0.787755102	0.6	0.791836735	0.3	0.808163265	0.6	0.791836735	0.453086469	0.791836735	1	0.934693878	0.5	0.791836735	0.819608798	0.808163265	0.691476844	0.914285714	0.9375	1	0.935102286	0.983673469	0.816954252	0.959183673
0.289797315	0.791836735	0.6	0.795918367	0.300000054	0.812244898	0.6	0.8	0.453086469	0.795918367	1	0.959183673	0.5	0.795918367	0.819608869	0.812244898	0.70357947	0.918367347	0.9375	1	0.9375	0.987755102	0.816954264	0.963265306
0.289797315	0.795918367	0.6	0.8	0.300000066	0.816326531	0.6	0.804081633	0.453086469	0.8	1	0.983673469	0.5	0.8	0.819608869	0.816326531	0.730238751	0.92244898	0.9375	1	0.9375	0.991836735	0.85756411	0.967346939
0.3	0.8	0.6	0.804081633	0.300000066	0.820408163	0.6	0.808163265	0.453086469	0.804081633	1	0.995918367	0.5	0.804081633	0.822700121	0.820408163	0.731679814	0.926530612	0.9375	1	0.9375	0.995918367	0.872754445	0.971428571
0.3	0.804081633	0.6	0.808163265	0.300000702	0.824489796	0.6	0.812244898	0.5	0.808163265	1.021619579	1	0.5	0.808163265	0.82769422	0.824489796	0.749999999	0.934693878	0.9375	1	1.045884288	1	0.873575097	0.975510204
0.3	0.808163265	0.6	0.812244898	0.300000702	0.828571429	0.6	0.816326531	0.5	0.812244898	1.021619579	1	0.5	0.812244898	0.828971939	0.828571429	0.75	0.959183673	0.9375	1	1.045884288	1	0.873575117	0.979591837
0.3	0.812244898	0.6	0.816326531	0.300000702	0.832653061	0.6	0.820408163	0.5	0.816326531	1.021619579	1	0.5	0.816326531	0.836113387	0.836734694	0.75	0.971428571	0.9375	1	1.045884288	1	0.881455695	0.983673469
0.3	0.816326531	0.6	0.820408163	0.300000702	0.836734694	0.6	0.824489796	0.5	0.820408163	1.021619579	1	0.5	0.820408163	0.836113398	0.840816327	0.789473684	0.979591837	0.9375	1	1.045884288	1	0.881455695	0.987755102
0.3	0.820408163	0.6	0.824489796	0.374967031	0.840816327	0.621286596	0.828571429	0.5	0.824489796	1.021619579	1	0.5	0.824489796	0.850080012	0.844897959	0.789473684	0.991836735	0.9375	1	1.045884288	1	0.881455695	0.991836735
0.3	0.824489796	0.621286686	0.828571429	0.374967033	0.844897959	0.621286596	0.832653061	0.5	0.828571429	1.021619579	1	0.5	0.828571429	0.858176339	0.848979592	0.805885578	0.995918367	0.9375	1	1.045884288	1	0.881455695	0.995918367
0.3	0.828571429	0.621286686	0.832653061	0.374997797	0.848979592	0.621286596	0.836734694	0.5	0.832653061	1.021619579	1	0.5	0.832653061	0.87777491	0.853061224	0.811747862	1	0.9375	1	1.045884288	1	0.895558803	1
0.3	0.832653061	0.621286686	0.836734694	0.374999059	0.853061224	0.621286596	0.840816327	0.5	0.836734694	1.021619579	1	0.5	0.836734694	0.87777491	0.857142857	0.811747862	1	0.9375	1	1.045884288	1	0.895558803	1
0.3	0.836734694	0.621286686	0.840816327	0.374999642	0.857142857	0.671548763	0.844897959	0.5	0.840816327	1.021619579	1	0.500000001	0.840816327	0.893617279	0.86122449	0.811747862	1	0.9375	1	1.045884288	1	0.895558803	1
0.315789671	0.840816327	0.671548639	0.844897959	0.375	0.86122449	0.671548763	0.848979592	0.5	0.844897959	1.021619579	1	0.500000001	0.844897959	0.893617279	0.865306122	0.811747862	1	0.9375	1	1.045884288	1	0.895558803	1
0.315789881	0.844897959	0.671548639	0.848979592	0.375	0.865306122	0.671548763	0.853061224	0.513363885	0.848979592	1.021619579	1	0.500000006	0.848979592	0.893617279	0.869387755	0.811747862	1	0.9375	1	1.045884288	1	0.895558803	1
0.315789881	0.848979592	0.671548639	0.853061224	0.375	0.869387755	0.671548763	0.857142857	0.513363886	0.853061224	1.021619579	1	0.500000279	0.853061224	0.893617279	0.873469388	0.811747862	1	0.9375	1	1.045884288	1	0.895558803	1
0.315789881	0.853061224	0.671548639	0.857142857	0.375	0.873469388	0.674381863	0.86122449	0.527584782	0.857142857	1.021619579	1	0.500003989	0.857142857	0.893617279	0.87755102	0.811747862	1	0.9375	1	1.045884288	1	0.895558803	1
0.327400295	0.857142857	0.674381026	0.86122449	0.375	0.87755102	0.67438227	0.865306122	0.530059803	0.86122449	1.021619579	1	0.500029072	0.86122449	0.89361728	0.881632653	0.811747862	1	0.9375	1	1.045884288	1	0.895558803	1
0.335760189	0.86122449	0.674382814	0.865306122	0.375	0.881632653	0.67438227	0.869387755	0.530059803	0.865306122	1.021619579	1	0.500029087	0.865306122	0.903200146	0.885714286	0.811747862	1	0.9375	1	1.045884288	1	0.895558803	1
0.335760189	0.865306122	0.674382814	0.869387755	0.375	0.885714286	0.67438227	0.873469388	0.548551156	0.869387755	1.021619579	1	0.543067016	0.869387755	0.903200146	0.889795918	0.811747862	1	0.9375	1	1.045884288	1	0.895558803	1
0.335760189	0.869387755	0.674382814	0.873469388	0.375	0.889795918	0.735376461	0.87755102	0.549169789	0.873469388	1.021619579	1	0.546918191	0.873469388	0.903200146	0.893877551	0.811747862	1	0.9375	1	1.045884288	1	0.895558803	1
0.335760189	0.873469388	0.719565001	0.87755102	0.375000659	0.893877551	0.735376461	0.881632653	0.584646636	0.87755102	1.021619579	1	0.560585073	0.87755102	0.903200146	0.897959184	0.811747862	1	0.9375	1	1.045884288	1	0.895558803	1
0.352757003	0.87755102	0.719565001	0.881632653	0.375000659	0.897959184	0.735376461	0.885714286	0.600005183	0.881632653	1.021619579	1	0.581749785	0.881632653	0.954434291	0.902040816	0.811747862	1	0.9375	1	1.045884288	1	0.895558803	1
0.352757003	0.881632653	0.75	0.885714286	0.375000734	0.902040816	0.75	0.889795918	0.604716873	0.885714286	1.021619579	1	0.585333434	0.885714286	0.999999962	0.906122449	0.811747862	1	0.9375	1	1.045884288	1	0.895558803	1
0.375	0.885714286	0.75	0.889795918	0.375000734	0.906122449	0.75	0.893877551	0.604716879	0.889795918	1.021619579	1	0.633974644	0.889795918	0.999999968	0.910204082	0.811747862	1	0.9375	1	1.045884288	1	0.895558803	1
0.375	0.889795918	0.75	0.893877551	0.375000734	0.910204082	0.75	0.897959184	0.613957422	0.893877551	1.021619579	1	0.63397465	0.893877551	0.999999977	0.914285714	0.811747862	1	0.9375	1	1.045884288	1	0.895558803	1
0.375	0.893877551	0.75	0.897959184	0.375010987	0.914285714	0.75	0.902040816	0.657511921	0.897959184	1.021619579	1	0.666666035	0.897959184	0.999999978	0.918367347	0.811747862	1	0.9375	1	1.045884288	1	0.895558803	1
0.375	0.897959184	0.763708689	0.902040816	0.375010987	0.918367347	0.763708491	0.906122449	0.687013628	0.902040816	1.021619579	1	0.666666035	0.902040816	0.99999998	0.92244898	0.811747862	1	0.9375	1	1.045884288	1	0.895558803	1
0.377987193	0.902040816	0.763708689	0.906122449	0.375010988	0.92244898	0.763708491	0.910204082	0.693607401	0.906122449	1.021619579	1	0.690582867	0.906122449	0.999999995	0.930612245	0.811747862	1	0.9375	1	1.045884288	1	0.895558803	1
0.377987193	0.906122449	0.763708689	0.910204082	0.375010989	0.926530612	0.763708491	0.914285714	0.700088058	0.914285714	1.021619579	1	0.690582876	0.910204082	0.999999995	0.93877551	0.811747862	1	0.9375	1	1.045884288	1	0.895558803	1
0.377987193	0.910204082	0.789082057	0.914285714	0.37501099	0.930612245	0.781218979	0.918367347	0.702998843	0.918367347	1.021619579	1	0.704291017	0.914285714	0.999999996	0.946938776	0.811747862	1	0.9375	1	1.045884288	1	0.895558803	1
0.385965557	0.914285714	0.789082057	0.918367347	0.375010991	0.934693878	0.781218979	0.92244898	0.709814707	0.92244898	1.021619579	1	0.966428592	0.918367347	0.999999996	0.963265306	0.811747862	1	0.9375	1	1.045884288	1	0.895558803	1
0.385965557	0.918367347	0.789082057	0.92244898	0.5	0.93877551	0.79017239	0.926530612	0.785574756	0.926530612	1.021619579	1	0.966432401	0.92244898	0.999999998	0.967346939	0.811747862	1	0.9375	1	1.045884288	1	0.895558803	1
0.385965586	0.92244898	0.790169425	0.926530612	0.5	0.942857143	0.790173735	0.930612245	0.800001942	0.930612245	1.021619579	1	0.966436839	0.926530612	0.999999999	0.971428571	0.811747862	1	0.9375	1	1.045884288	1	0.895558803	1
0.423077198	0.926530612	0.79017567	0.930612245	0.5	0.946938776	0.790173735	0.934693878	0.819955189	0.934693878	1.021619579	1	0.999999713	0.930612245	1	0.979591837	0.811747862	1	0.9375	1	1.045884288	1	0.895558803	1
0.423077198	0.930612245	0.79017567	0.934693878	0.5	0.951020408	0.881854246	0.93877551	0.830366139	0.93877551	1.021619579	1	0.999999995	0.93877551	1	0.991836735	0.811747862	1	0.9375	1	1.045884288	1	0.895558803	1
0.423077198	0.934693878	0.881854346	0.93877551	0.5	0.955102041	0.881854246	0.942857143	0.844460535	0.942857143	1.021619579	1	0.999999998	0.942857143	1	1	0.811747862	1	0.9375	1	1.045884288	1	0.895558803	1
0.423077198	0.93877551	0.881854346	0.942857143	0.5	0.959183673	0.881854246	0.946938776	0.870496874	0.946938776	1.021619579	1	0.999999999	0.946938776	1	1	0.811747862	1	0.9375	1	1.045884288	1	0.895558803	1
0.423077198	0.942857143	0.881854346	0.946938776	0.5	0.963265306	0.890405984	0.951020408	0.882065121	0.951020408	1.021619579	1	0.999999999	0.951020408	1	1	0.811747862	1	0.9375	1	1.045884288	1	0.895558803	1
0.423077198	0.946938776	0.890405901	0.951020408	0.5	0.967346939	0.890405984	0.955102041	0.88368461	0.955102041	1.021619579	1	1	0.955102041	1	1	0.811747862	1	0.9375	1	1.045884288	1	0.895558803	1
0.466413937	0.951020408	0.890405901	0.955102041	0.5	0.971428571	0.890405984	0.959183673	0.946544447	0.959183673	1.021619579	1	1	0.959183673	1	1	0.811747862	1	0.9375	1	1.045884288	1	0.895558803	1
0.466413937	0.955102041	0.890405901	0.959183673	0.5	0.975510204	0.964822446	0.963265306	0.983674651	0.963265306	1.021619579	1	1	0.963265306	1	1	0.811747862	1	0.9375	1	1.045884288	1	0.895558803	1
0.466413937	0.959183673	0.978477724	0.963265306	0.5	0.979591837	0.964822446	0.967346939	0.999999996	0.967346939	1.021619579	1	1	0.967346939	1	1	0.811747862	1	0.9375	1	1.045884288	1	0.895558803	1
0.466945022	0.963265306	0.978477724	0.967346939	0.5	0.983673469	0.964822446	0.971428571	1	0.975510204	1.021619579	1	1	0.979591837	1	1	0.811747862	1	0.9375	1	1.045884288	1	0.895558803	1
0.466945022	0.967346939	0.996816446	0.971428571	0.749911737	0.987755102	0.978478434	0.975510204	1	0.987755102	1.021619579	1	1	0.987755102	1	1	0.811747862	1	0.9375	1	1.045884288	1	0.895558803	1
0.497363862	0.971428571	0.996816446	0.975510204	0.749990028	0.991836735	0.978478434	0.979591837	1	0.995918367	1.021619579	1	1	0.995918367	1	1	0.811747862	1	0.9375	1	1.045884288	1	0.895558803	1
0.497363862	0.975510204	1	0.979591837	0.750009973	0.995918367	1.004369232	0.983673469	1.004633594	1	1.021619579	1	1.183012672	1	1	1	0.811747862	1	0.9375	1	1.045884288	1	0.895558803	1
0.5	0.979591837	1	0.983673469	0.750088267	1	1.009224138	0.987755102	1.004633594	1	1.021619579	1	1.183012672	1	1	1	0.811747862	1	0.9375	1	1.045884288	1	0.895558803	1
0.5	0.983673469	1	0.987755102	0.750088267	1	1.009224138	0.991836735	1.004633594	1	1.021619579	1	1.183012672	1	1	1	0.811747862	1	0.9375	1	1.045884288	1	0.895558803	1
0.5	0.987755102	1.004367472	0.991836735	0.750088267	1	1.103064672	1	1.004633594	1	1.021619579	1	1.183012672	1	1	1	0.811747862	1	0.9375	1	1.045884288	1	0.895558803	1
0.610747268	0.991836735	1.171212752	0.995918367	0.750088267	1	1.103064672	1	1.004633594	1	1.021619579	1	1.183012672	1	1	1	0.811747862	1	0.9375	1	1.045884288	1	0.895558803	1
0.610747268	0.995918367	1.171212752	1	0.750088267	1	1.103064672	1	1.004633594	1	1.021619579	1	1.183012672	1	1	1	0.811747862	1	0.9375	1	1.045884288	1	0.895558803	1
0.958070412	1	1.171212752	1	0.750088267	1	1.103064672	1	1.004633594	1	1.021619579	1	1.183012672	1	1	1	0.811747862	1	0.9375	1	1.045884288	1	0.895558803	1


==> Figs/CDF_Data_L.tex <==
Opt-L1-X	Opt-L1-Y	Super-L1-X	Super-L1-Y	Heur-L1-X	Heur-L1-Y	Opt-L5-X	Opt-L5-Y	Super-L5-X	Super-L5-Y	Heur-L5-X	Heur-L5-Y	Opt-L10-X	Opt-L10-Y	Super-L10-X	Super-L10-Y	Heur-L10-X	Heur-L10-Y	Opt-L15-X	Opt-L15-Y	Super-L15-X	Super-L15-Y	Heur-L15-X	Heur-L15-Y	Opt-L20-X	Opt-L20-Y
0.036202772	0	0.007513198	0	0.022616248	0	0.028945235	0	0.008220415	0	0.020861148	0	0.022778431	0	0.010573412	0	0.022963987	0	0.019612439	0	0.008440983	0	0.017298854	0	0.014509567	0
0.038155682	0.009259259	0.009474058	0.009259259	0.029401122	0.009259259	0.035976153	0.009259259	0.018755072	0.009259259	0.027513344	0.009259259	0.032896052	0.009259259	0.015236394	0.009259259	0.031199517	0.009259259	0.024650341	0.009191176	0.01452234	0.009191176	0.028725346	0.009191176	0.027949689	0.012973534
0.046319477	0.018518519	0.011680537	0.018518519	0.031662747	0.018518519	0.041837494	0.018518519	0.020088019	0.018518519	0.030720079	0.02037037	0.034771907	0.018518519	0.024331503	0.018518519	0.033592619	0.018518519	0.032326674	0.018382353	0.023402092	0.018382353	0.034548084	0.018382353	0.03663309	0.026206539
0.051861869	0.027777778	0.015083325	0.027777778	0.032206633	0.027777778	0.046856447	0.027777778	0.021944472	0.027777778	0.035675859	0.02962963	0.036890159	0.027777778	0.027948925	0.027777778	0.036998782	0.027777778	0.037294811	0.027573529	0.025233928	0.027573529	0.040604998	0.027573529	0.044720481	0.039180073
0.053774624	0.037037037	0.016482101	0.037037037	0.034687185	0.037037037	0.051415344	0.037037037	0.025404723	0.037037037	0.039018107	0.040740741	0.043386101	0.037037037	0.031353174	0.037037037	0.042567657	0.037037037	0.044930683	0.036764706	0.027766925	0.038602941	0.046582815	0.036764706	0.050580718	0.052153607
0.058071667	0.046296296	0.01741064	0.05	0.03597561	0.051851852	0.055706348	0.046296296	0.027540951	0.048148148	0.04541638	0.05	0.05299682	0.046296296	0.035410014	0.046296296	0.045228136	0.046296296	0.051095181	0.047794118	0.032293107	0.047794118	0.050639566	0.045955882	0.054989158	0.066165023
0.062709922	0.055555556	0.017862594	0.059259259	0.037308673	0.061111111	0.058183359	0.055555556	0.032001273	0.059259259	0.04789272	0.061111111	0.057723219	0.055555556	0.039127121	0.057407407	0.046720988	0.055555556	0.053457142	0.056985294	0.035054564	0.056985294	0.051840375	0.056985294	0.060002745	0.08017644
0.065109566	0.064814815	0.020459255	0.068518519	0.038414634	0.075925926	0.060176163	0.064814815	0.033964635	0.07037037	0.050144484	0.072222222	0.06162391	0.064814815	0.043869818	0.066666667	0.048886294	0.064814815	0.058721286	0.066176471	0.044010159	0.066176471	0.054906232	0.066176471	0.065993461	0.093668915
0.065222609	0.074074074	0.025585865	0.07962963	0.03902439	0.087037037	0.062954912	0.074074074	0.041311426	0.07962963	0.052491063	0.081481481	0.064560608	0.075925926	0.047284756	0.077777778	0.050335089	0.074074074	0.068038179	0.075367647	0.047968056	0.075367647	0.056075776	0.075367647	0.070774579	0.107680332
0.065222609	0.085185185	0.027952078	0.094444444	0.039859694	0.096296296	0.064086568	0.083333333	0.04321903	0.090740741	0.055495781	0.094444444	0.068410338	0.085185185	0.04990292	0.088888889	0.052272511	0.083333333	0.069310105	0.084558824	0.049886833	0.086397059	0.058574751	0.084558824	0.076573374	0.121172807
0.065222609	0.096296296	0.031271613	0.105555556	0.040322581	0.105555556	0.065060678	0.092592593	0.046765581	0.101851852	0.057458056	0.107407407	0.073286293	0.094444444	0.053109422	0.098148148	0.055618856	0.092592593	0.073035333	0.09375	0.057825771	0.095588235	0.059768186	0.095588235	0.081793621	0.135443695
0.065827511	0.105555556	0.033974141	0.12037037	0.040778424	0.114814815	0.067286519	0.101851852	0.051289462	0.111111111	0.0598659	0.116666667	0.079194569	0.105555556	0.056531005	0.111111111	0.056470943	0.101851852	0.075996079	0.104779412	0.06062423	0.104779412	0.062448864	0.104779412	0.08588719	0.149455112
0.067821125	0.114814815	0.036770651	0.131481481	0.041624622	0.125925926	0.070228692	0.111111111	0.057152912	0.12037037	0.060999802	0.127777778	0.080845083	0.114814815	0.061155747	0.12037037	0.058123911	0.114814815	0.078689867	0.117647059	0.066442715	0.113970588	0.064353426	0.113970588	0.089953212	0.163466528
0.070062889	0.124074074	0.038198546	0.144444444	0.042729592	0.137037037	0.071906389	0.12037037	0.060299306	0.12962963	0.064977258	0.137037037	0.081323835	0.125925926	0.062679278	0.12962963	0.060660236	0.125925926	0.080814274	0.126838235	0.07321455	0.123161765	0.065279302	0.123161765	0.093542036	0.176699533
0.070786598	0.135185185	0.04050706	0.157407407	0.043197033	0.146296296	0.077081272	0.12962963	0.063965709	0.148148148	0.066292901	0.148148148	0.081818167	0.135185185	0.066593364	0.140740741	0.062414938	0.137037037	0.08510327	0.136029412	0.076734162	0.134191176	0.066584888	0.132352941	0.09707609	0.19071095
0.07250789	0.144444444	0.043736956	0.17037037	0.044412145	0.155555556	0.077208299	0.138888889	0.070620958	0.159259259	0.068226121	0.159259259	0.084558575	0.144444444	0.068859548	0.151851852	0.064849166	0.146296296	0.085329588	0.145220588	0.082052839	0.147058824	0.068514496	0.141544118	0.100774148	0.204203425
0.072507898	0.153703704	0.046121379	0.185185185	0.04509334	0.166666667	0.079389399	0.148148148	0.075469982	0.17962963	0.069692334	0.168518519	0.085042102	0.153703704	0.074143028	0.161111111	0.065535685	0.159259259	0.086311367	0.154411765	0.087176598	0.161764706	0.070659326	0.150735294	0.106130805	0.217955371
0.072507898	0.162962963	0.049204075	0.2	0.045968205	0.175925926	0.083694047	0.157407407	0.077710728	0.188888889	0.071247989	0.177777778	0.085701119	0.162962963	0.078081716	0.175925926	0.067765131	0.172222222	0.086944858	0.163602941	0.091982779	0.170955882	0.073132674	0.165441176	0.111047229	0.231188376
0.073473275	0.172222222	0.054542218	0.209259259	0.046644985	0.185185185	0.085452341	0.166666667	0.082585215	0.201851852	0.07239715	0.187037037	0.087084738	0.172222222	0.084202989	0.2	0.069580882	0.181481481	0.090469026	0.172794118	0.093522145	0.183823529	0.075068056	0.174632353	0.113227313	0.24416191
0.073567464	0.181481481	0.064407916	0.25	0.047305965	0.194444444	0.086361807	0.175925926	0.086763557	0.225925926	0.072902202	0.196296296	0.08908511	0.183333333	0.0859595	0.22037037	0.071453898	0.192592593	0.095952351	0.185661765	0.097793901	0.204044118	0.076855391	0.183823529	0.117144347	0.258173326
0.076920259	0.190740741	0.069585373	0.259259259	0.047642119	0.205555556	0.090072948	0.185185185	0.09044896	0.248148148	0.074664012	0.205555556	0.090207996	0.192592593	0.088292298	0.237037037	0.072947459	0.203703704	0.097590604	0.194852941	0.101448126	0.222426471	0.080460075	0.193014706	0.120412369	0.271665802
0.080789621	0.2	0.077218221	0.292592593	0.048356727	0.214814815	0.092280665	0.194444444	0.098092804	0.274074074	0.075661696	0.214814815	0.092264954	0.201851852	0.090402181	0.253703704	0.073567835	0.212962963	0.099936948	0.204044118	0.105168709	0.246323529	0.081867236	0.202205882	0.126243412	0.284898806
0.080789621	0.209259259	0.08565399	0.342592593	0.048909557	0.225925926	0.095417156	0.203703704	0.103801747	0.294444444	0.07710728	0.224074074	0.094537815	0.211111111	0.094537815	0.285185185	0.075172361	0.222222222	0.102261491	0.213235294	0.118183955	0.259191176	0.083284537	0.211397059	0.129537321	0.298650752
0.080789621	0.218518519	0.092358433	0.4	0.049320054	0.237037037	0.097739785	0.212962963	0.108323006	0.32037037	0.077863979	0.233333333	0.095083043	0.22037037	0.100298126	0.301851852	0.076488759	0.235185185	0.102462885	0.222426471	0.120796107	0.277573529	0.085621817	0.220588235	0.13217274	0.312402698
0.08138515	0.227777778	0.09761558	0.498148148	0.050063776	0.246296296	0.100833609	0.222222222	0.110959457	0.35	0.07851034	0.242592593	0.095450206	0.22962963	0.101777977	0.314814815	0.077365191	0.244444444	0.103799258	0.231617647	0.127742753	0.294117647	0.08718631	0.229779412	0.134831042	0.326154645
0.08138515	0.237037037	0.110888693	0.566666667	0.050496405	0.255555556	0.101750266	0.231481481	0.113850036	0.375925926	0.07931343	0.251851852	0.096689278	0.238888889	0.106668681	0.342592593	0.078270801	0.253703704	0.104984784	0.240808824	0.13067116	0.310661765	0.089048572	0.238970588	0.137579161	0.33964712
0.08243215	0.246296296	0.1182531	0.633333333	0.051679587	0.274074074	0.101850591	0.240740741	0.118827592	0.401851852	0.080341202	0.261111111	0.097824209	0.248148148	0.112899515	0.362962963	0.080019885	0.264814815	0.10543542	0.25	0.134110851	0.329044118	0.089619723	0.248161765	0.140949983	0.352880125
0.083333379	0.255555556	0.12471139	0.705555556	0.052083333	0.287037037	0.105136066	0.25	0.125553103	0.440740741	0.081347108	0.27037037	0.097848104	0.257407407	0.121959852	0.381481481	0.080749013	0.275925926	0.110468221	0.259191176	0.138996388	0.351102941	0.092201031	0.257352941	0.143361725	0.365853659
0.083333379	0.264814815	0.132912897	0.766666667	0.052890827	0.301851852	0.107990734	0.259259259	0.130372279	0.47037037	0.083314181	0.27962963	0.100672381	0.266666667	0.125247349	0.396296296	0.082282696	0.285185185	0.114533889	0.268382353	0.143089111	0.373161765	0.09358232	0.266544118	0.145857481	0.379605605
0.083333379	0.274074074	0.142630158	0.824074074	0.053607467	0.316666667	0.108222038	0.268518519	0.134704376	0.501851852	0.083861816	0.290740741	0.100672381	0.275925926	0.135444635	0.412962963	0.085166374	0.298148148	0.115835358	0.277573529	0.148441371	0.400735294	0.095654253	0.275735294	0.148317569	0.39309808
0.085282082	0.283333333	0.168489125	0.875925926	0.054432957	0.32962963	0.108483307	0.277777778	0.136680603	0.522222222	0.085007728	0.3	0.102552608	0.287037037	0.140468965	0.431481481	0.086022168	0.307407407	0.118467975	0.286764706	0.154335962	0.424632353	0.097948694	0.284926471	0.151322979	0.406590555
0.085282082	0.292592593	0.187247279	0.924074074	0.055216165	0.340740741	0.11151657	0.287037037	0.141352958	0.546296296	0.085976741	0.311111111	0.105793537	0.296296296	0.14299131	0.45	0.08691426	0.316666667	0.121854723	0.295955882	0.160686911	0.454044118	0.09894817	0.294117647	0.155730056	0.41982356
0.085850631	0.301851852	0.211254928	0.959259259	0.056125722	0.351851852	0.111665059	0.296296296	0.145708629	0.566666667	0.086685824	0.32037037	0.106502777	0.305555556	0.148102429	0.474074074	0.089901464	0.325925926	0.130697226	0.305147059	0.169122212	0.472426471	0.101371286	0.303308824	0.15946145	0.433575506
0.085850631	0.311111111	0.264788511	0.990740741	0.0566605	0.361111111	0.11191087	0.305555556	0.149664708	0.588888889	0.088013032	0.32962963	0.107236805	0.314814815	0.149994338	0.490740741	0.091458796	0.335185185	0.134104181	0.314338235	0.175675676	0.496323529	0.102215375	0.3125	0.161962478	0.447586923
0.085850819	0.32037037	0.264788511	0.990740741	0.057391524	0.372222222	0.112661685	0.314814815	0.153984887	0.607407407	0.089059986	0.338888889	0.108142257	0.324074074	0.153811234	0.507407407	0.092553253	0.344444444	0.137122646	0.323529412	0.188571572	0.509191176	0.103596664	0.321691176	0.168578211	0.461338869
0.088898534	0.32962963	0.264788511	0.990740741	0.057939092	0.381481481	0.113321516	0.324074074	0.166799504	0.625925926	0.089240184	0.35	0.111477997	0.333333333	0.15877005	0.527777778	0.094299131	0.353703704	0.137446654	0.332720588	0.199232121	0.522058824	0.10461187	0.330882353	0.175492414	0.474831344
0.089660749	0.338888889	0.264788511	0.990740741	0.05893186	0.390740741	0.114540625	0.333333333	0.170677353	0.644444444	0.089779529	0.362962963	0.114063702	0.342592593	0.16643834	0.548148148	0.096678387	0.364814815	0.13935948	0.341911765	0.225655633	0.540441176	0.106147097	0.340073529	0.182363755	0.488064349
0.089660749	0.348148148	0.264788511	0.990740741	0.059392265	0.4	0.114540628	0.342592593	0.17606288	0.661111111	0.090515043	0.372222222	0.114798033	0.351851852	0.169291363	0.566666667	0.098202043	0.374074074	0.140791832	0.351102941	0.228463006	0.566176471	0.107099062	0.349264706	0.195477857	0.502594707
0.091358797	0.357407407	0.264788511	0.990740741	0.060572687	0.411111111	0.115873219	0.351851852	0.179200783	0.677777778	0.091515497	0.383333333	0.116112985	0.361111111	0.173361559	0.587037037	0.09890247	0.385185185	0.143928526	0.360294118	0.233784087	0.590073529	0.108135504	0.358455882	0.208805245	0.51894136
0.091358797	0.366666667	0.264788511	0.990740741	0.06130064	0.422222222	0.117348897	0.361111111	0.183841334	0.696296296	0.09263981	0.392592593	0.118049797	0.37037037	0.17983606	0.607407407	0.101100393	0.394444444	0.146385907	0.371323529	0.246190079	0.610294118	0.11055387	0.369485294	0.222441318	0.537882719
0.095610733	0.375925926	0.264788511	0.990740741	0.062248611	0.431481481	0.118970187	0.37037037	0.195558419	0.724074074	0.093235469	0.401851852	0.121547027	0.37962963	0.189139025	0.627777778	0.102419384	0.403703704	0.1473831	0.380514706	0.250048543	0.630514706	0.112269818	0.380514706	0.230422048	0.568240789
0.095610733	0.385185185	0.264788511	0.990740741	0.063075506	0.440740741	0.121052186	0.37962963	0.203320964	0.740740741	0.094339623	0.411111111	0.121688502	0.388888889	0.204614036	0.638888889	0.105132048	0.412962963	0.1473831	0.389705882	0.258950877	0.648897059	0.114580769	0.389705882	0.240824738	0.601712506
0.096974846	0.394444444	0.264788511	0.990740741	0.06376241	0.45	0.121052996	0.388888889	0.209823963	0.757407407	0.095818815	0.422222222	0.12567598	0.398148148	0.227087143	0.65	0.105909014	0.424074074	0.150462415	0.398897059	0.264373532	0.685661765	0.118154449	0.398897059	0.254251561	0.640114167
0.096974846	0.403703704	0.264788511	0.990740741	0.06505102	0.459259259	0.121808987	0.398148148	0.218720749	0.77037037	0.09768985	0.433333333	0.126154025	0.409259259	0.241859344	0.666666667	0.108630579	0.433333333	0.150462415	0.408088235	0.266908675	0.707720588	0.121437957	0.408088235	0.264353608	0.686559419
0.097883869	0.412962963	0.264788511	0.990740741	0.065789474	0.47037037	0.12293803	0.407407407	0.223142536	0.8	0.098847416	0.442592593	0.126385531	0.418518519	0.244547306	0.67962963	0.109499623	0.444444444	0.15076572	0.417279412	0.277992776	0.731617647	0.123190845	0.419117647	0.273824882	0.737675143
0.097922636	0.422222222	0.264788511	0.990740741	0.067219153	0.47962963	0.123089936	0.416666667	0.229448962	0.814814815	0.099629791	0.451851852	0.130781042	0.42962963	0.258018221	0.696296296	0.111594128	0.455555556	0.15189636	0.426470588	0.284025134	0.753676471	0.124046372	0.428308824	0.284316737	0.791385573
0.097922636	0.431481481	0.264788511	0.990740741	0.069765649	0.490740741	0.123494351	0.425925926	0.249400347	0.82962963	0.101137318	0.462962963	0.135107877	0.438888889	0.267170583	0.709259259	0.114713891	0.47037037	0.157096201	0.435661765	0.293381703	0.777573529	0.127253282	0.439338235	0.292716165	0.845096004
0.098366548	0.440740741	0.264788511	0.990740741	0.071369344	0.501851852	0.124999966	0.435185185	0.263389049	0.842592593	0.101931027	0.472222222	0.137500355	0.448148148	0.274628391	0.722222222	0.116657056	0.47962963	0.157524866	0.444852941	0.296882742	0.805147059	0.128932464	0.448529412	0.308148279	0.89699014
0.098366548	0.451851852	0.264788511	0.990740741	0.072553897	0.512962963	0.125	0.444444444	0.282705917	0.853703704	0.103448276	0.481481481	0.140620076	0.457407407	0.279377614	0.735185185	0.117808195	0.488888889	0.158218881	0.454044118	0.304589742	0.841911765	0.130987577	0.457720588	0.324942508	0.945511157
0.102827377	0.461111111	0.264788511	0.990740741	0.073442312	0.525925926	0.125000001	0.453703704	0.315260563	0.862962963	0.105344505	0.492592593	0.14648899	0.466666667	0.282666641	0.748148148	0.118870161	0.498148148	0.16089176	0.465073529	0.31054516	0.863970588	0.136119453	0.470588235	0.382845946	0.990659056
0.104842598	0.47037037	0.264788511	0.990740741	0.075331971	0.537037037	0.125000009	0.462962963	0.328350166	0.875925926	0.106862072	0.505555556	0.148697755	0.475925926	0.292982475	0.766666667	0.122714575	0.507407407	0.168974435	0.474264706	0.315506126	0.887867647	0.139510174	0.479779412	0.382845946	0.990659056
0.104842598	0.47962963	0.264788511	0.990740741	0.076699834	0.548148148	0.126041979	0.472222222	0.33752285	0.888888889	0.107643525	0.514814815	0.149564219	0.485185185	0.298170058	0.785185185	0.123546252	0.516666667	0.171156594	0.483455882	0.335582102	0.915441176	0.141003293	0.488970588	0.382845946	0.990659056
0.106384056	0.488888889	0.264788511	0.990740741	0.078729282	0.559259259	0.126587917	0.481481481	0.356938359	0.901851852	0.109778242	0.527777778	0.151008572	0.494444444	0.304156568	0.803703704	0.126264949	0.525925926	0.175675676	0.492647059	0.351351351	0.950367647	0.143812197	0.498161765	0.382845946	0.990659056
0.106384056	0.498148148	0.264788511	0.990740741	0.079778704	0.57037037	0.127223055	0.490740741	0.363511829	0.914814815	0.112128287	0.537037037	0.153827387	0.503703704	0.308548604	0.82037037	0.129053128	0.537037037	0.177701963	0.501838235	0.363471417	0.972426471	0.147797907	0.516544118	0.382845946	0.990659056
0.108046314	0.507407407	0.264788511	0.990740741	0.081031308	0.57962963	0.129469496	0.5	0.387458029	0.927777778	0.114106122	0.548148148	0.156063828	0.512962963	0.319020684	0.833333333	0.130413983	0.546296296	0.182697172	0.511029412	0.483934319	0.998161765	0.149023296	0.525735294	0.382845946	0.990659056
0.108335949	0.516666667	0.264788511	0.990740741	0.082354443	0.588888889	0.132922294	0.509259259	0.40140499	0.937037037	0.115804972	0.557407407	0.158255984	0.522222222	0.327181198	0.859259259	0.133495758	0.557407407	0.193201293	0.520220588	0.483934319	0.998161765	0.150587787	0.551470588	0.382845946	0.990659056
0.109115983	0.525925926	0.264788511	0.990740741	0.08299285	0.598148148	0.133490073	0.518518519	0.417377148	0.95	0.116973619	0.566666667	0.160180828	0.531481481	0.332876681	0.875925926	0.134657119	0.566666667	0.205330751	0.529411765	0.483934319	0.998161765	0.153586217	0.560661765	0.382845946	0.990659056
0.109115983	0.535185185	0.264788511	0.990740741	0.08524335	0.607407407	0.135150749	0.527777778	0.431591469	0.961111111	0.118353248	0.575925926	0.164753064	0.540740741	0.338582726	0.890740741	0.136433009	0.575925926	0.216620609	0.545955882	0.483934319	0.998161765	0.157323118	0.569852941	0.382845946	0.990659056
0.110173926	0.544444444	0.264788511	0.990740741	0.086823289	0.618518519	0.135744419	0.537037037	0.446285073	0.97037037	0.119327222	0.585185185	0.170079343	0.55	0.341867014	0.924074074	0.138040295	0.585185185	0.226234878	0.555147059	0.483934319	0.998161765	0.161455899	0.579044118	0.382845946	0.990659056
0.110173926	0.553703704	0.264788511	0.990740741	0.089841539	0.62962963	0.137091583	0.546296296	0.453609331	0.97962963	0.12353482	0.594444444	0.171329594	0.559259259	0.347394401	0.938888889	0.139670403	0.594444444	0.232608847	0.564338235	0.483934319	0.998161765	0.163353438	0.608455882	0.382845946	0.990659056
0.110790484	0.562962963	0.264788511	0.990740741	0.092418546	0.638888889	0.143987646	0.555555556	0.498800694	0.990740741	0.126561382	0.603703704	0.17219705	0.568518519	0.359130655	0.966666667	0.142824287	0.609259259	0.238306006	0.575367647	0.483934319	0.998161765	0.169073393	0.619485294	0.382845946	0.990659056
0.111228693	0.572222222	0.264788511	0.990740741	0.09375	0.648148148	0.144216186	0.564814815	0.498800694	0.990740741	0.127556883	0.614814815	0.174013867	0.577777778	0.378151261	0.988888889	0.146280348	0.618518519	0.243709445	0.599264706	0.483934319	0.998161765	0.172942892	0.634191176	0.382845946	0.990659056
0.112180327	0.581481481	0.264788511	0.990740741	0.094476744	0.661111111	0.145540412	0.574074074	0.498800694	0.990740741	0.129438603	0.624074074	0.174169477	0.587037037	0.378151261	0.988888889	0.14812792	0.627777778	0.257321337	0.626838235	0.483934319	0.998161765	0.18163797	0.648897059	0.382845946	0.990659056
0.112612438	0.590740741	0.264788511	0.990740741	0.096619898	0.672222222	0.149739579	0.583333333	0.498800694	0.990740741	0.131680167	0.633333333	0.175520437	0.596296296	0.378151261	0.988888889	0.153082461	0.637037037	0.265775813	0.663602941	0.483934319	0.998161765	0.190736297	0.663602941	0.382845946	0.990659056
0.113215424	0.6	0.264788511	0.990740741	0.098214286	0.683333333	0.152720834	0.592592593	0.498800694	0.990740741	0.133017941	0.644444444	0.177003061	0.605555556	0.378151261	0.988888889	0.157354575	0.646296296	0.27424529	0.696691176	0.483934319	0.998161765	0.19546371	0.693014706	0.382845946	0.990659056
0.113215424	0.609259259	0.264788511	0.990740741	0.100316031	0.692592593	0.158456643	0.601851852	0.498800694	0.990740741	0.134246744	0.655555556	0.18794531	0.614814815	0.378151261	0.988888889	0.161814689	0.655555556	0.275018256	0.724264706	0.483934319	0.998161765	0.200286883	0.715073529	0.382845946	0.990659056
0.116031856	0.618518519	0.264788511	0.990740741	0.101513865	0.701851852	0.160115312	0.611111111	0.498800694	0.990740741	0.136249141	0.664814815	0.19183509	0.624074074	0.378151261	0.988888889	0.166612472	0.664814815	0.289797953	0.75	0.483934319	0.998161765	0.211892746	0.759191176	0.382845946	0.990659056
0.11793292	0.627777778	0.264788511	0.990740741	0.102209945	0.712962963	0.163598572	0.62037037	0.498800694	0.990740741	0.138861337	0.674074074	0.201388618	0.633333333	0.378151261	0.988888889	0.173376419	0.674074074	0.294766189	0.768382353	0.483934319	0.998161765	0.218541895	0.792279412	0.382845946	0.990659056
0.11793292	0.637037037	0.264788511	0.990740741	0.10469223	0.724074074	0.166347646	0.62962963	0.498800694	0.990740741	0.14032567	0.687037037	0.211255103	0.642592593	0.378151261	0.988888889	0.181326681	0.685185185	0.30153144	0.805147059	0.483934319	0.998161765	0.229783144	0.821691176	0.382845946	0.990659056
0.119601857	0.646296296	0.264788511	0.990740741	0.10626892	0.735185185	0.16666702	0.638888889	0.498800694	0.990740741	0.143324737	0.696296296	0.216559602	0.651851852	0.378151261	0.988888889	0.1895591	0.696296296	0.307400798	0.834558824	0.483934319	0.998161765	0.237686257	0.84375	0.382845946	0.990659056
0.119602873	0.655555556	0.264788511	0.990740741	0.107734807	0.744444444	0.167497588	0.648148148	0.498800694	0.990740741	0.147292204	0.705555556	0.222184232	0.661111111	0.378151261	0.988888889	0.194504973	0.705555556	0.315049718	0.862132353	0.483934319	0.998161765	0.245524093	0.875	0.382845946	0.990659056
0.119683561	0.664814815	0.264788511	0.990740741	0.11000283	0.753703704	0.170056834	0.657407407	0.498800694	0.990740741	0.152747471	0.714814815	0.230028172	0.67037037	0.378151261	0.988888889	0.197777335	0.714814815	0.32178352	0.895220588	0.483934319	0.998161765	0.256949961	0.90625	0.382845946	0.990659056
0.119683561	0.674074074	0.264788511	0.990740741	0.112799263	0.764814815	0.173013682	0.666666667	0.498800694	0.990740741	0.157621556	0.724074074	0.234730961	0.67962963	0.378151261	0.988888889	0.202631	0.731481481	0.341318832	0.931985294	0.483934319	0.998161765	0.28202132	0.948529412	0.382845946	0.990659056
0.120717259	0.683333333	0.264788511	0.990740741	0.118902439	0.774074074	0.178411794	0.675925926	0.498800694	0.990740741	0.168771777	0.733333333	0.240123343	0.692592593	0.378151261	0.988888889	0.208377778	0.746296296	0.355403925	0.955882353	0.483934319	0.998161765	0.319337128	0.976102941	0.382845946	0.990659056
0.127816992	0.692592593	0.264788511	0.990740741	0.122335271	0.783333333	0.180639902	0.685185185	0.498800694	0.990740741	0.173080738	0.742592593	0.24858812	0.701851852	0.378151261	0.988888889	0.215517906	0.766666667	0.386402587	0.985294118	0.483934319	0.998161765	0.333581257	0.998161765	0.382845946	0.990659056
0.127816992	0.701851852	0.264788511	0.990740741	0.123780488	0.792592593	0.190408766	0.694444444	0.498800694	0.990740741	0.175547879	0.751851852	0.260420751	0.711111111	0.378151261	0.988888889	0.224477881	0.787037037	0.386402587	0.985294118	0.483934319	0.998161765	0.333581257	0.998161765	0.382845946	0.990659056
0.127876513	0.711111111	0.264788511	0.990740741	0.130948305	0.801851852	0.190834311	0.703703704	0.498800694	0.990740741	0.178043791	0.762962963	0.273404346	0.731481481	0.378151261	0.988888889	0.230352214	0.801851852	0.386402587	0.985294118	0.483934319	0.998161765	0.333581257	0.998161765	0.382845946	0.990659056
0.128619568	0.72037037	0.264788511	0.990740741	0.133290816	0.811111111	0.193189822	0.712962963	0.498800694	0.990740741	0.181936322	0.772222222	0.284600914	0.744444444	0.378151261	0.988888889	0.237116333	0.818518519	0.386402587	0.985294118	0.483934319	0.998161765	0.333581257	0.998161765	0.382845946	0.990659056
0.131595403	0.72962963	0.264788511	0.990740741	0.13705446	0.82037037	0.194133822	0.722222222	0.498800694	0.990740741	0.184386973	0.781481481	0.29739551	0.77037037	0.378151261	0.988888889	0.24593963	0.846296296	0.386402587	0.985294118	0.483934319	0.998161765	0.333581257	0.998161765	0.382845946	0.990659056
0.132341908	0.738888889	0.264788511	0.990740741	0.140220735	0.82962963	0.194133822	0.731481481	0.498800694	0.990740741	0.188017557	0.790740741	0.302665021	0.787037037	0.378151261	0.988888889	0.257885578	0.864814815	0.386402587	0.985294118	0.483934319	0.998161765	0.333581257	0.998161765	0.382845946	0.990659056
0.132341908	0.748148148	0.264788511	0.990740741	0.142030034	0.838888889	0.195823797	0.740740741	0.498800694	0.990740741	0.193673922	0.801851852	0.308738605	0.805555556	0.378151261	0.988888889	0.263707553	0.896296296	0.386402587	0.985294118	0.483934319	0.998161765	0.333581257	0.998161765	0.382845946	0.990659056
0.140572519	0.757407407	0.264788511	0.990740741	0.142930503	0.848148148	0.203505659	0.75	0.498800694	0.990740741	0.198458133	0.811111111	0.315719752	0.82037037	0.378151261	0.988888889	0.267710658	0.916666667	0.386402587	0.985294118	0.483934319	0.998161765	0.333581257	0.998161765	0.382845946	0.990659056
0.141479954	0.768518519	0.264788511	0.990740741	0.144517822	0.857407407	0.207409983	0.759259259	0.498800694	0.990740741	0.203614983	0.82037037	0.320361655	0.838888889	0.378151261	0.988888889	0.273767735	0.935185185	0.386402587	0.985294118	0.483934319	0.998161765	0.333581257	0.998161765	0.382845946	0.990659056
0.14374257	0.77962963	0.264788511	0.990740741	0.147578204	0.866666667	0.214717731	0.768518519	0.498800694	0.990740741	0.208655332	0.82962963	0.32989634	0.855555556	0.378151261	0.988888889	0.282395847	0.955555556	0.386402587	0.985294118	0.483934319	0.998161765	0.333581257	0.998161765	0.382845946	0.990659056
0.14374257	0.788888889	0.264788511	0.990740741	0.156064914	0.875925926	0.218522538	0.777777778	0.498800694	0.990740741	0.21137965	0.838888889	0.342659189	0.885185185	0.378151261	0.988888889	0.308746226	0.985185185	0.386402587	0.985294118	0.483934319	0.998161765	0.333581257	0.998161765	0.382845946	0.990659056
0.143875899	0.798148148	0.264788511	0.990740741	0.168597561	0.885185185	0.218750018	0.787037037	0.498800694	0.990740741	0.215925449	0.848148148	0.348338954	0.907407407	0.378151261	0.988888889	0.368154306	1	0.386402587	0.985294118	0.483934319	0.998161765	0.333581257	0.998161765	0.382845946	0.990659056
0.148832377	0.807407407	0.264788511	0.990740741	0.172560976	0.894444444	0.220249234	0.796296296	0.498800694	0.990740741	0.225947109	0.857407407	0.352545528	0.925925926	0.378151261	0.988888889	0.368154306	1	0.386402587	0.985294118	0.483934319	0.998161765	0.333581257	0.998161765	0.382845946	0.990659056
0.148832377	0.816666667	0.264788511	0.990740741	0.178658537	0.903703704	0.22467691	0.805555556	0.498800694	0.990740741	0.238540692	0.866666667	0.364229713	0.953703704	0.378151261	0.988888889	0.368154306	1	0.386402587	0.985294118	0.483934319	0.998161765	0.333581257	0.998161765	0.382845946	0.990659056
0.148974724	0.825925926	0.264788511	0.990740741	0.187338501	0.912962963	0.230794157	0.814814815	0.498800694	0.990740741	0.243047575	0.877777778	0.377290247	0.977777778	0.378151261	0.988888889	0.368154306	1	0.386402587	0.985294118	0.483934319	0.998161765	0.333581257	0.998161765	0.382845946	0.990659056
0.149434582	0.835185185	0.264788511	0.990740741	0.198643411	0.922222222	0.239191248	0.824074074	0.498800694	0.990740741	0.252111761	0.887037037	0.432080123	0.992592593	0.378151261	0.988888889	0.368154306	1	0.386402587	0.985294118	0.483934319	0.998161765	0.333581257	0.998161765	0.382845946	0.990659056
0.153254996	0.844444444	0.264788511	0.990740741	0.2046716	0.931481481	0.254852782	0.833333333	0.498800694	0.990740741	0.259110539	0.9	0.432080123	0.992592593	0.378151261	0.988888889	0.368154306	1	0.386402587	0.985294118	0.483934319	0.998161765	0.333581257	0.998161765	0.382845946	0.990659056
0.156298575	0.853703704	0.264788511	0.990740741	0.219603763	0.940740741	0.270301497	0.842592593	0.498800694	0.990740741	0.272988506	0.914814815	0.432080123	0.992592593	0.378151261	0.988888889	0.368154306	1	0.386402587	0.985294118	0.483934319	0.998161765	0.333581257	0.998161765	0.382845946	0.990659056
0.156298575	0.862962963	0.264788511	0.990740741	0.232764748	0.95	0.294349632	0.853703704	0.498800694	0.990740741	0.290722997	0.925925926	0.432080123	0.992592593	0.378151261	0.988888889	0.368154306	1	0.386402587	0.985294118	0.483934319	0.998161765	0.333581257	0.998161765	0.382845946	0.990659056
0.168771848	0.872222222	0.264788511	0.990740741	0.261468675	0.959259259	0.314483897	0.864814815	0.498800694	0.990740741	0.304691484	0.938888889	0.432080123	0.992592593	0.378151261	0.988888889	0.368154306	1	0.386402587	0.985294118	0.483934319	0.998161765	0.333581257	0.998161765	0.382845946	0.990659056
0.170795357	0.881481481	0.264788511	0.990740741	0.297113752	0.968518519	0.331908986	0.877777778	0.498800694	0.990740741	0.317506676	0.95	0.432080123	0.992592593	0.378151261	0.988888889	0.368154306	1	0.386402587	0.985294118	0.483934319	0.998161765	0.333581257	0.998161765	0.382845946	0.990659056
0.171257102	0.890740741	0.264788511	0.990740741	0.323947278	0.977777778	0.339964546	0.887037037	0.498800694	0.990740741	0.337231969	0.962962963	0.432080123	0.992592593	0.378151261	0.988888889	0.368154306	1	0.386402587	0.985294118	0.483934319	0.998161765	0.333581257	0.998161765	0.382845946	0.990659056
0.172318139	0.9	0.264788511	0.990740741	0.39978678	0.987037037	0.376526935	0.898148148	0.498800694	0.990740741	0.360653723	0.977777778	0.432080123	0.992592593	0.378151261	0.988888889	0.368154306	1	0.386402587	0.985294118	0.483934319	0.998161765	0.333581257	0.998161765	0.382845946	0.990659056
0.1728954	0.909259259	0.264788511	0.990740741	0.424248228	0.996296296	0.387987403	0.912962963	0.498800694	0.990740741	0.381691479	0.988888889	0.432080123	0.992592593	0.378151261	0.988888889	0.368154306	1	0.386402587	0.985294118	0.483934319	0.998161765	0.333581257	0.998161765	0.382845946	0.990659056
0.181730204	0.918518519	0.264788511	0.990740741	0.424248228	0.996296296	0.395207587	0.927777778	0.498800694	0.990740741	0.434746328	0.998148148	0.432080123	0.992592593	0.378151261	0.988888889	0.368154306	1	0.386402587	0.985294118	0.483934319	0.998161765	0.333581257	0.998161765	0.382845946	0.990659056
0.207721204	0.927777778	0.264788511	0.990740741	0.424248228	0.996296296	0.406029958	0.940740741	0.498800694	0.990740741	0.434746328	0.998148148	0.432080123	0.992592593	0.378151261	0.988888889	0.368154306	1	0.386402587	0.985294118	0.483934319	0.998161765	0.333581257	0.998161765	0.382845946	0.990659056
0.208137307	0.937037037	0.264788511	0.990740741	0.424248228	0.996296296	0.416923053	0.95	0.498800694	0.990740741	0.434746328	0.998148148	0.432080123	0.992592593	0.378151261	0.988888889	0.368154306	1	0.386402587	0.985294118	0.483934319	0.998161765	0.333581257	0.998161765	0.382845946	0.990659056
0.213885096	0.946296296	0.264788511	0.990740741	0.424248228	0.996296296	0.434596453	0.961111111	0.498800694	0.990740741	0.434746328	0.998148148	0.432080123	0.992592593	0.378151261	0.988888889	0.368154306	1	0.386402587	0.985294118	0.483934319	0.998161765	0.333581257	0.998161765	0.382845946	0.990659056
0.226602479	0.957407407	0.264788511	0.990740741	0.424248228	0.996296296	0.44935382	0.972222222	0.498800694	0.990740741	0.434746328	0.998148148	0.432080123	0.992592593	0.378151261	0.988888889	0.368154306	1	0.386402587	0.985294118	0.483934319	0.998161765	0.333581257	0.998161765	0.382845946	0.990659056
0.252462932	0.966666667	0.264788511	0.990740741	0.424248228	0.996296296	0.463492874	0.981481481	0.498800694	0.990740741	0.434746328	0.998148148	0.432080123	0.992592593	0.378151261	0.988888889	0.368154306	1	0.386402587	0.985294118	0.483934319	0.998161765	0.333581257	0.998161765	0.382845946	0.990659056
0.276709096	0.975925926	0.264788511	0.990740741	0.424248228	0.996296296	0.509705564	0.994444444	0.498800694	0.990740741	0.434746328	0.998148148	0.432080123	0.992592593	0.378151261	0.988888889	0.368154306	1	0.386402587	0.985294118	0.483934319	0.998161765	0.333581257	0.998161765	0.382845946	0.990659056
0.285415811	0.985185185	0.264788511	0.990740741	0.424248228	0.996296296	0.509705564	0.994444444	0.498800694	0.990740741	0.434746328	0.998148148	0.432080123	0.992592593	0.378151261	0.988888889	0.368154306	1	0.386402587	0.985294118	0.483934319	0.998161765	0.333581257	0.998161765	0.382845946	0.990659056
0.31732827	0.994444444	0.264788511	0.990740741	0.424248228	0.996296296	0.509705564	0.994444444	0.498800694	0.990740741	0.434746328	0.998148148	0.432080123	0.992592593	0.378151261	0.988888889	0.368154306	1	0.386402587	0.985294118	0.483934319	0.998161765	0.333581257	0.998161765	0.382845946	0.990659056


==> Figs/CDF_Data_U.tex <==
Opt-U10-X	Opt-U10-Y	Super-U10-X	Super-U10-Y	Heur-U10-X	Heur-U10-Y	Super-U20-X	Super-U20-Y	Heur-U20-X	Heur-U20-Y
0.00472425	0	0.001267256	0	0.003442222	0	0.000560484	0	0.001934012	0
0.005724487	0.006393862	0.001867657	0.006393862	0.003831858	0.006393862	0.000744556	0.003142678	0.002917068	0.006285355
0.007234356	0.012787724	0.002819482	0.012787724	0.004713185	0.012787724	0.000978149	0.006285355	0.003463803	0.01257071
0.007785554	0.019181586	0.003516759	0.019181586	0.005735239	0.019181586	0.001107636	0.009428033	0.003846781	0.019484601
0.008241216	0.025575448	0.00423945	0.025575448	0.006280656	0.025575448	0.001291521	0.013199246	0.004048843	0.025769956
0.008558123	0.031969309	0.004640288	0.035805627	0.006538939	0.031969309	0.001403774	0.016341923	0.004237979	0.032055311
0.008754928	0.038363171	0.005240156	0.042199488	0.007135444	0.038363171	0.001597921	0.019484601	0.004502944	0.038340666
0.009785905	0.044757033	0.005792324	0.04859335	0.007526309	0.046035806	0.001783847	0.022627278	0.004808025	0.045883092
0.010212901	0.051150895	0.006150093	0.056265985	0.0080457	0.052429668	0.001841452	0.025769956	0.005205656	0.052168448
0.010297687	0.057544757	0.006367858	0.063938619	0.008528785	0.060102302	0.00212162	0.028912634	0.005311046	0.059082338
0.010936444	0.063938619	0.006652888	0.070332481	0.008762179	0.066496164	0.002309083	0.032055311	0.005425143	0.065367693
0.011537531	0.070332481	0.006960016	0.076726343	0.009252555	0.072890026	0.002424896	0.035197989	0.005576723	0.07416719
0.011805829	0.076726343	0.007177832	0.083120205	0.009825122	0.08056266	0.002525566	0.038340666	0.005685968	0.080452546
0.012220477	0.083120205	0.007894489	0.090792839	0.010188978	0.086956522	0.002630021	0.041483344	0.005829421	0.086737901
0.012343228	0.089514066	0.00845083	0.097186701	0.010621095	0.094629156	0.002765391	0.045883092	0.00599238	0.093023256
0.01234403	0.095907928	0.008630871	0.106138107	0.01078561	0.101023018	0.003048741	0.04902577	0.006137532	0.100565682
0.012998808	0.10230179	0.009346945	0.112531969	0.011027504	0.10741688	0.003105488	0.053425519	0.006296086	0.106851037
0.013597405	0.108695652	0.009898281	0.118925831	0.011187222	0.113810742	0.003189707	0.056568196	0.006407256	0.115021999
0.013881435	0.115089514	0.01024326	0.125319693	0.01141671	0.120204604	0.003312426	0.060339409	0.006498279	0.121935889
0.013891632	0.121483376	0.011017783	0.131713555	0.011546445	0.126598465	0.003411921	0.063482087	0.00660744	0.130106851
0.014451345	0.127877238	0.011394564	0.145780051	0.011805916	0.132992327	0.003573964	0.067881835	0.006723558	0.137020742
0.015108229	0.1342711	0.011897314	0.153452685	0.012000519	0.140664962	0.00361019	0.071024513	0.006823692	0.143934632
0.016517276	0.140664962	0.01288969	0.16112532	0.012246886	0.148337596	0.003681969	0.07416719	0.006924883	0.150219987
0.016666666	0.147058824	0.013142728	0.167519182	0.012458737	0.15601023	0.003723968	0.077938404	0.007042254	0.157762414
0.016666667	0.153452685	0.013603244	0.181585678	0.012778192	0.162404092	0.003795009	0.082966688	0.007219759	0.164676304
0.016871326	0.159846547	0.014119109	0.18797954	0.012997305	0.168797954	0.003854347	0.086109365	0.007310924	0.171590195
0.017205688	0.166240409	0.014605288	0.194373402	0.01311449	0.175191816	0.004149686	0.089880578	0.00743349	0.17787555
0.017693163	0.172634271	0.015831561	0.200767263	0.013310617	0.181585678	0.004245164	0.093023256	0.007535014	0.185417976
0.01814497	0.179028133	0.016743355	0.207161125	0.013466502	0.18797954	0.004347683	0.096794469	0.00766241	0.191703331
0.01839348	0.185421995	0.017099233	0.21483376	0.013622211	0.195652174	0.004498614	0.099937146	0.00778974	0.197988686
0.018629656	0.191815857	0.017833023	0.226342711	0.013708162	0.203324808	0.004585664	0.10370836	0.007907425	0.206159648
0.018715088	0.198209719	0.018537313	0.24168798	0.014056036	0.20971867	0.004611633	0.108108108	0.00801956	0.21433061
0.019130352	0.204603581	0.019281054	0.260869565	0.014385667	0.217391304	0.004763852	0.111250786	0.008111174	0.2212445
0.019571812	0.210997442	0.019616626	0.280051151	0.014667168	0.223785166	0.004854637	0.114393463	0.008258355	0.228786926
0.019820163	0.217391304	0.020657398	0.296675192	0.01492723	0.230179028	0.005094197	0.117536141	0.008336216	0.235700817
0.02	0.223785166	0.021435982	0.305626598	0.015059961	0.23657289	0.005196525	0.121307354	0.008509651	0.242614708
0.020150517	0.230179028	0.021745226	0.320971867	0.015318146	0.242966752	0.005279467	0.124450031	0.008604718	0.248900063
0.020174466	0.23657289	0.022500001	0.337595908	0.015452245	0.250639386	0.00553518	0.127592709	0.008717379	0.257071025
0.020497435	0.242966752	0.023201554	0.355498721	0.015524423	0.257033248	0.005606777	0.131363922	0.008851744	0.263984915
0.020814265	0.249360614	0.023446285	0.372122762	0.015929204	0.264705882	0.005751551	0.135135135	0.008958838	0.270898806
0.020837449	0.255754476	0.024337047	0.386189258	0.016076696	0.271099744	0.005863588	0.138277813	0.009090909	0.277812696
0.021008261	0.262148338	0.024742446	0.404092072	0.016244028	0.277493606	0.006092999	0.142049026	0.009185149	0.285355123
0.021500431	0.268542199	0.025208969	0.423273657	0.016552575	0.28516624	0.006146187	0.145820239	0.009285342	0.292269013
0.021580787	0.274936061	0.025844199	0.442455243	0.016628783	0.291560102	0.006287403	0.149591452	0.0094392	0.299182904
0.021772032	0.281329923	0.02682782	0.455242967	0.016839468	0.297953964	0.006367746	0.152734129	0.009560097	0.305468259
0.022116453	0.287723785	0.027800137	0.469309463	0.016961652	0.304347826	0.006504983	0.156505343	0.009672237	0.31238215
0.022396889	0.294117647	0.028412113	0.488491049	0.017109145	0.31202046	0.006592508	0.160276556	0.009777621	0.31929604
0.022396892	0.300511509	0.029952603	0.498721228	0.017319998	0.319693095	0.006747456	0.164676304	0.009910581	0.327467002
0.022500004	0.306905371	0.030721188	0.523017903	0.017516984	0.326086957	0.006828113	0.169076053	0.010045029	0.333752357
0.022835287	0.313299233	0.031427679	0.542199488	0.0176586	0.332480818	0.007241311	0.17221873	0.010161022	0.340666248
0.02306256	0.319693095	0.032101494	0.554987212	0.01794191	0.340153453	0.007600331	0.175361408	0.01027001	0.347580138
0.023074981	0.326086957	0.033085943	0.569053708	0.018124178	0.346547315	0.007752936	0.178504085	0.01038312	0.355122564
0.023138617	0.332480818	0.033861039	0.588235294	0.018228592	0.352941176	0.007853811	0.181646763	0.010480802	0.363293526
0.023214296	0.33887468	0.034246779	0.603580563	0.018584071	0.359335038	0.008232567	0.185417976	0.010602504	0.370207417
0.023292499	0.345268542	0.034760768	0.615089514	0.018701367	0.367007673	0.008271814	0.189189189	0.010730674	0.377121307
0.023405588	0.351662404	0.035281432	0.627877238	0.018961598	0.373401535	0.008400658	0.193588938	0.010800386	0.387806411
0.02356368	0.358056266	0.03563557	0.645780051	0.019147372	0.379795396	0.008684738	0.197360151	0.010907825	0.395348837
0.024810005	0.364450128	0.036345432	0.659846547	0.019276445	0.386189258	0.008952177	0.205531113	0.010972701	0.403519799
0.024999966	0.37084399	0.036807666	0.672634271	0.019619113	0.39258312	0.009233862	0.20867379	0.011060692	0.409805154
0.025	0.377237852	0.038012248	0.685421995	0.01975087	0.400255754	0.009282256	0.211816468	0.011177347	0.416090509
0.025000011	0.383631714	0.038506294	0.696930946	0.020078936	0.406649616	0.009541401	0.214959145	0.011239288	0.4230044
0.025000083	0.390025575	0.03945266	0.71483376	0.020355711	0.413043478	0.009903698	0.228158391	0.011316527	0.42991829
0.025557421	0.396419437	0.040408273	0.730179028	0.020592526	0.420716113	0.010185818	0.231301069	0.011404087	0.438089252
0.025641646	0.402813299	0.042383724	0.74168798	0.020766937	0.427109974	0.010367554	0.234443746	0.011512605	0.444374607
0.025737219	0.409207161	0.043202043	0.757033248	0.021014543	0.433503836	0.010663498	0.245757385	0.011610194	0.450659962
0.026135717	0.415601023	0.044095877	0.771099744	0.021296986	0.441176471	0.010853989	0.259585167	0.011719026	0.456945317
0.02654568	0.421994885	0.044862855	0.782608696	0.021407235	0.447570332	0.011010345	0.262727844	0.011913511	0.465116279
0.026897517	0.428388747	0.046167647	0.799232737	0.021567351	0.453964194	0.011460354	0.277812696	0.012032932	0.473287241
0.027017447	0.434782609	0.047563539	0.81202046	0.02173913	0.460358056	0.01199703	0.294783155	0.012102243	0.479572596
0.027207408	0.441176471	0.049250556	0.822250639	0.02189781	0.468030691	0.012265541	0.303582652	0.012240896	0.486486486
0.027371922	0.447570332	0.05	0.833759591	0.022079861	0.474424552	0.012596432	0.320553111	0.012415622	0.493400377
0.027783264	0.453964194	0.051254051	0.841432225	0.022206131	0.482097187	0.012823455	0.33186675	0.012571727	0.500942803
0.028594169	0.460358056	0.053596891	0.847826087	0.022381477	0.488491049	0.012986231	0.344437461	0.012742176	0.507228158
0.02875003	0.466751918	0.057483982	0.854219949	0.022545404	0.496163683	0.013183566	0.355122564	0.012889029	0.514770585
0.028810548	0.47314578	0.059005321	0.861892583	0.022722918	0.502557545	0.013670963	0.362036455	0.013013517	0.52105594
0.029230252	0.479539642	0.062713554	0.869565217	0.023000745	0.508951407	0.013981685	0.373350094	0.013178831	0.527341295
0.029585099	0.485933504	0.065637533	0.879795396	0.023066711	0.515345269	0.01441385	0.388434947	0.01340405	0.534883721
0.029835954	0.492327366	0.06988952	0.886189258	0.023300048	0.52173913	0.014642956	0.39912005	0.013543599	0.542426147
0.030286123	0.498721228	0.071541383	0.893861893	0.023474792	0.528132992	0.015014939	0.41734758	0.013586397	0.549340038
0.030472016	0.50511509	0.073112815	0.901534527	0.023730501	0.534526854	0.015388367	0.433689503	0.013732394	0.556882464
0.030738149	0.511508951	0.074227337	0.907928389	0.02395911	0.542199488	0.015601892	0.446888749	0.013887531	0.56442489
0.030766642	0.517902813	0.076024495	0.914322251	0.02417208	0.54859335	0.015892986	0.458202388	0.014054966	0.571338781
0.030927062	0.524296675	0.077861223	0.925831202	0.024449196	0.554987212	0.016196289	0.470773099	0.014232489	0.578881207
0.031163027	0.530690537	0.07921361	0.932225064	0.025058082	0.561381074	0.016480122	0.48460088	0.014439519	0.587680704
0.031163027	0.537084399	0.080816546	0.941176471	0.025211319	0.567774936	0.016939138	0.49717159	0.014577425	0.593966059
0.03120745	0.543478261	0.082141128	0.952685422	0.025505329	0.574168798	0.017199967	0.512256442	0.014692844	0.600251414
0.031432268	0.549872123	0.084767448	0.959079284	0.025747823	0.58056266	0.017569391	0.526712759	0.014843548	0.606536769
0.031590215	0.556265985	0.088722072	0.969309463	0.025914782	0.586956522	0.017911786	0.539912005	0.014977645	0.61345066
0.032055269	0.562659847	0.090660332	0.97826087	0.026094953	0.593350384	0.018280659	0.552482715	0.01521377	0.619736015
0.032291256	0.569053708	0.096292807	0.985933504	0.026401413	0.599744246	0.01846104	0.565681961	0.015406162	0.627906977
0.032701205	0.57544757	0.1	0.998721228	0.026806817	0.60741688	0.018693812	0.5769956	0.015584833	0.635449403
0.03333302	0.581841432	0.1	0.998721228	0.027068402	0.616368286	0.019165745	0.588937775	0.01570773	0.642991829
0.033333333	0.588235294	0.1	0.998721228	0.027374451	0.622762148	0.019334144	0.598994343	0.015825298	0.64990572
0.033333333	0.594629156	0.1	0.998721228	0.027606329	0.630434783	0.019583166	0.608422376	0.015994398	0.65681961
0.033595334	0.601023018	0.1	0.998721228	0.027688981	0.636828645	0.020353339	0.619736015	0.016079812	0.665619107
0.033835993	0.60741688	0.1	0.998721228	0.028504096	0.643222506	0.020523616	0.627278441	0.01627543	0.672532998
0.033905506	0.613810742	0.1	0.998721228	0.028877601	0.649616368	0.02089096	0.637335009	0.016414566	0.680075424
0.034084328	0.620204604	0.1	0.998721228	0.029190295	0.65601023	0.021428515	0.646763042	0.016554889	0.686360779
0.034198306	0.626598465	0.1	0.998721228	0.029640197	0.662404092	0.021741211	0.655562539	0.016644693	0.692646135
0.034914462	0.632992327	0.1	0.998721228	0.030332287	0.668797954	0.021844117	0.667504714	0.016909621	0.699560025
0.035383776	0.639386189	0.1	0.998721228	0.031120944	0.676470588	0.022128587	0.676932747	0.017056758	0.707102451
0.035532512	0.645780051	0.1	0.998721228	0.03145223	0.68286445	0.022583615	0.688246386	0.017156693	0.713387806
0.035885159	0.652173913	0.1	0.998721228	0.031996015	0.689258312	0.022903345	0.69893149	0.017289424	0.719673162
0.036242831	0.658567775	0.1	0.998721228	0.03259587	0.695652174	0.023429635	0.70584538	0.017507942	0.726587052
0.036745823	0.664961637	0.1	0.998721228	0.033038348	0.705882353	0.023972111	0.715273413	0.01775503	0.732872407
0.036954652	0.671355499	0.1	0.998721228	0.033485393	0.71483376	0.024260531	0.724701446	0.017898458	0.739157762
0.038058811	0.677749361	0.1	0.998721228	0.033800301	0.721227621	0.02461229	0.732872407	0.018083008	0.747328724
0.03821816	0.684143223	0.1	0.998721228	0.033990659	0.727621483	0.024834054	0.744186047	0.018394407	0.754242615
0.038455982	0.690537084	0.1	0.998721228	0.034315245	0.734015345	0.024932769	0.754242615	0.018999367	0.76052797
0.038564361	0.696930946	0.1	0.998721228	0.034660767	0.74168798	0.025237404	0.763670647	0.019343452	0.768070396
0.039376941	0.703324808	0.1	0.998721228	0.035386045	0.748081841	0.025647278	0.771841609	0.019553599	0.776241358
0.039832382	0.70971867	0.1	0.998721228	0.035879511	0.754475703	0.025982217	0.783155248	0.019986145	0.782526713
0.040257112	0.716112532	0.1	0.998721228	0.036537468	0.760869565	0.026403718	0.791954745	0.020187793	0.789440603
0.041272369	0.722506394	0.1	0.998721228	0.037169023	0.767263427	0.026649149	0.801382778	0.020500522	0.795725959
0.041293666	0.728900256	0.1	0.998721228	0.037726098	0.773657289	0.02690618	0.808925204	0.020687872	0.802639849
0.041951745	0.735294118	0.1	0.998721228	0.038645132	0.781329923	0.027452191	0.817724701	0.020938897	0.808925204
0.042489476	0.74168798	0.1	0.998721228	0.038823644	0.789002558	0.028009693	0.82212445	0.021428848	0.815210559
0.043167796	0.748081841	0.1	0.998721228	0.039360529	0.796675192	0.028303418	0.832181018	0.021724334	0.821495915
0.043767559	0.754475703	0.1	0.998721228	0.040342845	0.803069054	0.028811505	0.840980515	0.022108774	0.828409805
0.04411368	0.760869565	0.1	0.998721228	0.041225455	0.810741688	0.029767196	0.848522942	0.0224497	0.835952231
0.044232906	0.767263427	0.1	0.998721228	0.041960837	0.81713555	0.030043759	0.856065368	0.022987229	0.842237586
0.044444432	0.773657289	0.1	0.998721228	0.042231621	0.823529412	0.030670132	0.863607794	0.02331244	0.848522942
0.044730115	0.780051151	0.1	0.998721228	0.042955129	0.829923274	0.031733661	0.87115022	0.023845007	0.856693903
0.045099843	0.786445013	0.1	0.998721228	0.043552337	0.836317136	0.032742707	0.878692646	0.024143351	0.864236329
0.045256776	0.792838875	0.1	0.998721228	0.044082687	0.842710997	0.032985386	0.884978001	0.024509804	0.871778755
0.045687346	0.799232737	0.1	0.998721228	0.045043126	0.849104859	0.033552436	0.891263356	0.024807136	0.878064111
0.04615634	0.805626598	0.1	0.998721228	0.045529716	0.856777494	0.034029704	0.897548712	0.02518083	0.884349466
0.046428592	0.81202046	0.1	0.998721228	0.046071749	0.863171355	0.03441581	0.904462602	0.025803036	0.890634821
0.04674454	0.818414322	0.1	0.998721228	0.04706634	0.869565217	0.034794309	0.910747957	0.026056338	0.896920176
0.048532366	0.824808184	0.1	0.998721228	0.049453162	0.875959079	0.035566341	0.916404777	0.026983027	0.903834067
0.049999998	0.831202046	0.1	0.998721228	0.050807559	0.884910486	0.036470558	0.922690132	0.027982861	0.910119422
0.05	0.837595908	0.1	0.998721228	0.052390623	0.891304348	0.037213526	0.928975487	0.028642481	0.916404777
0.05	0.84398977	0.1	0.998721228	0.052988752	0.89769821	0.03833149	0.935260842	0.030551416	0.922690132
0.052419856	0.850383632	0.1	0.998721228	0.055667664	0.906649616	0.039662863	0.942803268	0.032452713	0.928975487
0.056774394	0.856777494	0.1	0.998721228	0.057400965	0.914322251	0.040461192	0.947831552	0.033074479	0.937146449
0.06062302	0.863171355	0.1	0.998721228	0.061395349	0.923273657	0.041597937	0.954116908	0.033759023	0.943431804
0.065588326	0.869565217	0.1	0.998721228	0.064048525	0.933503836	0.044087514	0.959773727	0.034542385	0.949717159
0.068396609	0.875959079	0.1	0.998721228	0.066363976	0.941176471	0.044756918	0.965430547	0.035465484	0.956002514
0.069527984	0.882352941	0.1	0.998721228	0.068679981	0.950127877	0.048211857	0.96920176	0.037357316	0.962287869
0.071065031	0.89258312	0.1	0.998721228	0.070071672	0.959079284	0.05533779	0.972972973	0.03846401	0.968573224
0.07450421	0.900255754	0.1	0.998721228	0.074834991	0.968030691	0.060460199	0.976115651	0.039683586	0.97485858
0.077114693	0.906649616	0.1	0.998721228	0.078689202	0.976982097	0.062197449	0.979258328	0.041335584	0.981143935
0.079280672	0.914322251	0.1	0.998721228	0.084417494	0.988491049	0.065406531	0.982401006	0.049444119	0.988686361
0.080697865	0.920716113	0.1	0.998721228	0.092175644	0.997442455	0.066994396	0.985543683	0.054755784	0.995600251
0.081408161	0.927109974	0.1	0.998721228	0.092175644	0.997442455	0.071350968	0.988686361	0.054755784	0.995600251
0.08344585	0.938618926	0.1	0.998721228	0.092175644	0.997442455	0.075552489	0.991829038	0.054755784	0.995600251
0.086323147	0.945012788	0.1	0.998721228	0.092175644	0.997442455	0.079391738	0.994971716	0.054755784	0.995600251
0.087690757	0.955242967	0.1	0.998721228	0.092175644	0.997442455	0.090465105	0.998114393	0.054755784	0.995600251
0.088465813	0.962915601	0.1	0.998721228	0.092175644	0.997442455	0.090465105	0.998114393	0.054755784	0.995600251
0.090000018	0.974424552	0.1	0.998721228	0.092175644	0.997442455	0.090465105	0.998114393	0.054755784	0.995600251
0.09348908	0.982097187	0.1	0.998721228	0.092175644	0.997442455	0.090465105	0.998114393	0.054755784	0.995600251
0.1	0.993606138	0.1	0.998721228	0.092175644	0.997442455	0.090465105	0.998114393	0.054755784	0.995600251


==> Figs/CDF_Plot_L.tex <==
\begin{figure}[t]
    \centering
    \resizebox{0.75\columnwidth}{!}{%
    
    \begin{tikzpicture}

    \begin{axis}
    [
    % put axis lines at left and bottom
    axis lines = left,
    % control axis labels
    xlabel = \smaller {Rate=Delivered chunks per time},
    ylabel = \smaller {CDF},
    ylabel near ticks,
    % control legend position
    legend pos = south east,
    % control size of tick marks (10,20,30,etc)
    ticklabel style={font=\smaller},
    % control major grids
    grid=both,
    major grid style={line width=.2pt,draw=gray!30},
    % control minor grids
    %grid style={line width=.1pt, draw=gray!10},
    %minor tick num=5,
    ]
    
    % \addplot[black]
    % table[y=Opt-L1-Y,x=Opt-L1-X]{Figs/CDF_data_L.tex};
    % \addlegendentry{\smaller $L=1$, Analytical}
    % \addplot[black,dashed]
    % table[y=Super-L1-Y,x=Super-L1-X]{Figs/CDF_data_L.tex};
    % \addlegendentry{\smaller $L=1$, Super-user}
    % \addplot[black!50]
    % table[y=Heur-L1-Y,x=Heur-L1-X]{Figs/CDF_data_L.tex};
    % \addlegendentry{\smaller $L=1$, RGA}
    
    % \addplot[green]
    % table[y=Opt-L5-Y,x=Opt-L5-X]{Figs/CDF_data_L.tex};
    % \addlegendentry{\smaller $L=5$, Analytical}
    % \addplot[green,dashed]
    % table[y=Super-L5-Y,x=Super-L5-X]{Figs/CDF_data_L.tex};
    % \addlegendentry{\smaller $L=5$, Super-user}
    % \addplot[green!50]
    % table[y=Heur-L5-Y,x=Heur-L5-X]{Figs/CDF_data_L.tex};
    % \addlegendentry{\smaller $L=5$, RGA}
    
    \addplot[black]
    table[y=Opt-L1-Y,x=Opt-L1-X]{Figs/CDF_data_L.tex};
    \addlegendentry{\smaller $L=1$}
    \addplot[blue]
    table[y=Opt-L5-Y,x=Opt-L5-X]{Figs/CDF_data_L.tex};
    \addlegendentry{\smaller $L=5$}
    \addplot[green]
    table[y=Opt-L10-Y,x=Opt-L10-X]{Figs/CDF_data_L.tex};
    \addlegendentry{\smaller $L=10$}
    \addplot[red]
    table[y=Opt-L15-Y,x=Opt-L15-X]{Figs/CDF_data_L.tex};
    \addlegendentry{\smaller $L=15$}
    \addplot[gray]
    table[y=Opt-L20-Y,x=Opt-L20-X]{Figs/CDF_data_L.tex};
    \addlegendentry{\smaller $L=20$}
    

    \end{axis}

    \end{tikzpicture}
    }
    \caption{CDF for changing $L$, $U=10$, analytical solution, $\frac{M}{N} = 0.2$, Time is calculated assuming a full video chunk can be transmitted in one second.}
    \label{fig:cdf_l}
\end{figure}


==> Figs/CDF_Plot_U.tex <==
\begin{figure}[t]
    \centering
    \resizebox{0.75\columnwidth}{!}{%
    
    \begin{tikzpicture}

    \begin{axis}
    [
    % put axis lines at left and bottom
    axis lines = left,
    % control axis labels
    xlabel = \smaller {Rate= Delivered chunks per unit time of a codeword},
    ylabel = \smaller {CDF},
    ylabel near ticks,
    xticklabel style={
            /pgf/number format/fixed,
            /pgf/number format/precision=2
            %/pgf/number format/fixed zerofill
        },
        scaled x ticks=false,
    % control legend position
    legend pos = south east,
    % control size of tick marks (10,20,30,etc)
    ticklabel style={font=\smaller},
    % control major grids
    grid=both,
    major grid style={line width=.2pt,draw=gray!30},
    % control minor grids
    %grid style={line width=.1pt, draw=gray!10},
    %minor tick num=5,
    ]
    
    \addplot[black]
    table[y=Opt-U10-Y,x=Opt-U10-X]{Figs/CDF_data_U.tex};
    \addlegendentry{\smaller $U=10$, Analytical}
    
    \addplot[gray]
    table[y=Super-U10-Y,x=Super-U10-X]{Figs/CDF_data_U.tex};
    \addlegendentry{\smaller $U=10$, Super-user}
    
    \addplot[blue]
    table[y=Heur-U10-Y,x=Heur-U10-X]{Figs/CDF_data_U.tex};
    \addlegendentry{\smaller $U=10$, RGA}

    \addplot[green]
    table[y=Super-U20-Y,x=Super-U20-X]{Figs/CDF_data_U.tex};
    \addlegendentry{\smaller $U=20$, Super-user}
    
    \addplot[red]
    table[y=Heur-U20-Y,x=Heur-U20-X]{Figs/CDF_data_U.tex};
    \addlegendentry{\smaller $U=20$, RGA}
    

    \end{axis}

    \end{tikzpicture}
    }
    \caption{CDF for changing $U$, $L=5$, $\frac{M}{N}$ = 0.2.}
    \label{fig:cdf_u}
\end{figure}


==> KaganAlgorithm.tex <==
In this section, we provide a novel scheduling algorithm which we call \emph{Random Greedy Association (RGA)} to find a sub-optimal solution to the optimization problem~\eqref{eq:optimization_problem_main}. The proposed algorithm has low computational overhead and is applicable to large-scale networks with multiple helpers. Moreover, due to its underlying scheduling structure, it is applicable to dynamic network conditions where the users can move (and join/leave the network) freely or start/stop video streaming at any time.

The pseudo-code of the proposed greedy scheduling solver is provided in Algorithm~\ref{alg:main_body}, and its two auxiliary procedures $\textsc{AssignUsers}$ and $\textsc{AssignHelpers}$ are detailed in Algorithms~\ref{alg:assign_users} and~\ref{alg:assign_helpers}, respectively (c.f the appendix). 
%We have used new notations to denote the variables in the pseudo-code. 
The description of new notations and their possible initial values (assigned with the $\textsc{Initialize}$ step at the beginning of Algorithm~\ref{alg:main_body}), are as follows:
\begin{itemize}
    \item $\Bh_{\mathrm{on}}$ and $\Bh_{\mathrm{off}}$ include active and non-active helpers, respectively. $\Bh_{\mathrm{new}}$ also includes active helpers, but only the ones activated recently. Initially, all helpers are inactive;
    \item $\Sfv(u_k)$ denotes the number of chunks served to user $u_k$ and is initialized to zero. $v_{\mathrm{limit}}$ is a control parameter: the algorithm stops when the number of chunks received by every user exceeds $v_{\mathrm{limit}}$;
    \item $\Bd $ denotes the \emph{degree vector}. Defining the degree of user $u_k$, denoted as $\Sfd(u_k)$, as the number of helpers $h_i$ for which $|\Sfx(h_i)-\Sfx(u_k)| \le r_{\mathrm{inter}}$, $\Bd[s]$ corresponds to $s$-th smallest degree $\Sfd(u_k)$ for all $k\in{[K]}$;
    %, and $\Sfd(u_k)$ is the degree of user $u_k$, defined as the number of helpers $h_i$ for which $|\Sfx(h_i)-\Sfx(u_k)| \le r_{\mathrm{inter}}$;
    \item $\Bm_i$, $i \in [H]$, is a vector of size $L$, initialized to zero. $\Bm_i[l] = u_k$ only if helper $h_i$ is serving $u_k$ and $\SfL(u_k) = l$. Otherwise, it is zero. %of users $u_k$ that are supposed to receive data from helper $h_i$. $\Bn_i$ is initially empty. Also, at any time, the users in every $\Bn_i$ should be assigned to distinct cache profiles;
    \item Auxiliary variables $\Sft(h_i)$ represent the amount of time helper $h_i$ requires to serve users in $\Bm_i$. Also, $T$ is the total delivery time, initially set to zero;
    \item Auxiliary vector $\Bu_{\mathrm{cnd}}$, initially empty, is a placeholder for candid users to be served by the algorithm.
    % = [\Sfd(u_1),\Sfd(u_2),\cdots,\Sfd(u_K)]
    \end{itemize}
We have also used two auxiliary functions: $\textsc{Shuffle}(\Bv)$ randomly shuffles the order of data in $\Bv$, and $\textsc{Connect}(h_i,u_k)$ returns one only if $u_k$ is within radius $r_{\mathrm{trans}}$ of $h_i$ and outside of radius $r_{\mathrm{inter}}$ of every active helper in the network (other than --possibly-- $h_i$ itself), and zero otherwise. Finally, we have used a special notation in line 3 of Algorithm~\ref{alg:assign_helpers}: $[\Bm_{(i)}]$ denotes the set of all users $u_k$ that are receiving data from some helper.

As a brief explanation, at every iteration, the algorithm first checks if inactive helpers can be made active without causing interference to the active ones ($\textsc{AssignHelpers}$ script), and if that's possible, tries to maximize the number of users assigned to such recently activated helpers ($\textsc{AssignUsers}$ script). In both checks, users are filtered based on their degree values $\Sfd(\cdot)$, and it is ensured that every active helper serves at most one user assigned to every cache profile. A new iteration starts after at least one of the active helpers finishes delivering video chunks, and it is assumed that the helpers that do not finish delivery remain active in the new iteration.\footnote{This is an important practical consideration as without that, we may need to further split subpackets into arbitrary smaller parts.} The algorithm runs as long as a minimum number of chunks are delivered to every user.
It should be noted that we shuffle various vectors repeatedly during the algorithm runtime to avoid stalling. An example of stalling possibility without shuffling is provided in Example~\ref{exmp:stalling} (c.f appendix).

%\todo[inline]{From this part, the text is not revised.}

%\begin{itemize}
    %\item What's the main role of the heuristic algorithm? It provides good performance, with a purely algorithmic and implementable approach, and can handle dynamic network conditions and a finite number of user requests.
    %\item What are the steps? 1. Initializing the variables, 2. searching for new users to be serviced by currently active helpers, 3. searching for new helpers to be activated without causing interference on currently active users, 4. updating the delivery times.
    %\item We also shuffle some arrays during the algorithm runtime. The goal is to avoid stalling. We can put an example of stalling in the footnote.
%\end{itemize}



%\todo[inline]{Here starts Kagan's text}

%let $\delta(G)=\max_{u_k\in{\CU}}d(u_k)$ be the maximum number of edges adjacent to a user and let $\theta(G)=\min_{u_k\in{\CU}}d(u_k)$ be the minimum number of edges adjacent to a user. We assume that the graph $G$ is finite, in real life we have finite number of users and helpers, so $\delta(G)$ is a positive integer. 

%For a vector $\Bx$, let $g:\Bx\rightarrow\Bx$ be a random permutation on the ordering of the elements of the vector $\Bx$. 

%Let $\CH_{ad}$ denote the set of activated helpers and $\CH_{ia}$ denote the set of inactive helpers and $\CU$ denote the set of users. We order the helpers in $\CH_{ia}$ and the users in $\CU$ in any order we would like and put them in vectors $\Bh^{ia}$ and $\Bu$ respectively. Also let $\Bd$ be the degree vector where  $\Bd=[\theta(G),\theta(G)+1,\theta(G)+2,...,\delta(G)]$(We may not have the intermediate degrees I will fix this later). Let $\Bh^{ad}$ denote the vector of activated helpers. At first, $\CH_{ad}=\emptyset$ and $\Bh^{ad}$ is empty. $\Bu^{ct}$ is the vector which consists of candidate users and initially it is empty. Let $\Bv(h)$ denote the delivery column vector of helper $h$ where $\Bv_l(h)$ corresponds to a user $u_k$ which is in cache group $l$ and at $l$th row of $\Bv(h)$. Let $c(u_k)$ denote the cache group of user $u_k$. Let $t(\Bv(h))$ be the serving time of the delivery column of helper $h$ and let $f(u_k)$ denote the total files served by the algorithm to user $u_k$. Initially $f(u_k)=0$ $\forall{u_k}\in\CU$. Let $\Br$ denote the vector of average rates of the users where $\Br_k$ corresponds to the average rate of user $u_k\in{\CU}$.

%Let $T$ denote the total time of the algorithm and $V$ be the minimum video chunks or files that a user need to be served to evaluate the performance of the algorithm.

%\todo[inline]{this part is Mohammad's explanations}
%In the beginning, mention that the algorithm is provided in ...

%The Random Greedy Association Algorithm repeatedly serves the user requests until a minimum number of served files is reached. In line 1 $V$, the minimum files need to be served is set. 

%The algorithm searches the users to attach to helpers by looking at the degrees one by one, and for a fixed degree it looks at which helper it can attach users also one by one. In line 2 of the algorithm the order of the inactive helpers and order of the degrees are randomly shuffled, the rationale behind this is to be more fair to the users. Also since the algorithm searches for users to attach to helpers by looking at the helpers one by one and since the users which can be served by a helper may differ from helper to helper, activating a helper may prevent another helper from activating which in turn may prevent some users to be served at all and randomly shuffling the order of the helpers prevents this. (For instance, we have 3 helpers and first helper and second helper has a user in their transmission radius which can just be served by both and similarly first and third helper has a user in their transmission which can just be served by both. These users have different cache. Also second and third helper has a user in their transmission radius which can just be served by both. There are other users with degree 1. If degree we are looking for is 1, we can activate all helpers because the users have degree 1, then we can't serve any users with degree 2 because they are all interfered by at least another helper. If we start the search from degree 2 first helper serves the two users with degree 2 which have different caches, but then we still can't activate helper 2 or 3 and the third user with degree 2 can not be served. So whatever degree ordering we have we can't serve all users)  The order of the degrees of the users is also randomly shuffled not to prioritize some users over others. (For instance assume that three different users have the same cache but two of them have degree 1 and can be served by two different helpers and the third user have degree 2 and can be just served by these two helpers. So whatever helper ordering we have if we start from degree 1 to attach users we can not definitely serve the third user.) Simulations also show that shuffling the helper and degree orders are both necessary to be able to serve all users in the system, otherwise depending on the topology some users may not even receive a single file.

%In line 3 the 'search'(Lines 3-26) for finding users and attaching to helpers start. We start from the first degree. Lines 4-13 corresponds to attaching users to 'activated' helpers where an 'activated' helper corresponds to a helper which was inactive before the search was initiated but activated during the search. Lines 14-26 corresponds to activating inactive helpers and attaching users to them. Attaching users to activated helpers precedes activating new helpers since activating a helper automatically increases the interference on the unserved users which are waiting to be served and we would like to attach many users as possible before increasing interference. In line 7 the candidate users which can be attached to the active helper are found. A user can be considered as a candidate user if it has the degree that we are looking for, it is in the transmission radius of the helper which we want to attach to  and it is not interfered by any other active helper. In Line 9 the order of the candidate users are also shuffled to be fair to the users with same caches, otherwise some users would be prioritized and some may not be even served one single packet which the simulations also show us. For instance for the users with degree 1 and same cache, without shuffling just one of them can be served since they can all be served by a single helper. In lines 11-12 we put the candidate user in the delivery column of the helper if the helper doesn't have another user with the same cache in its delivery column. In line 15 before looking for users to attach and activate a helper we check if the helpers is interfering with the active users which are being served, i.e the users in the delivery columns. If there is interference, we can't activate this helper. Other than this, lines 16-23 for attaching users to inactive helpers are similar as in lines 6-13 for attaching user to activated helpers. In 24-26 if users are attached to the inactive helper we say that this helper is activated and also active. In line 28 we calculate the delivery times of the activated helpers and then since the search is finished in line 29 we reset the activated helpers. In lines 30-37 we calculate the minimum time left to serve the users in all delivery columns, we update the times with respect to first finishing columns, we say that helpers which served their users are inactive now and update the number of files the users served in the first finishing delivery columns and erase the users from the finished columns. In 38 we calculate the total time of the algorithm. After the minimum number of served files $V$ for all users is achieved, in line 40 we calculate the average rate of the users by dividing the total number of files served by total time of the algorithm for each user and in line 41 we return the rate vector of the users.

% \begin{algorithm}
% \caption{Random Greedy Association}
% \begin{algorithmic}[1]
% \While{$\min_{u_k\in{\CU}}f(u_k)<V$}
% \State $\Bh^{ia} \gets g(\Bh^{ia})$ and $\Bd \gets g(\Bd)$ 
% \For{$j=1:|\Bd|$}
%  \If{$\Bh^{ad}$ is not empty}
%   \For{$i=1:|\Bh^{ad}|$}
%    \For{$k=1:|\Bu|$}
%     \If{$d(\Bu_k)=j$, $\Bh^{ad}_i\Bu_k\in{\CE_t}$ and $\nexists{}h\in{\CH_{a}},h\neq{\Bh^{ad}_i}$ s.t. $h\Bu_k\in{\CE}$}
%      \State $\Bu^{ct} \gets [\Bu^{ct},\Bu_k]$
%     \EndIf
%    \EndFor
%    \State $\Bu^{ct} \gets g(\Bu^{ct})$
%    \For{$k=1:|\Bu^{ct}|$}
%      \If{$l:=c(\Bu^{ct}_k)$th row of $\Bv(\Bh_{\mathrm{off}}^{ad})$ is empty}
%        \State $\Bv_{l}(\Bh_{\mathrm{off}}^{ad}) \gets \Bu^{ct}_k$
%      \EndIf
%    \EndFor
%    \State $\Bu^{ct} \gets$ [ ]  
%   \EndFor
%  \EndIf
%  \For{$i=1:|\Bh^{ia}|$}
%   \If{$\nexists{u_k}\in{\Bv(h)}$, $h\in{\CH}$ s.t. $\Bh^{ia}_iu_k\in{\CE}$}
%    \For{$k=1:|\Bu|$}
%     \If{$d(\Bu_k)=j$, $\Bh^{ia}_i\Bu_k\in{\CE_t}$ and $\nexists{}h\in{\CH_{a}}$ s.t. $h\Bu_k\in{\CE}$}
%      \State $\Bu^{ct} \gets [\Bu^{ct},\Bu_k]$    
%     \EndIf
%    \EndFor
%    \State $\Bu^{ct} \gets g(\Bu^{ct})$
%    \For{$k=1:|\Bu^{ct}|$}
%      \If{$l:=c(\Bu^{ct}_k)$th row of $\Bv(\Bh_{\mathrm{off}}^{ia})$ is empty}
%        \State $\Bv_{l}(\Bh_{\mathrm{off}}^{ia}) \gets \Bu^{ct}_k$
%      \EndIf
%    \EndFor
%     \State $\Bu^{ct} \gets$ [ ]   
%   \EndIf
%   \If{$\Bv(\Bh_{\mathrm{off}}^{ia})$ is not empty}
%    \State $\CH_a \gets \CH_a\cup{}\Bh_{\mathrm{off}}^{ia}$
%    \State $\Bh^{ad} \gets [\Bh^{ad},\Bh_{\mathrm{off}}^{ia}]$ and erase $\Bh_{\mathrm{off}}^{ia}$ from $\Bh^{ia}$
%   \EndIf
%  \EndFor
% \EndFor
% \ForAll{$h$ in $\Bh^{ad}$}
%   \State $t(\Bv(h)) \gets \binom{L}{\gamma+1}-\binom{L-|\Bv(h)|}{\gamma+1}$
% \EndFor
% \State $\Bh^{ad} \gets$ [ ]
% \State $m \gets \min_{h\in{\CH_a}}t(\Bv(h))$
% \ForAll{$h\in{\CH_a}$}
%   \State $t(\Bv(h)) \gets t(\Bv(h))-m $
%   \If{$t(\Bv(h))=0$}
%     \State $\CH_a \gets \CH_a\backslash{h}$ and $\Bh^{ia} \gets [\Bh^{ia},h]$
%     \ForAll{$u_k\in{\Bv(h)}$}
%       \State $f(u_k) \gets f(u_k)+1$  
%     \EndFor
%     \State $\Bv(h) \gets$ []
%   \EndIf
% \EndFor
% \State $T \gets T+m$
% \EndWhile
% \ForAll{$u_k\in{\CU}$}
%   \State $\Br_k \gets f(u_k)/T$
% \EndFor
% \State \Return $\Br$
% \end{algorithmic}
% \end{algorithm}


==> old_SimResults.tex <==
%Comment from Giuseppe:
%Generally speaking, for networks of moderate size .. we would like to show that

%a) restiricting the maximal vectors to the vectors that maximize the multiplexing gain yields no %loss of optimality … IF WE CANNOT PROVE THIS … IT SHOULD BE AT LEAST OBSERVED EXPERIMENTALLY

%b) using the super-user restriction yields generally a small loss

%c) for networks of larger size, we can compare the heuristic approach with the optimization %approach, where the optimization approach can be restricted to the superuser case for %tractability … and yet show that the heuristic approach is ``quite good’’. 

\input{Figs/CDF_Plot_L.tex}
\input{Figs/CDF_Plot_U.tex}

We use numerical results to compare the performance of various solutions. We assume $H$ helpers are located at the center of hexagons on a limited hexagonal grid. Every hexagon has a radius of~$1$, and we have $r_{\mathrm{trans}} = 1$ and $r_{\mathrm{inter}}  =1.2$. The users are placed according to a homogeneous Poisson Point Process in the transmission area of helpers. The average number of users per helper, shown by $U$, is determined by the density of the Poisson process. Every user is randomly assigned with a cache profile $l \in [L]$.

In Tables~\ref{tab:utiliy_u} and~\ref{tab:utiliy_l}, we have compared the utility function value of the analytical (Section~\ref{section:analytical_solution}), super-user (Section~\ref{section:super-user}), and RGA (Section~\ref{section:kagan_solution}) solutions, for different values of $U$ and $L$, respectively. For the analytical solution, we have limited $\mathrm{Conv}(\Br(j,s_j))$ to maximal rate vectors that also maximize the coded caching gain, as the more general case is intractable even for small networks due to its complexity (even with the restriction, we cannot simulate large networks as is visible in the table).\footnote{Of course, for very small networks, we get the same solution with and without the proposed restriction of the throughput region. However, as discussed, proving the optimality for this subset of rate vectors is challenging for the general case.} From the tables, we can see that:
\begin{itemize}
    \item both RGA and super-user solutions perform well; for small networks, their performance is quite close to the analytical solution. Moreover, in all cases, RGA performs at most $10\%$ worse than the super-user method;
    \item system performance gets worse as $U$ is increased. This is expected, as with more users, the portion of resources allocated to each user becomes more limited;
    \item system performance improves as $L$ is increased ($L=1$ corresponds to the uncoded caching scheme). This is due to the increased multicasting opportunities as $L$ grows;
    \item As $L$ keeps growing, the utility function converges to a certain value irrespective of the selected solver. This is because $U$ is fixed, and hence, the multicasting opportunities are limited even if $L$ gets very large. 
    %This behavior is also verified in the CDF plot of Figure~\ref{fig:cdf_l}.
    %since we increase our multicast opportunities where $L=1$ corresponds to the uncoded caching scheme. However as $L$ increases all of the algorithms converge to a certain utility value because $U$ is fixed and we can't achieve more by increasing the subpacketization order when there are no users to take advantage of it where the convergence of CDF can be seen for the analytical solution directly from Figure \ref{fig:cdf_l}.
\end{itemize}

In Figure~\ref{fig:cdf_l}, we have extended the comparisons by plotting the CDF of the achievable rate (in terms of delivered chunks per time) of all users, for the analytical solver and for $L \in \{1,5,10,15,20\}$. 
Similarly, in Figure~\ref{fig:cdf_u}, we have plotted the CDF of the achievable rates (in terms of the number of delivered chunks) of all users, for different solvers and for $U \in \{10,20\}$.
These CDF plots essentially confirm the observations made by Tables~\ref{tab:utiliy_u} and~\ref{tab:utiliy_l}: the heuristic algorithms perform well, and the rate values converge as $L$ keeps getting larger.

%As CDF increases, the difference between CDF of super-user and analytical solutions becomes negligible. However in all the cases RGA outperforms super-user solution for the smaller rates, i.e. for the slowest users. So if the slowest users (users with a bad channel) are a high priority, RGA can be used for bigger networks and optimal solution is not feasible. 

%Note that time is calculated in Figure \ref{fig:cdf_l} by assuming that a full video chunk can be transmitted in 1 seconds or unit time so a codeword can be transmitted in $1/\binom{L}{t}$ seconds. In Figures~\ref{fig:cdf_l} and ~\ref{fig:cdf_u} $M/N=0.2$.

%The helpers are placed hexagonally next to each other in the topology. We say that the edge of a helper has unit length, i.e. $1$. We let $r_{trans}=1$, $r_{inter}=1,2$. Since the length of the edges and $r_{trans}$ are equal this implies that a user can be served at most by two different helpers. The users are placed according to a homogeneous Poisson Point Process within a circle of area $A$ which contains the union of the transmission circles of the helpers which we denote by $A_H$ so that $A>A_H$. Let $n$ be the number of helpers. To ensure a fixed predetermined number of average user per helper $c$, we choose the density of the users $\lambda=nc/A_H$. We put the users which are not in any $r_{trans}$ radius of any helper out of the system since they can not be served and we have average of $nc$ number of users in the system. Each user in the system chooses a cache group $l$ randomly and independent of the other users. This implies that the density of the users in the same cache group $l$ is $\lambda_l=nc/(A_HL)$.

%We find the average final rates of the users with optimal method, super-user method and heurestics by averaging over (20 or 100 or etc.) topologies. 

\begin{table}[t]
    \centering
    \begin{tabular}{c||c|c|c|c|c|c}
         $U$ & 5 & 10 & 15 & 20 & 25 & 30  \\
         \hline
         \hline
         Analytical & 59 & 138 & & & &  \\
         \hline
         Super-user & 60 & 142 & 229 & 336 & 443 & 533 \\
         \hline
         RGA & 63 & 147 & 236 & 347  & 455  & 551 
    \end{tabular}
    \caption{$\mathrm{round}(|f|)$ vs average users per helper $U$, $L=5$.}
    \label{tab:utiliy_u}
\end{table}

\begin{table}[t]
    \centering
    \begin{tabular}{c||c|c|c|c|c}
         $L$ & 1 & 5 & 10 & 15 & 20 \\
         \hline
         \hline
         Analytical &  86 & 75 & 72 & 70 & 69 \\
         \hline
         Super-user & 95 & 78 & 74 & 72 & 71 \\
         \hline
         RGA & 98 & 84 & 81 & 79 & 78
    \end{tabular}
    \caption{$\mathrm{round}(|f|)$ vs cache profile count $L$, $U=10$.}
    \label{tab:utiliy_l}
\end{table}

%Keypoints:(Utility table:We can see that for fixed L as U increases  the utility of all the schemes decrease since in table we have $|f|$ as expected, however all the schemes are close to each other, especially the super-user method is much closer compared to RGA. For fixed U as L increases especially after L=5 since U=10 all the algorithms converge to their utility values where all users have different caches, i.e. there is no reduced subpacketization order.Note that for fixed L we calculate rate as number of chunks/total number of codewords transmitted, for fixed U we calculate rate as number of chunks/time assuming $C_{access}=C_{front}=F=1$ as in \cite{mozhgan}).






 \begin{figure}[htp]
     \centering
     \includegraphics[width=10cm]{Figs/All_methods_L=1.eps}
 \end{figure} 

 \begin{figure}[htp]
     \centering
     \includegraphics[width=10cm]{Figs/All_methods_L=3.eps}
 \end{figure} 

 \begin{figure}[htp]
     \centering
     \includegraphics[width=10cm]{Figs/All_methods_L=6.eps}
 \end{figure} 

 \begin{figure}[htp]
     \centering
     \includegraphics[width=10cm]{Figs/All_methods_L=9.eps}
 \end{figure}


 \begin{figure}[htp]
     \centering
     \includegraphics[width=10cm]{Figs/Antenna_both_methods_gain_L=1-6.eps}
 \end{figure}

 \begin{figure}[htp]
     \centering
     \includegraphics[width=10cm]{Figs/2_antenna_2_methods.eps}
 \end{figure}

==> old_SysModel.tex <==
%The system model will take about 0.75 of a page.

%Put figures for the system model and the graphs.

%Explain the caching scheme.

%Explain the problem, which is how to do the delivery.

%You can briefly discuss the next chapters: we first solve the problem using solutions with convex optimization (Analytical solutions), and then, provide a heuristic solution (Put a name for your algorithm).

%\textbf{WRITE THE SYSTEM MODEL BEFORE GOING INTO THE TECHNICAL DISCUSSIONS.} \\

%\todo[inline]{here starts the text:}

\begin{figure}[t]
    %\begin{subfigure}{0.3\columnwidth}
        \centering
        \includegraphics[width = 0.8\columnwidth]{Figs/NetworkModel.png} \label{fig:network_model}
        \vspace{-1pt}
    \caption{Example network with $H=2$, $K=5$.}
    \vspace{-12pt}
    \label{fig:network_model}
\end{figure}


The system model considered in the paper is the extension of the broadcast/collision model of~\cite{mozhgan}, [ISIT] to the multi-antenna case: A single server, connected to $H$ multi-antenna helper nodes (APs in WLAN) via error-free fronthaul links, serves the requests of $K$ single-antenna, cache-enabled users. We use $h_i$ and $u_k$, $i \in [H]$ and $k \in [K]$, to represent helpers and users, respectively. Every $u_k$ is connected to a limited number of helpers via a wireless access network, and every $h_i$ can transmit data with the spatial multiplexing gain of $\alpha$\footnote{This requires that the helper nodes have at least $\alpha$ transmit antennas.}
%has $\alpha$ antennas and
within an effective transmission radius of $r_{\mathrm{trans}}$ and an interference radius of $r_{\mathrm{inter}} \ge r_{\mathrm{trans}}$. We call a helper $h_i$ `active' at a time instant if it is transmitting data in that time instant. Denoting the locations of the helper $h_i$ and user $u_k$ as $\Sfx(h_i), \Sfx(u_k) \in \mathbb{R}^2$, respectively, $u_k$ can successfully decode the received message transmitted by $h_i$ if and only if 1) $|\Sfx(h_i) - \Sfx(u_k)| \le r_{\mathrm{trans}}$, and 2) if $u_k$ is in the interference radius of another active helper $h_{i'}$, the interference caused by $h_{i'}$ is nulled out with transmit precoders at $h_{i'}$ (this will be elaborated more shortly).
%$u_k$ doesn't receive any kind of transmission from another active helper node $h_{i'}$. The necessary condition for $u_k$ to receive any kind of transmission from an active helper $h_i$ is $|\Sfx(h_i) - \Sfx(u_k)| \le r_{\mathrm{inter}}$ and the sufficient condition will be clear later. 
A graphical representation of the system model is shown in Figure~\ref{fig:network_model}.

Similar to [ISIT], we also consider a video streaming application as the use case. We assume every video file is split into multiple `chunks,' each representing a few seconds of the multimedia content, and a user streaming a video generates a sequence of requests for the corresponding chunks of that video. We denote the total number of chunks (for all video files) in $N$, 
%there exist a total number of $N$ chunks (for all video files), 
every chunk has the same size, and every user has a cache memory large enough to store at most $M<N$ chunks. We also use $W_n$, $n \in [N]$, to denote a general video chunk.% and $\CF$ to represent the set of all chunks. 
%
%The total multicast capacity of each helper is assumed to be $C_{\mathrm{access}}$.
%
%We have the broadcast/collision model of \cite{mozhgan} where we have one server, $H$ helpers, $N$ files $W_n$ where $n\in{\lbrace1,2,...,N\rbrace}$ and each file $W_n$ has $F$ bits and $K$ users where each user can cache up to $MF$ bits and $M\in{\lbrace0,1,...,N\rbrace}$. The server is connected to the helpers with $H$ error-free fronthaul links with capacity $C_{front}$ bits/s where each helper has a multicast capacity of $C_{access}$ bits/s. Each helper $h_i$ and each user $u_k$, where $i\in{\lbrace1,2,...,H\rbrace}$ and $k\in{\lbrace1,2,...,K\rbrace}$, are on a 2-dimensional plane in $\mathbb{R}^2$ such that the positions of user $u_k$ and helper $h_i$ on the plane will be denoted by $x(u_k)$ and $x(h_i)$ respectively where $x(h_i),x(u_k)\in{}\mathbb{R}^2$. Each helper $h_i$ has a radius of effective transmission $r_{trans}$ and a radius of interference $r_{inter}$ such that $r_{trans}\leq{}r_{inter}$. A  user $u_k$ can successfully decode the transmitted message of $h_i$ if and only if $\vert{}x(h_i)-x(u_k)\vert{}\leq{}r_{trans}$ and there is no other helper $h_{i'}$ transmitting a message at the same time instance where $\vert{}x(h_{i'})-x(u_k)\vert{}\leq{}r_{inter}$. We say that a helper $h_i$ is `active' at a time instance if it is transmitting.

System operation consists of two phases, placement and delivery. During the placement phase, users' cache memories are filled up with subpackets (i.e., smaller portions) of all the video chunks. Similar to [ISIT], we use the decentralized cache replication algorithm of~\cite{caire,parrinellomultiantenna}:\footnote{The cache replication model helps reduce the subpacketization~\cite{caire,parrinellomultiantenna}.} we fix a number of $L < K$ \emph{cache profiles} and assign each user randomly to one of the profiles. Let us use $\SfL(u_k) \in [L]$ to denote the cache profile assigned with user $u_k$. Given $L$, we define $t = \frac{LM}{N}$ and divide every chunk $W_n$, $n \in [N]$, into $\binom{L}{t}$ non-overlapping equal-sized subpackets $W_{n,\CS}$, where $\CS$ can be any subset of $[L]$ with size $|\CS| = t$. Then, if $\SfL(u_k) = l$ for a user $u_k$, it stores every subpacket $W_{n,\CS}$, for every $n \in [N]$ and $\CS \ni l$. Clearly, all users assigned to the same profile will cache the same data.

%For the cache placement, we use the decentralized cache replication method of \cite{caire} which is an extension of the MAN cache placement \cite{maddah2014fundamental}. We fix $L<K$ and define $\gamma=LM/N$ where $\gamma$ is an integer and $0\leq{}\gamma\leq{}L$, and we divide every file $W_n$ to $\binom{L}{\gamma}$ non-overlapping equal sized subfiles  $W_{n,\mathcal{T}}$ where $\mathcal{T}\in{\Omega_\gamma^L}$ such that $\Omega_\gamma^L=\lbrace{}U\subseteq{\lbrace1,2,...,L\rbrace} : |U|=\gamma\rbrace{}$. For each user $u_k$, where $k\in{\lbrace1,2,...,K\rbrace}$, an integer $l\in{\lbrace1,2,...,L\rbrace}$ is randomly chosen independently of the other users which corresponds to the cache group of the user and user $u_k$ caches the subfiles $W_{n,\mathcal{T}}$ for all  $\mathcal{T}\ni{l}$ and all $n\in{\lbrace1,2,...,N\rbrace}$. Notice that the subfiles stored in the caches of the users in the same cache group are identical.

During the delivery phase, users reveal their requested video chunks (corresponding to the videos they want to stream). We assume users can start streaming at arbitrary times, and when they start streaming, they repeatedly generate requests for consecutive video chunks. With this model, we can safely assume a single chunk is requested by at most one user at a given time, as even if two users are streaming the same video, it is unlikely that they have started streaming at the same time. Given the set of user requests and
%In this paper, we consider data delivery after every user has revealed their requested chunk sequence. Then, 
using a delivery algorithm, 
the server creates a number of transmission vectors and transmits them through a selection of active helpers. The goal is to serve requested video chunks while optimizing a performance function of, e.g., delivery time, energy, or fairness.

%In this paper, we first use the following two simplifying assumptions to find an optimal delivery solution in Section~\ref{section:optimal_solution}: 1) network topology is static, and the users do not move during the delivery session, and 2) each user instantly requests another file after it receives the previously requested one.\footnote{A real-world example can be a video delivery application in a large hall (e.g., an airport), where multiple Wi-Fi routers facilitate data transmission. Files in $\CF$ represent chunks of the video files, and every user requests the next chunk right after it finishes the reception of the previous one.}
%We also assume the worst-case scenario where the users request different files.\footnote{This is a fair assumption for the example video delivery application. This is because even if two users are watching the same video, there is little chance that they have started streaming simultaneously.}
%Then, in Section~\ref{section:kagan_solution}, we provide a heuristic solution that supports dynamic network conditions and non-continuous file requests.

%\todo[inline]{the following part needs changing: users are static and always have requests. there is no concept of a time frame}
%In this paper, we slightly simplify this model: we assume the time horizon is divided into multiple time frames, and users' requests are queued until the starting point of the next frame. Then, at the beginning of each frame, the server fetches every request in the queue and uses the delivery algorithm to serve them efficiently. We assume users being served in a time frame do not change their locations during that frame. The next time frame begins right after all the requests at the beginning of the previous frame are fully served. Using this model, without losing practicality, we can assume the same procedure is repeated in each frame and eliminate the frame index.

With $H$ helpers that can be either active or inactive, there exist $2^H$ selections for the \emph{activation pattern} of the helpers. 
%An active helper $h_i$ may choose not to send any transmission to maximum of $\alpha-1$ users $u_k$ such that $|\Sfx(h_i) - \Sfx(u_k)| \le r_{\mathrm{inter}}$ by transmitting ZF-precoded vectors~\cite{parrinellomultiantenna,lampiris2018adding} and this can be helpful if the users $u_k$ can be served by other helpers $h_{i'}$. We call this `interference cancellation'. 
Let us use vectors $\Bp_j$, $j \in [2^H]$, to denote activation patterns. Every $\Bp_j$ has $H$ binary elements $\Bp_j[i]$, $i \in [H]$, and $\Bp_j[i] = 1$ only if helper $h_i$ is active in the corresponding activation pattern. 
%The activation pattern determines which users can be served by each active helper and whether they can be served by multicasting codewords instead of unicasting.
%the user(s) that each active helper can serve. It also clarifies if these users can be served through codeword multicasting:
%
We assume zero-force (ZF) transmit precoders (i.e., beamformers) are used at every active helper.\footnote{For appropriate performance in the finite-SNR regime...} As the spatial multiplexing gain is $\alpha$, these precoders can null out every data stream at up to $\alpha-1$ users. We also make the simplifying assumption that irrespective of the precoder design, the transmit and interference radii do \emph{not} change...

\todo[inline]{This paragraph still needs to be completed.}

The codeword creation is done as in~\cite{parrinellomultiantenna} where a codeword can be created for every subset of users $\CV$ of size $0 < |\CV| \le \alpha(t + 1)$ if all users in $\CV$ are served by the same active helper $h_i$ where the total number of distinct cache profiles of users in $\CV$ is upper bounded by $t+1$ and the total number of users having the same cache profile in $\CV$ is upper bounded by $\alpha$ for each cache profile. \textbf{We can put a footnote here and say we can do better for larger number of antennas}. We call this `congestion control'. Notice that for every activation pattern $\Bp_j$, an active helper $h_i$ may choose to do interference cancellation for $\beta$ number of users and can serve $\gamma$ number of users with the same cache profile with the same codeword by doing congestion control such that $\beta+\gamma=\alpha$. However, for the sake of simplicity we assume that every active helper $h_i$ in an activation pattern either does interference cancellation for maximum of $\alpha-1$ users or does congestion control and can serve extra $\alpha-1$ users for each cache profile compared to the single antenna case [ISIT]. Of course, due to the repetition in cache profile assignments, for instance for congestion control if more than $\alpha$ users have the same cache profile for an active helper given an activation pattern, multiple choices for the size of $\CV$ and for interference cancellation choosing from different possible set of users not to transmit, there may exist multiple codeword creation possibilities for each helper.
Codeword creation %follows the same basics of~\cite{maddah2014fundamental,caire} and 
is explained in more detail in Section~\ref{section:optimal_solution}. 

The server may need to choose multiple activation patterns to serve all the requests. This is because it is likely that for a specific pattern $\Bp_j$, some users could not be served at all due to interference from active helpers and cache congestion. 
%Multiple patterns may be activated over various communication resources. In this paper, we assume consecutive time slots are used, where every pattern $\Bp_j$ is activated for $a_j \ge 0$ seconds. 
Moreover, as discussed, we may have multiple choices for codeword creation with every activation pattern. Let us assume the number of such choices for activation pattern $\Bp_j$ is $\Sfc(\Bp_j)$.
We use the term \emph{policy} to refer to a selection of an activation pattern and a codeword creation choice, and $\pi(j,s_j)$ to represent the policy resulting from activation pattern $\Bp_j$ and codeword choice $s_j$, $s_j \in [\Sfc(\Bp_j)]$. 
Clearly, the total number of policies is $\sum_{j \in [2^H]} \Sfc(\Bp_j)$.
Every policy $\pi(j,c_j)$ results in a rate vector $\Br(j,c_j)$, where the element $k$, $k \in [K]$, in $\Br(j,s_j)$ denotes the rate of user~$u_k$ with policy $\pi(j,s_j)$. The network throughput region is defined as the convex hull of all rate vectors, shown by $\mathrm{Conv}(\Br(j,s_j))$. The goal is to optimize a fairness function of the rate values, which can be any concave component-wise non-descending function over $\mathrm{Conv}(\Br(j,s_j))$. For example, we may choose any function from the alpha-fairness family~\cite{fairness}: for $\alpha = 1$, we get proportional fairness; for $\alpha = 0$, we get sum-rate (unfair); and for $\alpha \rightarrow \infty$, we get max-min (hard) fairness. In this paper, for the sake of brevity, we chose the proportional fairness function $\Sff = \sum_k \log(r_k)$ as our metric, where $r_k$ is the time-averaged delivery rate of user ~$u_k$ (usually referred to as the `throughput rate’).

%Multicasting enables more users to be served with a single transmission, thus enhancing the system's performance. 
%So, intuitively, we like to create as many codewords as possible for any given activation pattern $\Bp_j$.
%A coded transmission through active helper $h_i$ is possible if the users served by $h_i$ are assigned to different cache profiles.

%Given a pattern $\Bp_j$, the server may be able to create one or multiple codewords for every active helper $h_i$.
%The final step is determining which users could be served simultaneously with a single codeword. 
 
%(i.e., $\SfL(u_k) \neq \SfL(u_m)$ for distinct users $u_k, u_m \in \CU_i$). 

%\todo[inline]{we should provide a hint to how the codewords are created, either in general form or using an example}
%Of course, here we have the extra condition that the users served by a single codeword should all be connected to (\textbf{DEFINE CONNECTION}) the same helper node.
%\todo[inline]{Maybe an example here.}







%Successful data delivery may require using multiple policies, which can be done over various communication resources. In this paper, without loss of generality, we assume consecutive time slots are used, where every policy $\pi(j,s_j)$ is used for $a(j,s_j) \ge 0$ seconds. 
%As we will see in Section~\ref{section:optimal_solution}, every policy $\pi(j,s_j)$ results in a rate vector $\Br(j,s_j)$, where the element $k$, $k \in [K]$, in $\Br(j,s_j)$ denotes the rate of user~$u_k$ with policy $\pi(j,s_j)$. Then, the sum rate vector can be defined as
%\begin{equation}
%    \Br_{\mathrm{sum}} = \sum_{j \in [2^H]} \sum_{s_j \in [\Sfc(\Bp_j)]} a(j,s_j) \Br(j,s_j) .
%\end{equation}
%Let us denote the sum rate of user~$u_k$ (i.e., the element $k$ of $\Br_{\mathrm{sum}}$) as $r_k$.  
%In this paper, we use the proportional fairness function $\Sff = \sum_k \log(r_k)$ as our metric\footnote{In fact, we can choose any function from the alpha-fairness family: for $\alpha = 1$ we get proportional fairness, for $\alpha = 0$ we get sum-rate (unfair), and for $\alpha \rightarrow \infty$ we get max-min (the hard fairness). In this paper, proportional fairness is chosen for sake of brevity.} and try finding $a(j,s_j)$ values such that $\Sff$ is maximized.\\



% \begin{figure}[t]
%     \centering
%     \begin{tikzpicture}[scale=0.6,transform shape]

%         \draw[thick] (2,2) circle (2 cm);
%         \draw[thick] (5,2) circle (2 cm);
%         \draw[red!50,fill=red!50](2,2) circle (0.1 cm);
%         \draw[red!50,fill=red!50](5,2) circle (0.1 cm);
%         \draw[dashed] (2,2) circle (2.7 cm);
%         \draw[dashed] (5,2) circle (2.7 cm);
%         \draw[blue!50,fill=blue!50](3.5,2) circle (0.05cm);
%         \draw[blue!50,fill=blue!50](3,3.2) circle (0.05cm);
%         \draw[blue!50,fill=blue!50](1.2,1.3) circle (0.05cm);
%         \draw[blue!50,fill=blue!50](5.5,2.9) circle (0.05cm);
%         \draw[blue!50,fill=blue!50](4.8,0.8) circle (0.05cm);

%     \end{tikzpicture}
%     \caption{Example network with $H=2$, $K=5$.}
%     \label{fig:network_model}
% \end{figure}

%In this example number in parantheses corresponds to cache group $l$ of the users. $L=3$, $\gamma=1$. We have $3$ instantaneous maximal rate vectors which maximizes the number of users per helper and 3 maximal superuser vectors. $[0.5, 0, 0, 0, 0.33, 0.33]$, $[0.33, 0.33, 0.33, 0, 0]$ and $[0, 0, 0.33, 0.33, 0]$ corresponds to former, $[0.5 ,0 ,0 ,0 ,0.33, 0.33]$, $[0.33 ,0.33 ,0.33 ,0 ,0]$ and $[0, 0 ,0.167 ,0.33 ,0.167]$ corresponds to latter.


%As we will see in Section~\ref{section:optimal_solution}, a selection of an activation pattern and a codeword creation choice results in a rate vector $\Br_q$, $q \in Q$, where $Q = \sum_{j \in [2^H]} \Sfc(\Bp_j)$ is the total number of such selections and the element $k$, $k \in [K]$ in $\Br_q$ denotes the rate of user $u_k$ if policy $\pi_q$ is selected. 

%\todo[inline]{here comes the definition of the rate}

%Moreover, for a given activation pattern of helpers, the server may have multiple choices for creating codewords (as multiple users with the same cache profile may be connected to the same active helper). The result is multiple rate vectors $\Br$ ...

%Also, the server may have to choose multiple activation patterns in a single time frame, as every user requesting data at the beginning of the time frame may not be served with a single activation pattern. Multiple activation patterns could be activated over any orthogonal network resource. In this paper, we assume the time frame is split into smaller time intervals of size $a_j$, and the rate vector $\Br_j$ is achieved for a time duration of $a_j$. The goal is to find out the rate vectors $\Br_j$ and the weights $a_i$ such that ...
%\todo[inline]{The optimization problem comes here.}
%\todo[inline]{Big question: where to discuss how the rate vectors are created?}

%\todo[inline]{The discussion should be more general here: given a specific pattern, the server has multiple choices for creating codewords, depending on which users could be served by every active helper and what the assigned profile of each user is. The selection of active helpers and the users to be served provides us with a respective rate vector for that activation pattern. The goal is to describe how this vector could be found, then. The question is, where to describe each part? System model or the next section?}
%\todo[inline]{I think it is better to describe the codeword generation process here, maybe a toy example. The graph representation can be moved to the next section, then. But the rate function should be defined here.}
%consider a set of users $\CU_h$ that all can receive data from an active helper $h \in [H]$ and every user $u_k \in \CU_h$ is assigned to a different cache profile $\SfL(k) \in [L]$. As the number of profiles is $L$, we must have $|\CU_h| \le L$. Then, for every non-empty subset of users $\CT_h \subseteq \CU_h$ with $|\CT_h| \le \gamma+1$, the server can create the codeword
%\begin{equation}
%\label{eq:exmp_XOR}
%    \bigoplus_{u_k \in \CT_h} W_{d_k,} \quad,
%\end{equation}
%where $\oplus$ denotes the bit-wise XOR operation, and send it to every user $u_k \in \CT_h$ through helper $h$, so that every user $k \in \CT_h$ receives part of its requested file $W_{d_k}$. This is possible because after receiving the codeword, every user $u_k \in \CT_h$ can use its cached content to remove the unwanted terms, and decode ... .

%\todo[inline]{now we should explain the delivery phase. Mohammad to do this by 27.1}

%During the delivery phase, network users reveal their requested files.
%\begin{itemize}
%    \item multiple codewords can be sent in parallel.
%    \item we have many choices for activation patterns.
%    \item we need to have multiple time intervals to serve all the users (as all the users might not be served with a single pattern).
%    \item every selection of activation pattern gives us a rate vector.
%    \item the length of the time intervals should also be defined.
%    \item the goal is to optimize the $\sum \log$ function.
%\end{itemize}

%\todo[inline]{The old text}

%As in \cite{mozhgan}, the number of XORs a helper needs to serve all the users in its delivery column is $\binom{L}{\gamma+1}-\binom{L-l'}{\gamma+1}$ where $l'$ is the number of users in the delivery column.

%(We assume $F=C_{access}=C_{front}$ so that the time it takes a helper to serve all the $l'$ users in its delivery column is $(\binom{L}{\gamma+1}-\binom{L-l'}{\gamma+1})/\binom{L}{\gamma}$.)

%\todo[inline]{The old text}

%We define the rate $R_k$ of a user $u_k$ in a delivery scheme as the (average) percentage of a file $u_k$ receive per one XOR transmission. The aim of this paper is to maximize the rates of the users by also being `fair' to the users, to be more rigorous, we do proportional fairness utility maximization of the rates. Let $\mathbf{D}$ be the set of all possible delivery schemes for a fixed topology with predetermined caches of the users. Let $\mathbf{R}=\lbrace{}R_1,R_2,...,R_k\rbrace{}$. Then $\arg(\max_{\mathbf{D}}\sum_{k}\log{R_k}):=d^*$ is the delivery scheme which maximizes the proportional fairness utility function.

%In the next sections we show how to find $d^*$ exactly by using convex optimization over a convex set, we also show an (approximation) which we call the `super-user method'. We also show a heurestics method which follows a different approach but finds a rate vector $R'$ which is fairly close to the optimal rate vector $R^*$ found by using $d^*$.



==> old_intro.tex <==
%\todo[inline]{bold-face sentences to be checked by Kagan}

\todo[inline]{Tentative budget: 1 page for intro, 1 page for system model, 1 page for single-antenna work, 1 page for interference cancellation, 1 page for congestion control, and the last page for simulation results and references.}

The increasing amount of data traffic, especially driven by multimedia applications, has necessitated the development of new communication techniques. One interesting resource is on-device memory; it is cheap and can be used to proactively store a large part of multimedia content, e.g., for video-on-demand (VoD) applications. As a result, many researchers have considered the efficient use of onboard memory in the context of \emph{caching}. Pioneering works in this regard introduced femtocaching~\cite{shanmugam2013femtocaching} and F-RAN models~\cite{park2016joint}. A major breakthrough happened with the introduction of coded caching (CC)~\cite{maddah2014fundamental}, which showed that a speedup factor in the achievable rate, scaling with the cumulative cache size in the network, is possible by multicasting carefully created codewords. Later, many works extended the original work of~\cite{maddah2014fundamental}, e.g., for wireless~\cite{tolli2017multi}, multi-server~\cite{shariatpanahi2016multi}, multi-antenna~\cite{shariatpanahi2018physical,parrinellomultiantenna}, and multi-hop networks with helpers assisting the communication~\cite{mozhgan}. 
%Many extensions of the original model exist, e.g., for wireless links~\cite{tolli2017multi}, multi-server~\cite{shariatpanahi2016multi} and multi-antenna~\cite{shariatpanahi2018multi,salehi2021MIMO} setups, and multi-hop networks with or without processing capabilities in the middle nodes~\cite{mozhgan}. 
Meantime, many challenges hindering the applicability of CC techniques in real networks were addressed. For example, the subpacketization bottleneck was studied for single- and multi-antenna setups~\cite{lampiris2018adding,salehi2020lowcomplexity}, simpler beamformer designs were introduced~\cite{salehi2020lowcomplexity,mahmoodi2021low}, and the problem of supporting network dynamicity was addressed~\cite{caire,salehi2021low,abolpour2022coded}.

\textbf{REFER TO OUR RECENT ISIT SUBMISSION AS WELL AS MOZHGAN'S.}
In this paper, following a system model similar to~\cite{mozhgan}, we consider the application of CC in two-hop wireless local area networks (WLAN), where a single server transmits data to a large number of users through multiple access points (AP). WLANs play an important role in wireless data delivery; they facilitate data access, e.g., in our homes, malls, airports, and cars. Two important properties of WLANs are a) unit frequency reuse due to the scarce availability of unlicensed bands and b) the collision-type interference model (i.e., packets are lost if a receiver gets the superposition of concurrent packets, all above a certain interference threshold, from different APs). Considering multi-AP WLANs and single per-user requests, the authors in~\cite{mozhgan} optimized the worst-case delivery time of all requests. Using basic principles of the multi-round delivery method in~\cite{caire} (which was later proved by~\cite{parrinellomultiantenna} to be optimal for the shared-cache model), they first used graph coloring to construct a reuse pattern of APs and optimized the AP-user allocation to minimize the delivery time. Next, they introduced the `Avalanche' algorithm to leverage the interference-free state of the users as APs finished their multi-round delivery.

%This paper builds upon earlier work in~\cite{mozhgan} on extending the original scheme of~\cite{maddah2014fundamental} to two-hop networks. We use the same data placement and user allocation to caching profiles as in~\cite{caire} as it allows handling network dynamicity with controlled subpacketization. We build our work upon the more practical broadcast/collision model used there, which considers a network with broadcast constraints at the helpers and collision interference at the users. The work in~\cite{mozhgan} considers the case where each user in the system requests a single file and investigates the worst case delivery time of all of the user requests. 
%Based on multi-round delivery of ~\cite{caire}, which was proven to be optimal for the shared-link model in \cite{parinello}, Mozhgan et. al. use graph coloring for constructing a reuse pattern of helpers and then optimize the allocation between the helpers and the users and also another method which they call Avalanche where they leverage users becoming free of interference when helpers finish their multi-round delivery. 

\textbf{THIS PARAGRAPH NEEDS TO CHANGE. WE DON'T NEED TO MENTION THE WEAKNESSES OF MOZHGAN'S WORK ANYMORE. WE HAVE TO FOCUS ON EXTENDING THE ISIT WORK TO MULTI-ANTENNA SETUPS. A BASIC OUTLINE OF THE TWO IDEAS SHOULD BE REPRESENTED.}
Both the graph coloring and avalanche schemes of~\cite{mozhgan} are heuristic methods, however, and while they compare well with the multi-round method of~\cite{caire}, neither of them achieves any optimality metric. Moreover, the single-request assumption of~\cite{mozhgan} is not appealing for real-world implementation of CC techniques in WLAN. This is because, in practice, CC applied to VoD streaming requires the sequential delivery of a long sequence of ``chunks’’ forming the streaming session. Each chunk contains a relatively small segment of video, and the chunks must be delivered at a rate (slightly) higher than the playback rate at which the video buffer is emptied at the user video player application.  Hence, the most important requirement is the delivery rate in terms of chunks per unit of time rather than the worst-case single-request delivery time considered by~\cite{mozhgan}. Accordingly, in this paper, we consider a multi-AP WLAN model similar to~\cite{mozhgan} but with sequential requests. We obtain a computational way to determine the theoretical throughput region of per-user delivery rates and solve the fairness scheduling problem, which maximizes a desired fairness metric of user delivery rates over this region. We also provide two heuristic methods based on restricting the throughput region and a greedy algorithmic approach to achieve a sub-optimal solution with reduced complexity. Numerical analyses are used to evaluate the performance of the proposed solutions.

%(Maybe no need to mention this:The problem in Avalanche lies in the fact that for initialization it assumes that there are users which are in the tranmission radius of a helper free from interference of other helpers and also while the algorithm is running if more than one helper finish at the same time there may not be another helper to serve the users which are freed from their interference since they may be the only ones who can serve them at the first place.)

%(\textbf{WRITE THE MAIN CONTRIBUTIONS OF MOZHGAN'S WORK}, we formulate the problem as \textcolor{blue}{designing a transmission strategy over a set of possible actions, and show that the problem can be solved with linear programming (?). However, the complexity grows exponentially (?) with network dimensions. Then, we introduce a heurisitic algorithm to solve the problem sub-optimally. Finally, we show through simulations that the gap between the heurisitic method and the optimal solution is small.} \textbf{WRITE YOUR OWN IDEA OF OUR CONTRIBUTION INSTEAD OF THE BLUE TEXT.})

%\todo[inline]{the super-user idea should be fit in-between}

%\todo[inline]{I need to read Mozhgan's paper and talk with Kagan to find the novelty aspects better}

%\todo[inline]{Should we go into details of the video delivery application already in the introduction? If we have extra space, we will put one paragraph here.}

%\todo[inline]{One paragraph describing the notations. Mohammad will do that.}
%So, $\Ba$ is a vector, and $\BA$ is a matrix, and $\CA$ is a set.

%In this paper, we have used the following notations...
We have used boldface lower- and upper-case letters to denote vectors and matrices, respectively. Sets are represented by calligraphic letters. $\Bv[i]$ is the element $i$ of vector $\Bv$, and $\CA \backslash \CB$ denotes the set of elements of $\CA$ not in $\CB$. For integer $J$, $[J]$ represents the set $\{1,2,\cdots,J\}$. $\binom{n}{k}$ denotes binomial coefficient, and its value is zero if $n < k$. %Other notations are defined as used in the text.

%\todo[inline]{Here starts the revised text}



%The intro and abstract will take about 1 page.


%In the introduction:
%\begin{enumerate}
%    \item Why we are doing this? There is lots of traffic ...
%    \item CC scheme is good to address this issue ...
%    \item There are problems and some of them are addressed ...
%    \item One other issue is the application of CC techniques in a multi-level network. In this paper, we address the ...
%    \item Some other ideas: users are repeatedly asking for content, and references to the previous work, ...
%    \item A paragraph briefly explaining the idea and novel parts. Novel parts are the original solution, the super-user idea and the algorithm.
%    \item A paragraph or sentence about how you are evaluating your new algorithm and what are the results.
%\end{enumerate}

%Some other notes:
%\begin{enumerate}
%    \item We need to explain the super-user idea already in this paper. Because otherwise, we cannot produce nice simulation results.
%\end{enumerate}
